Reinforcement Learning for Traffic Signal Control: Comparison with Commercial Systems

Recently, Intelligent Transportation Systems are leveraging the power of increased sensory coverage and computing power to deliver data-intensive solutions achieving higher levels of performance than traditional systems. Within Traffic Signal Control (TSC), this has allowed the emergence of Machine Learning (ML) based systems. Among this group, Reinforcement Learning (RL) approaches have performed particularly well. Given the lack of industry standards in ML for TSC, literature exploring RL often lacks comparison against commercially available systems and straightforward formulations of how the agents operate. Here we attempt to bridge that gap. We propose three different architectures for TSC RL agents and compare them against the currently used commercial systems MOVA, SurTrac and Cyclic controllers and provide pseudo-code for them. The agents use variations of Deep Q-Learning and Actor Critic, using states and rewards based on queue lengths. Their performance is compared in across different map scenarios with variable demand, assessing them in terms of the global delay and average queue length. We find that the RL-based systems can significantly and consistently achieve lower delays when compared with existing commercial systems.

==> TRPRO_14CTE_2021 <==
SyncTeX Version:1
Input:1:D:\Narendra_Journals\Elsevier\Procedia_Templates\13-03-2019\TRPRO_EWGT_2018_TeX_Template\trpro-template-EWGT_2018.tex
Input:2:D:\Narendra_Journals\Elsevier\Procedia_Templates\13-03-2019\TRPRO_EWGT_2018_TeX_Template\elsarticle.cls
Input:3:C:\Program Files\MiKTeX 2.9\tex\latex\base\article.cls
Input:4:C:\Program Files\MiKTeX 2.9\tex\latex\base\size10.clo
Input:5:C:\Program Files\MiKTeX 2.9\tex\latex\graphics\graphicx.sty
Input:6:C:\Program Files\MiKTeX 2.9\tex\latex\graphics\keyval.sty
Input:7:C:\Program Files\MiKTeX 2.9\tex\latex\graphics\graphics.sty
Input:8:C:\Program Files\MiKTeX 2.9\tex\latex\graphics\trig.sty
Input:9:C:\Program Files\MiKTeX 2.9\tex\latex\graphics-cfg\graphics.cfg
Input:10:C:\Program Files\MiKTeX 2.9\tex\latex\graphics-def\xetex.def
Input:11:C:\Program Files\MiKTeX 2.9\tex\latex\psnfss\pifont.sty
Input:12:C:\Program Files\MiKTeX 2.9\tex\latex\psnfss\upzd.fd
Input:13:C:\Program Files\MiKTeX 2.9\tex\latex\psnfss\upsy.fd
Input:14:D:\Narendra_Journals\Elsevier\Procedia_Templates\13-03-2019\TRPRO_EWGT_2018_TeX_Template\trpro-template-EWGT_2018.spl
Input:15:C:\Program Files\MiKTeX 2.9\tex\latex\natbib\natbib.sty
Input:16:C:\Program Files\MiKTeX 2.9\tex\latex\geometry\geometry.sty
Input:17:C:\Program Files\MiKTeX 2.9\tex\generic\oberdiek\ifpdf.sty
Input:18:C:\Program Files\MiKTeX 2.9\tex\generic\oberdiek\ifvtex.sty
Input:19:C:\Program Files\MiKTeX 2.9\tex\generic\ifxetex\ifxetex.sty
Input:20:C:\Program Files\MiKTeX 2.9\tex\xelatex\xetexconfig\geometry.cfg
Input:21:D:\Narendra_Journals\Elsevier\Procedia_Templates\13-03-2019\TRPRO_EWGT_2018_TeX_Template\framed.sty
Input:22:C:\Program Files\MiKTeX 2.9\tex\latex\txfonts\txfonts.sty
Input:23:D:\Narendra_Journals\Elsevier\Procedia_Templates\13-03-2019\TRPRO_EWGT_2018_TeX_Template\ecrc.sty
Input:24:C:\Program Files\MiKTeX 2.9\tex\latex\base\fleqn.sty
Input:25:C:\Program Files\MiKTeX 2.9\tex\latex\base\fleqn.clo
Input:26:C:\Program Files\MiKTeX 2.9\tex\latex\amsfonts\amssymb.sty
Input:27:C:\Program Files\MiKTeX 2.9\tex\latex\amsfonts\amsfonts.sty
Input:28:C:\Program Files\MiKTeX 2.9\tex\latex\graphics\rotating.sty
Input:29:C:\Program Files\MiKTeX 2.9\tex\latex\base\ifthen.sty
Input:30:C:\Program Files\MiKTeX 2.9\tex\latex\hyperref\hyperref.sty
Input:31:C:\Program Files\MiKTeX 2.9\tex\generic\oberdiek\hobsub-hyperref.sty
Input:32:C:\Program Files\MiKTeX 2.9\tex\generic\oberdiek\hobsub-generic.sty
Input:33:C:\Program Files\MiKTeX 2.9\tex\latex\oberdiek\auxhook.sty
Input:34:C:\Program Files\MiKTeX 2.9\tex\latex\oberdiek\kvoptions.sty
Input:35:C:\Program Files\MiKTeX 2.9\tex\latex\hyperref\pd1enc.def
Input:36:C:\Program Files\MiKTeX 2.9\tex\latex\00miktex\hyperref.cfg
Input:37:C:\Program Files\MiKTeX 2.9\tex\latex\url\url.sty
Input:38:C:\Program Files\MiKTeX 2.9\tex\latex\hyperref\hxetex.def
Input:39:C:\Program Files\MiKTeX 2.9\tex\latex\hyperref\puenc.def
Input:40:C:\Program Files\MiKTeX 2.9\tex\generic\oberdiek\stringenc.sty
Input:41:C:\Program Files\MiKTeX 2.9\tex\latex\oberdiek\rerunfilecheck.sty
Input:42:D:\Narendra_Journals\Elsevier\Procedia_Templates\13-03-2019\TRPRO_EWGT_2018_TeX_Template\trpro-template-EWGT_2018.aux
Input:43:C:\Program Files\MiKTeX 2.9\tex\latex\txfonts\omltxmi.fd
Input:44:C:\Program Files\MiKTeX 2.9\tex\latex\txfonts\omstxsy.fd
Input:45:C:\Program Files\MiKTeX 2.9\tex\latex\txfonts\omxtxex.fd
Input:46:C:\Program Files\MiKTeX 2.9\tex\latex\txfonts\utxexa.fd
Input:47:C:\Program Files\MiKTeX 2.9\tex\latex\txfonts\ot1txr.fd
Input:48:C:\Program Files\MiKTeX 2.9\tex\latex\graphics\color.sty
Input:49:C:\Program Files\MiKTeX 2.9\tex\latex\graphics-cfg\color.cfg
Input:50:C:\Program Files\MiKTeX 2.9\tex\latex\hyperref\nameref.sty
Input:51:C:\Program Files\MiKTeX 2.9\tex\generic\oberdiek\gettitlestring.sty
Input:52:C:\Program Files\MiKTeX 2.9\tex\latex\txfonts\omstxr.fd
Input:53:C:\Program Files\MiKTeX 2.9\tex\latex\txfonts\utxmia.fd
Input:54:C:\Program Files\MiKTeX 2.9\tex\latex\amsfonts\umsa.fd
Input:55:C:\Program Files\MiKTeX 2.9\tex\latex\amsfonts\umsb.fd
Input:56:C:\Program Files\MiKTeX 2.9\tex\latex\txfonts\utxsyc.fd
Input:57:C:\Program Files\MiKTeX 2.9\tex\latex\txfonts\ot1txss.fd
Input:58:C:\Program Files\MiKTeX 2.9\tex\generic\oberdiek\se-ascii-print.def
Output:pdf
Magnification:1000
Unit:1
X Offset:0
Y Offset:0
Content:
!4302
{1
[1,222:4736287,44990034:28358645,40253747,0
(1,222:4736287,4736287:0,0,0
)
[1,222:4736287,4736287:0,0,0
(1,222:4736287,2656652:0,0,0
k1,222:4736287,2656652:2377984
)
]
[1,222:4736287,44990034:28358645,40253747,0
[1,222:2424084,44990034:30670848,41969252,0
[1,222:2424084,3676142:30670848,655360,0
(1,222:2424084,7770175:30670848,4749393,113377
(1,222:2424084,7770175:30670848,4749393,113377
g1,222:2587924,7770175
[1,222:2587924,7770175:3538935,4063222,0
(1,222:2587924,7770175:3538935,4063222,0
h1,222:2587924,7770175:0,0,0
r1,222:2587924,7770175:0,4063222,0
g1,222:2417530,7770175
g1,222:2417530,7770175
(1,222:2417530,7770175:3538935,4063222,0
(1,222:2417530,7573567:3538935,3866614,0
(1,222:2417530,7573567:3538935,3866614,0
(1,222:2417530,7573567:3538944,3866624,0
(1,222:2417530,7573567:3538944,3866624,0
(1,222:2417530,7573567:0,3866624,0
(1,222:2417530,7573567:3538944,3866624,0
)
k1,222:2417530,7573567:-3538944
)
)
)
)
)
)
k1,222:6126859,7770175:170394
g1,222:6126859,7770175
)
]
g1,222:6290699,7770175
k1,222:9288976,7770175:2998277
[1,222:9288976,7770175:14942208,4143056,-82576
(1,222:9288976,7770175:14942208,4143056,0
g1,222:9288976,7770175
h1,222:9288976,7770175:0,0,0
(1,222:9288976,7770175:14942208,4143056,0
(1,222:9288976,5568165:14942208,1941046,0
[1,222:9288976,5568165:14942208,1941046,0
(1,222:9288976,4026635:14942208,399516,8685
k1,222:11522683,4026635:2233707
h1,222:11522683,4026635:0,0,0
x1,222:11896423,4026635
x1,222:12154174,4026635
x1,222:13323580,4026635
x1,222:13748309,4026635
g1,222:13904080,4026635
x1,222:15399038,4026635
g1,222:15554809,4026635
x1,222:16022123,4026635
g1,222:16177894,4026635
x1,222:17391571,4026635
x1,222:21997477,4026635
g1,222:21997477,4026635
k1,222:24231184,4026635:2233707
)
(1,222:9288976,5568165:14942208,851965,0
k1,222:13614360,5568165:4325384
h1,222:13614360,5568165:0,0,0
(1,222:13614360,5568165:6291440,851965,0
(1,222:13614360,5568165:6291456,851968,0
(1,222:13614360,5568165:6291456,851968,0
(1,222:13614360,5568165:0,851968,0
(1,222:13614360,5568165:6291456,851968,0
)
k1,222:13614360,5568165:-6291456
)
)
)
)
g1,222:19905800,5568165
k1,222:24231184,5568165:4325384
)
]
)
)
g1,222:24231184,7770175
g1,222:24231184,7770175
)
(1,222:9288976,7573567:14942208,357826,114032
k1,222:11141547,7573567:1852571
h1,222:11141547,7573567:0,0,0
(1,222:11141547,7573567:11237066,357826,114032
x1,222:11461887,7573567
x1,222:14210205,7573567
g1,222:14341277,7573567
x1,222:16262793,7573567
g1,222:16393865,7573567
x1,222:18228349,7573567
g1,222:18359421,7573567
x1,222:18883709,7573567
g1,222:19014781,7573567
x1,222:20412533,7573567
g1,222:20543605,7573567
x1,222:21330037,7573567
x1,222:22378613,7573567
)
g1,222:22378613,7573567
k1,222:24231184,7573567:1852571
)
]
k1,222:27229460,7770175:2998276
(1,222:27229460,7770175:5865472,4749393,113377
(1,222:27229460,5620594:5865472,2599812,2262958
$1,222:27229460,5620594
[1,222:27229460,5620594:5865472,2599812,2262958
(1,222:27229460,5188057:5865472,2167275,1830421
h1,222:27229460,5188057:0,0,0
$1,222:27229460,5188057
[1,222:27229460,5188057:5701632,2167275,1830421
(1,222:27229460,7739362:5701632,4718580,0
h1,222:27229460,7739362:0,0,0
r1,222:27229460,7739362:0,4718580,0
g1,222:25558292,7739362
g1,222:25558292,7739362
(1,222:25558292,7739362:7208942,4718580,0
(1,222:25558292,7739362:7208960,4718592,0
(1,222:25558292,7739362:7208960,4718592,0
(1,222:25558292,7739362:0,4718592,0
(1,222:25558292,7739362:7208960,4718592,0
)
k1,222:25558292,7739362:-7208960
)
)
)
)
k1,222:32931092,7739362:163858
g1,222:32931092,7739362
)
]
$1,222:32931092,5188057
k1,222:33094932,5188057:163840
g1,222:33094932,5188057
)
(1,222:27229460,7769520:5865472,357826,114032
r1,222:27229460,7769520:0,471858,114032
g1,222:25656596,7769520
g1,222:25656596,7769520
x1,222:26792204,7769520
x1,222:27704465,7769520
x1,222:28506626,7769520
x1,222:32855070,7769520
k1,222:33094932,7769520:239862
g1,222:33094932,7769520
)
]
$1,222:33094932,5620594
)
)
)
)
]
[1,222:2424084,44990034:30670848,40658532,0
[1,222:2424084,44244163:30670848,39912661,0
(1,192:2424084,9705454:30670848,536739,171048
k1,192:4944598,9705454:2520514
(1,192:4944598,9705454:0,0,0
g1,192:4944598,9705454
g1,192:4944598,9705454
g1,192:4616918,9705454
(1,192:4616918,9705454:0,0,0
)
g1,192:4944598,9705454
)
x1,192:6517462,9705454
g1,192:6714070,9705454
x1,192:8286934,9705454
x1,192:8823280,9705454
g1,192:9019888,9705454
x1,192:9762280,9705454
x1,192:11752739,9705454
g1,192:11949347,9705454
x1,192:13958681,9705454
g1,192:14155289,9705454
x1,192:14941721,9705454
g1,192:15138329,9705454
x1,192:15618839,9705454
x1,192:19741316,9705454
g1,192:19937924,9705454
x1,192:22755710,9705454
g1,192:22952318,9705454
x1,192:25223534,9705454
g1,192:25420142,9705454
x1,192:27189614,9705454
g1,192:27386222,9705454
x1,192:30574418,9705454
g1,192:30574418,9705454
k1,192:33094932,9705454:2520514
)
(1,192:2424084,11324195:30670848,935849,401084
k1,192:5482553,11324195:3058469
h1,192:5482553,11324195:0,0,0
r1,192:5482553,11324195:0,786432,235932
x1,192:8019385,11324195
g1,192:8297913,11324195
x1,192:10493828,11324195
g1,192:10772356,11324195
x1,192:12133801,11324195
g1,192:12412329,11324195
x1,192:14145887,11324195
g1,192:14424415,11324195
x1,192:15352470,11324195
g1,192:15630998,11324195
x1,192:17673165,11324195
g1,192:17951693,11324195
x1,192:20426136,11324195
x1,192:20660099,11324195
g1,192:20938627,11324195
x1,192:25456351,11324195
g1,192:25734879,11324195
x1,192:27468436,11324195
g1,192:27746964,11324195
x1,192:30036464,11324195
r1,192:30036464,11324195:0,1336933,401084
g1,192:30036464,11324195
k1,192:33094932,11324195:3058468
)
(1,192:2424084,12952749:30670848,716289,120127
k1,192:9542812,12952749:7118728
h1,192:9542812,12952749:0,0,0
x1,192:11105320,12952749
g1,192:11318312,12952749
x1,192:13731937,12952749
$1,192:13731937,12952749
(1,192:13731937,12643485:297558,271350,6261
x1,192:13996727,12643485
)
$1,192:14029495,12952749
x1,192:14242487,12952749
g1,192:14455479,12952749
x1,192:16963673,12952749
g1,192:17176665,12952749
x1,192:19590290,12952749
$1,192:19590290,12952749
(1,192:19590290,12643485:330955,407025,6261
x1,192:19888477,12643485
)
$1,192:19921245,12952749
x1,192:20134237,12952749
g1,192:20347229,12952749
x1,192:22240301,12952749
g1,192:22453293,12952749
x1,192:24866918,12952749
$1,192:24866918,12952749
(1,192:24866918,12643485:1109287,407025,84088
x1,192:25728081,12643485
$1,192:25728081,12643485
x1,192:26008973,12643485
$1,192:26008973,12643485
g1,192:25943437,12643485
)
$1,192:25976205,12952749
g1,192:25976205,12952749
k1,192:33094932,12952749:7118727
)
(1,192:2424084,14001325:30670848,363724,107741
k1,192:12086057,14001325:9661973
h1,192:12086057,14001325:0,0,0
$1,192:12086057,14001325
(1,192:12086057,13811009:229376,173408,4718
x1,192:12282665,13811009
)
$1,192:12315433,14001325
x1,192:12635773,14001325
x1,192:12961880,14001325
x1,192:13306337,14001325
g1,192:13437409,14001325
x1,192:13699553,14001325
x1,192:15591708,14001325
g1,192:15722780,14001325
x1,192:16771356,14001325
x1,192:17523709,14001325
g1,192:17654781,14001325
x1,192:18528769,14001325
g1,192:18659841,14001325
x1,192:19446273,14001325
g1,192:19577345,14001325
x1,192:19897685,14001325
x1,192:21457442,14001325
x1,192:21583271,14001325
g1,192:21714343,14001325
x1,192:23432959,14001325
g1,192:23432959,14001325
k1,192:33094932,14001325:9661973
)
(1,192:2424084,14689453:30670848,459275,107741
k1,192:11824437,14689453:9400353
h1,192:11824437,14689453:0,0,0
$1,192:11824437,14689453
(1,192:11824437,14499137:229376,268959,4718
x1,192:12021045,14499137
)
$1,192:12053813,14689453
x1,192:13567957,14689453
g1,192:13699029,14689453
x1,192:13961173,14689453
x1,192:15853328,14689453
g1,192:15984400,14689453
x1,192:17032976,14689453
x1,192:17785329,14689453
g1,192:17916401,14689453
x1,192:18790389,14689453
g1,192:18921461,14689453
x1,192:19707893,14689453
g1,192:19838965,14689453
x1,192:20159305,14689453
x1,192:21719062,14689453
x1,192:21844891,14689453
g1,192:21975963,14689453
x1,192:23694579,14689453
g1,192:23694579,14689453
k1,192:33094932,14689453:9400353
)
(1,174:2424084,17282678:30670848,394886,7962
x1,174:4618818,17282678
k1,174:33094932,17282678:28476114
g1,174:33094932,17282678
)
(1,177:2424084,18436112:30670848,402554,128286
x1,177:3767112,18436112
g1,176:3914568,18436112
x1,176:4929655,18436112
g1,176:5077111,18436112
x1,176:6158258,18436112
g1,176:6305714,18436112
x1,176:8140066,18436112
g1,176:8287522,18436112
x1,176:8713375,18436112
x1,176:9310866,18436112
k1,177:33094932,18436112:23784066
g1,177:33094932,18436112
)
(1,177:2424084,19930333:30670848,402554,128286
[1,177:2424084,19930333:508428,286578,91422
(1,177:2424084,19930333:508428,286578,0
g1,177:2424084,19930333
(1,177:2424084,19930333:508428,286578,0
k1,177:2547357,19930333:123273
(1,177:2547357,19912124:261882,268369,6193
x1,177:2809239,19912124
)
k1,177:2932512,19930333:123273
)
g1,177:2932512,19930333
)
(1,177:2424084,19930333:508428,391937,91422
g1,177:2424084,19930333
(1,177:2424084,19930333:508428,391937,91422
x1,177:2932512,19930333
)
g1,177:2932512,19930333
)
]
g1,177:3079968,19930333
x1,177:4259616,19930333
g1,177:4407072,19930333
x1,177:5324248,19930333
g1,177:5471704,19930333
x1,177:7519572,19930333
g1,177:7667028,19930333
x1,177:9993883,19930333
g1,177:10141339,19930333
x1,177:10731163,19930333
g1,177:10878619,19930333
x1,177:11894295,19930333
x1,177:12796725,19930333
g1,177:12944181,19930333
x1,177:13910902,19930333
x1,177:13982270,19930333
k1,177:33094932,19930333:19112662
g1,177:33094932,19930333
)
(1,177:2424084,20638122:30670848,402554,128286
x1,177:3472201,20638122
x1,177:3656815,20638122
x1,177:4115108,20638122
x1,177:4821127,20638122
x1,177:5232234,20638122
g1,177:5379690,20638122
x1,177:6722719,20638122
g1,177:6870175,20638122
x1,177:10081765,20638122
g1,177:10229221,20638122
x1,177:10720544,20638122
g1,177:10868000,20638122
x1,177:11588765,20638122
g1,177:11736221,20638122
x1,177:13276251,20638122
x1,177:13866075,20638122
g1,177:14013531,20638122
x1,177:16503768,20638122
g1,177:16651224,20638122
x1,177:17142547,20638122
g1,177:17290003,20638122
x1,177:18010768,20638122
g1,177:18158224,20638122
x1,177:19337872,20638122
g1,177:19485328,20638122
x1,177:20664975,20638122
x1,177:21067235,20638122
g1,177:21214691,20638122
x1,177:21771485,20638122
x1,177:23264329,20638122
g1,177:23411785,20638122
x1,177:24918785,20638122
g1,177:25066241,20638122
x1,177:25656065,20638122
g1,177:25803521,20638122
x1,177:26163903,20638122
x1,177:29255759,20638122
g1,177:29403215,20638122
x1,177:31516554,20638122
x1,177:31664010,20638122
k1,177:33094932,20638122:1430922
g1,177:33094932,20638122
)
(1,181:2424084,21825207:30670848,403439,121208
x1,181:2817496,21825207
x1,179:3058734,21825207
x1,179:4220686,21825207
x1,179:4919626,21825207
g1,179:5067082,21825207
g1,179:5198154,21825207
x1,179:5518494,21825207
k1,180:5198154,21825207:-41943
x1,180:6233623,21825207
g1,180:6364695,21825207
x1,180:7325715,21825207
g1,180:7456787,21825207
x1,180:7718931,21825207
x1,180:7946472,21825207
x1,180:8579287,21825207
x1,180:9476868,21825207
g1,180:9607940,21825207
x1,180:10641312,21825207
g1,180:10772384,21825207
x1,180:12752096,21825207
g1,180:12883168,21825207
x1,180:13407456,21825207
g1,180:13538528,21825207
x1,180:15897824,21825207
g1,180:16028896,21825207
x1,180:16174648,21825207
k1,181:24634790,21825207:8460142
k1,181:33094932,21825207:8460142
)
(1,192:2424084,22103701:30670848,0,0
r1,192:2424084,22103701:0,0,0
g1,192:-7013100,22103701
g1,192:-7013100,22103701
(1,192:-7013100,22103701:0,0,0
(1,192:-7013100,21317269:0,0,0
)
)
g1,192:-6849260,22103701
k1,192:33094932,22103701:39944192
g1,192:33094932,22103701
)
(1,205:2424084,25041557:30670848,449576,8847
(1,205:2424084,25041557:819200,449576,8847
g1,205:2424084,25041557
x1,205:2915604,25041557
g1,205:3243284,25041557
)
x1,205:4736194,25041557
g1,205:4900034,25041557
x1,205:5337159,25041557
x1,205:6113760,25041557
k1,205:33094932,25041557:26981172
g1,205:33094932,25041557
)
(1,209:2424084,26627528:30670848,447283,142540
h1,208:2424084,26627528:786432,0,0
x1,208:4483881,26627528
k1,208:4675663,26627528:191782
x1,208:7150958,26627528
k1,208:7342740,26627528:191782
x1,208:8143590,26627528
k1,208:8335372,26627528:191782
x1,208:9790927,26627528
x1,208:9928552,26627528
k1,208:10120334,26627528:191782
x1,208:11066674,26627528
k1,208:11258456,26627528:191782
x1,208:12096006,26627528
k1,208:12287788,26627528:191782
x1,208:12578768,26627528
k1,208:12770550,26627528:191782
x1,208:16337675,26627528
k1,208:16529457,26627528:191782
x1,208:16929882,26627528
k1,208:17121664,26627528:191782
x1,208:19669049,26627528
x1,208:19790290,26627528
k1,208:19982072,26627528:191782
x1,208:20491942,26627528
k1,208:20683725,26627528:191783
x1,208:20974705,26627528
k1,208:21166487,26627528:191782
x1,208:22149527,26627528
k1,208:22341309,26627528:191782
x1,208:23506539,26627528
k1,208:23698321,26627528:191782
x1,208:24499171,26627528
k1,208:24690953,26627528:191782
x1,208:26037718,26627528
k1,208:26229500,26627528:191782
x1,208:27285285,26627528
k1,208:27477067,26627528:191782
x1,208:28496152,26627528
k1,208:28687934,26627528:191782
x1,208:29233849,26627528
k1,208:29425631,26627528:191782
x1,208:30226481,26627528
k1,208:30418263,26627528:191782
x1,208:31364603,26627528
k1,208:31556385,26627528:191782
x1,208:32102300,26627528
k1,208:32294082,26627528:191782
x1,208:33094932,26627528
k1,208:33094932,26627528:0
)
(1,209:2424084,27413960:30670848,447283,142540
x1,209:3879639,27413960
x1,208:4007434,27413960
k1,208:4224926,27413960:217492
x1,208:5244011,27413960
k1,208:5461503,27413960:217492
x1,208:8336568,27413960
k1,208:8554060,27413960:217492
x1,208:10811120,27413960
k1,208:11028611,27413960:217491
x1,208:12302631,27413960
k1,208:12520123,27413960:217492
x1,208:13647998,27413960
k1,208:13865490,27413960:217492
x1,208:14811830,27413960
k1,208:15029322,27413960:217492
x1,208:15829517,27413960
k1,208:16047009,27413960:217492
x1,208:17212239,27413960
k1,208:17429731,27413960:217492
x1,208:19904371,27413960
k1,208:20121863,27413960:217492
x1,208:20777223,27413960
k1,208:20994715,27413960:217492
x1,208:23488360,27413960
k1,208:23705851,27413960:217491
x1,208:27109791,27413960
k1,208:27327283,27413960:217492
x1,208:29183918,27413960
k1,208:29401410,27413960:217492
x1,208:30347750,27413960
k1,208:30565242,27413960:217492
x1,208:33094932,27413960
k1,208:33094932,27413960:0
)
(1,209:2424084,28200392:30670848,447283,142540
x1,209:3443169,28200392
g1,208:3607009,28200392
x1,208:5463644,28200392
g1,208:5627484,28200392
x1,208:7957289,28200392
g1,208:8121129,28200392
x1,208:8921324,28200392
g1,208:9085164,28200392
x1,208:11377614,28200392
g1,208:11541454,28200392
x1,208:12196814,28200392
g1,208:12360654,28200392
x1,208:14781554,28200392
g1,208:14945394,28200392
x1,208:16110624,28200392
g1,208:16274464,28200392
x1,208:17220804,28200392
g1,208:17384644,28200392
x1,208:18040004,28200392
g1,208:18203844,28200392
x1,208:18877554,28200392
g1,208:19041394,28200392
x1,208:20314759,28200392
g1,208:20478599,28200392
x1,208:21716574,28200392
x1,208:22428295,28200392
g1,208:22592135,28200392
x1,208:24375370,28200392
g1,208:24539210,28200392
x1,208:27597775,28200392
g1,208:27761615,28200392
x1,208:28525765,28200392
g1,208:28689605,28200392
x1,208:30782825,28200392
k1,209:33094932,28200392:2312107
g1,209:33094932,28200392
)
v1,216:2424084,29503603:0,393216,0
(1,216:2424084,33794243:30670848,4683856,681574
g1,216:2424084,33794243
(1,216:2424084,33794243:30670848,4683856,681574
(1,216:2424084,34475817:30670848,5365430,0
[1,216:2424084,34475817:30670848,5365430,0
(1,216:2424084,34449603:30670848,5313002,0
r1,216:2450298,34449603:26214,5313002,0
[1,216:2450298,34449603:30618420,5313002,0
(1,216:2450298,33794243:30618420,4002282,0
[1,216:3105658,33794243:29307700,4002282,0
(1,210:3105658,30492868:29294592,438763,11468
(1,210:3105658,30492868:0,0,0
g1,210:3105658,30492868
)
(1,210:3105658,30492868:0,0,0
(1,210:3105658,30492868:0,0,0
(1,210:3105658,29706436:0,0,0
)
)
g1,210:3105658,30492868
)
x1,210:6782228,30492868
x1,210:7061411,30492868
k1,210:32400251,30492868:25338840
g1,210:32400251,30492868
)
(1,212:3105658,32078839:29294592,447283,6881
(1,212:3105658,32078839:1310720,438435,0
(1,212:3105658,32078839:1310720,438435,0
x1,212:3578828,32078839
g1,212:4234188,32078839
)
)
x1,212:6018078,32078839
g1,212:6181918,32078839
x1,212:6727833,32078839
k1,212:32400249,32078839:25672416
g1,212:32400249,32078839
)
(1,213:3105658,32865271:29294592,447283,142540
(1,213:3105658,32865271:1310720,438435,0
(1,213:3105658,32865271:1310720,438435,0
x1,213:3542783,32865271
g1,213:4198143,32865271
)
)
x1,213:6528603,32865271
g1,213:6692443,32865271
x1,213:7238358,32865271
k1,213:32400250,32865271:25161892
g1,213:32400250,32865271
)
(1,214:3105658,33651703:29294592,447283,142540
(1,214:3105658,33651703:1310720,438435,8846
(1,214:3105658,33651703:1310720,438435,8846
x1,214:3542783,33651703
g1,214:4198143,33651703
)
)
x1,214:6199613,33651703
g1,214:6363453,33651703
x1,214:9930578,33651703
g1,214:10094418,33651703
x1,214:12606413,33651703
g1,214:12770253,33651703
x1,214:13425613,33651703
x1,214:14210079,33651703
g1,214:14373919,33651703
x1,214:15174769,33651703
g1,214:15338609,33651703
x1,214:16575929,33651703
g1,214:16739769,33651703
x1,214:18305424,33651703
g1,214:18469264,33651703
x1,214:19270114,33651703
g1,214:19433954,33651703
x1,214:19907124,33651703
x1,214:20407163,33651703
g1,214:20571003,33651703
x1,214:21554043,33651703
k1,214:32400250,33651703:10846207
g1,214:32400250,33651703
)
]
)
]
r1,216:33094932,34449603:26214,5313002,0
)
]
)
)
g1,216:33094932,33794243
)
h1,216:2424084,34475817:0,0,0
(1,218:2424084,36037417:30670848,438108,10813
(1,218:2424084,36037417:1310720,438108,7863
g1,218:2424084,36037417
x1,218:3407124,36037417
g1,218:3734804,36037417
)
g1,218:3898644,36037417
x1,218:6046914,36037417
x1,218:6313645,36037417
k1,218:33094933,36037417:26781288
g1,218:33094933,36037417
)
(1,220:2424084,37610281:30670848,447283,142540
h1,219:2424084,37610281:786432,0,0
x1,219:4485191,37610281
k1,219:4681185,37610281:195994
x1,219:5955860,37610281
k1,219:6151855,37610281:195995
x1,219:6770515,37610281
k1,219:6966509,37610281:195994
x1,219:7476379,37610281
k1,219:7672373,37610281:195994
x1,219:8764203,37610281
x1,219:9482478,37610281
k1,219:9678440,37610281:195962
x1,219:11425630,37610281
k1,219:11621625,37610281:195995
x1,219:12786855,37610281
k1,219:12982849,37610281:195994
x1,219:13929189,37610281
k1,219:14125183,37610281:195994
x1,219:15873028,37610281
k1,219:16069023,37610281:195995
x1,219:16687683,37610281
k1,219:16883677,37610281:195994
x1,219:19431717,37610281
k1,219:19627711,37610281:195994
x1,219:20391861,37610281
k1,219:20587856,37610281:195995
x1,219:22080111,37610281
k1,219:22276105,37610281:195994
x1,219:24515470,37610281
k1,219:24711464,37610281:195994
x1,219:26131629,37610281
k1,219:26327624,37610281:195995
x1,219:27128474,37610281
k1,219:27324468,37610281:195994
x1,219:28635843,37610281
k1,219:28831805,37610281:195962
x1,219:29923635,37610281
x1,219:30641910,37610281
k1,219:30837872,37610281:195962
x1,219:33094932,37610281
k1,219:33094932,37610281:0
)
(1,220:2424084,38396713:30670848,447283,142540
x1,220:3297679,38396713
x1,219:4907898,38396713
g1,219:5071738,38396713
x1,219:7037818,38396713
g1,219:7201658,38396713
x1,219:8147998,38396713
g1,219:8311838,38396713
x1,219:9840793,38396713
g1,219:10004633,38396713
x1,219:11752478,38396713
g1,219:11916318,38396713
x1,219:12534978,38396713
g1,219:12698818,38396713
x1,219:15392348,38396713
g1,219:15556188,38396713
x1,219:16502528,38396713
g1,219:16666368,38396713
x1,219:17503918,38396713
g1,219:17667758,38396713
x1,219:19888773,38396713
g1,219:20052613,38396713
x1,219:22709443,38396713
x1,219:22830684,38396713
k1,220:33094932,38396713:10264248
g1,220:33094932,38396713
)
(1,222:2424084,39183145:30670848,447283,142540
h1,221:2424084,39183145:786432,0,0
x1,221:4884961,39183145
k1,221:5016164,39183145:131203
x1,221:6144694,39183145
x1,221:6429120,39183145
k1,221:6560323,39183145:131203
x1,221:7652153,39183145
k1,221:7783356,39183145:131203
x1,221:8766396,39183145
k1,221:8897599,39183145:131203
x1,221:9880639,39183145
k1,221:10011842,39183145:131203
x1,221:10885437,39183145
k1,221:11016640,39183145:131203
x1,221:11562555,39183145
k1,221:11693758,39183145:131203
x1,221:13149968,39183145
k1,221:13281171,39183145:131203
x1,221:13827086,39183145
k1,221:13958289,39183145:131203
x1,221:14868584,39183145
x1,221:15305709,39183145
x1,221:16106559,39183145
k1,221:16237762,39183145:131203
x1,221:16893122,39183145
x1,221:18094397,39183145
k1,221:18225600,39183145:131203
x1,221:19536320,39183145
k1,221:19667523,39183145:131203
x1,221:20177393,39183145
k1,221:20308596,39183145:131203
x1,221:21509871,39183145
k1,221:21641074,39183145:131203
x1,221:22587414,39183145
x1,221:22915094,39183145
x1,221:24644589,39183145
k1,221:24775792,39183145:131203
x1,221:25758832,39183145
x1,221:26705172,39183145
k1,221:26836375,39183145:131203
x1,221:28310935,39183145
k1,221:28442138,39183145:131203
x1,221:29643413,39183145
k1,221:29774616,39183145:131203
x1,221:30320531,39183145
k1,221:30451734,39183145:131203
x1,221:31762454,39183145
k1,221:31893657,39183145:131203
x1,221:33094932,39183145
k1,221:33094932,39183145:0
)
(1,222:2424084,39969577:30670848,447283,142540
x1,222:2933954,39969577
k1,221:3098163,39969577:164209
x1,221:3899013,39969577
k1,221:4063221,39969577:164208
x1,221:4427601,39969577
x1,221:4926985,39969577
k1,221:5091194,39969577:164209
x1,221:6219724,39969577
k1,221:6383932,39969577:164208
x1,221:9095157,39969577
k1,221:9259366,39969577:164209
x1,221:10206361,39969577
x1,221:11534776,39969577
k1,221:11698984,39969577:164208
x1,221:12172154,39969577
x1,221:12476896,39969577
x1,221:13768611,39969577
k1,221:13932820,39969577:164209
x1,221:15079045,39969577
k1,221:15243254,39969577:164209
x1,221:16371784,39969577
k1,221:16535992,39969577:164208
x1,221:17991547,39969577
k1,221:18155756,39969577:164209
x1,221:19357031,39969577
x1,221:20595006,39969577
k1,221:20759214,39969577:164208
x1,221:21414574,39969577
x1,221:22470359,39969577
k1,221:22634568,39969577:164209
x1,221:23508163,39969577
x1,221:24599993,39969577
x1,221:25601383,39969577
k1,221:25765591,39969577:164208
x1,221:26166016,39969577
x1,221:26441267,39969577
k1,221:26605476,39969577:164209
x1,221:26896456,39969577
x1,221:27211028,39969577
x1,221:28035470,39969577
k1,221:28199678,39969577:164208
x1,221:28855038,39969577
x1,221:29764678,39969577
x1,221:30310593,39969577
x1,221:31402423,39969577
k1,221:31566632,39969577:164209
x1,221:31857612,39969577
x1,221:33094932,39969577
k1,221:33094932,39969577:0
)
(1,192:2424084,42137179:30670848,435814,196610
h1,192:2424084,42137179:0,0,0
(1,192:2424084,42137179:786432,366083,0
k1,192:2795936,42137179:371852
$1,192:2795936,42137179
(1,192:2795936,41946863:414580,175767,0
$1,192:2795936,41946863
x1,192:2981140,41946863
$1,192:2981140,41946863
g1,192:3177748,41946863
)
$1,192:3210516,42137179
)
g1,192:3341588,42137179
(1,192:3341588,42137179:0,435814,0
r1,192:3341588,42137179:0,435814,0
)
r1,192:3341588,42137179:0,632424,196610
g1,192:3210516,42137179
g1,192:3210516,42137179
x1,192:6326884,42137179
g1,192:6457956,42137179
x1,192:7797512,42137179
x1,192:7899748,42137179
g1,192:8030820,42137179
x1,192:8351160,42137179
x1,192:8969820,42137179
g1,192:9100892,42137179
x1,192:9871071,42137179
x1,192:10832091,42137179
x1,192:11793111,42137179
x1,192:12841687,42137179
g1,192:12972759,42137179
x1,192:13118511,42137179
g1,192:13249583,42137179
x1,192:13424171,42137179
x1,192:14059608,42137179
g1,192:14190680,42137179
x1,192:14960859,42137179
x1,192:15921879,42137179
x1,192:16882899,42137179
x1,192:18062547,42137179
g1,192:18193619,42137179
r1,192:18193619,42137179:0,196610,196610
k1,192:33094932,42137179:14901313
g1,192:33094932,42137179
)
(1,195:2424084,42802371:30670848,435814,7077
h1,195:2424084,42802371:0,0,0
(1,195:2424084,42802371:786432,190316,0
k1,195:2981140,42802371:557056
$1,195:2981140,42802371
(1,195:2981140,42612055:229376,0,0
g1,195:3177748,42612055
)
$1,195:3210516,42802371
)
g1,195:3341588,42802371
(1,195:3341588,42802371:0,435814,0
r1,195:3341588,42802371:0,435814,0
)
r1,195:3341588,42802371:0,442891,7077
g1,195:3210516,42802371
g1,195:3210516,42802371
x1,195:3705444,42802371
x1,195:4637628,42802371
g1,195:4768700,42802371
x1,195:5759080,42802371
x1,195:6554949,42802371
g1,195:6686021,42802371
x1,195:11115730,42802371
k1,195:33094932,42802371:21979202
g1,195:33094932,42802371
)
(1,195:2424084,44244163:30670848,0,196610
h1,195:2424084,44244163:0,0,0
r1,195:2424084,44244163:0,196610,196610
k1,195:33094932,44244163:30670848
g1,195:33094932,44244163
)
]
]
(1,222:2424084,44990034:30670848,0,0
(1,222:2424084,44990034:30670848,0,0
(1,222:2424084,44990034:30670848,0,0
[1,222:2424084,43725189:30670848,0,0
(1,222:2424084,44083015:30670848,357826,114032
h1,222:2424084,44083015:0,0,0
x1,222:3647248,44083015
x1,222:4695824,44083015
g1,222:4826896,44083015
[1,222:4826896,44083015:451936,254737,81264
(1,222:4826896,44083015:451936,254737,0
g1,222:4826896,44083015
(1,222:4826896,44083015:451936,254737,0
k1,222:4936472,44083015:109576
(1,222:4936472,44066829:232784,238551,5505
x1,222:5169256,44066829
)
k1,222:5278832,44083015:109576
)
g1,222:5278832,44083015
)
(1,222:4826896,44083015:451936,348389,81264
g1,222:4826896,44083015
(1,222:4826896,44083015:451936,348389,81264
x1,222:5278832,44083015
)
g1,222:5278832,44083015
)
]
g1,222:5409904,44083015
x1,222:6458480,44083015
g1,222:6589552,44083015
x1,222:7404820,44083015
g1,222:7535892,44083015
x1,222:9356220,44083015
g1,222:9487292,44083015
x1,222:11555608,44083015
g1,222:11686680,44083015
x1,222:12210968,44083015
g1,222:12342040,44083015
x1,222:13244864,44083015
x1,222:14047025,44083015
g1,222:14178097,44083015
x1,222:15037405,44083015
x1,222:15100844,44083015
k1,222:33094932,44083015:17994088
g1,222:33094932,44083015
)
(1,222:2424084,44738375:30670848,357826,114032
x1,222:3355744,44738375
x1,222:3519846,44738375
x1,222:3927218,44738375
x1,222:4554791,44738375
x1,222:4920220,44738375
g1,222:5051292,44738375
x1,222:6245096,44738375
g1,222:6376168,44738375
x1,222:9230916,44738375
g1,222:9361988,44738375
x1,222:9798720,44738375
g1,222:9929792,44738375
x1,222:10570472,44738375
g1,222:10701544,44738375
x1,222:12070460,44738375
x1,222:12594748,44738375
g1,222:12725820,44738375
x1,222:14939364,44738375
g1,222:15070436,44738375
x1,222:15507168,44738375
g1,222:15638240,44738375
x1,222:16278920,44738375
g1,222:16409992,44738375
x1,222:17458568,44738375
g1,222:17589640,44738375
x1,222:18638216,44738375
x1,222:18995780,44738375
g1,222:19126852,44738375
x1,222:19621780,44738375
x1,222:20948753,44738375
g1,222:21079825,44738375
x1,222:22419381,44738375
g1,222:22550453,44738375
x1,222:23074741,44738375
g1,222:23205813,44738375
x1,222:23526153,44738375
x1,222:26274471,44738375
g1,222:26405543,44738375
x1,222:28415139,44738375
k1,222:33094932,44738375:4679793
g1,222:33094932,44738375
)
(1,222:2424084,45393735:30670848,0,0
h1,222:2424084,45393735:0,0,0
k1,222:33094932,45393735:30670848
g1,222:33094932,45393735
)
]
)
)
)
]
]
]
!27043
}1
!10
{2
[1,272:4736287,44691685:28641483,39955398,0
[1,272:4736287,4736287:0,0,0
(1,272:4736287,2656652:0,0,0
k1,272:4736287,2656652:2095146
)
]
[1,272:4736287,44691685:28641483,39955398,0
[1,272:2706922,44691685:30670848,41969252,0
[1,272:2706922,3377793:30670848,655360,0
(1,272:2706922,3377793:30670848,358613,107741
(1,272:2706922,3377793:30670848,358613,107741
x1,272:2969066,3377793
k1,272:10951876,3377793:7982810
x1,272:11272216,3377793
x1,272:12397862,3377793
g1,272:12528934,3377793
x1,272:13664542,3377793
g1,272:13795614,3377793
x1,272:13890510,3377793
g1,272:14021582,3377793
x1,272:14313086,3377793
x1,272:14488198,3377793
x1,272:17160493,3377793
g1,272:17291565,3377793
x1,272:18747513,3377793
x1,272:18960898,3377793
x1,272:19215177,3377793
g1,272:19346249,3377793
x1,272:19870537,3377793
x1,272:21244696,3377793
g1,272:21375768,3377793
x1,272:21900056,3377793
g1,272:22031128,3377793
x1,272:23428880,3377793
g1,272:23559952,3377793
x1,272:24346384,3377793
x1,272:25394960,3377793
k1,272:33377770,3377793:7982810
)
)
]
[1,272:2706922,44691685:30670848,40658532,0
(1,222:2706922,4688513:30670848,447283,142540
x1,222:3689962,4688513
k1,221:3844512,4688513:154550
x1,221:4644707,4688513
k1,221:4799257,4688513:154550
x1,221:6947527,4688513
k1,221:7102076,4688513:154549
x1,221:7720736,4688513
x1,221:9104201,4688513
k1,221:9258751,4688513:154550
x1,221:9768621,4688513
k1,221:9923171,4688513:154550
x1,221:10796766,4688513
k1,221:10951316,4688513:154550
x1,221:11752166,4688513
k1,221:11906715,4688513:154549
x1,221:14891225,4688513
x1,221:15612121,4688513
k1,221:15766671,4688513:154550
x1,221:16931246,4688513
x1,221:17950986,4688513
k1,221:18105536,4688513:154550
x1,221:18651451,4688513
k1,221:18806001,4688513:154550
x1,221:19206426,4688513
x1,221:19924701,4688513
k1,221:20079241,4688513:154540
x1,221:20807346,4688513
x1,221:20989536,4688513
x1,221:21717641,4688513
x1,221:21845436,4688513
k1,221:21999986,4688513:154550
x1,221:22364366,4688513
x1,221:22864405,4688513
x1,221:23374275,4688513
x1,221:23831061,4688513
k1,221:23985611,4688513:154550
x1,221:24932606,4688513
k1,221:25087156,4688513:154550
x1,221:25414836,4688513
x1,221:26469966,4688513
k1,221:26624515,4688513:154549
x1,221:28044025,4688513
k1,221:28198575,4688513:154550
x1,221:29036125,4688513
x1,221:29873675,4688513
k1,221:30028225,4688513:154550
x1,221:33377770,4688513
k1,221:33377770,4688513:0
)
(1,222:2706922,5474945:30670848,447283,142540
x1,222:3107347,5474945
x1,222:3266599,5474945
x1,222:4085799,5474945
k1,221:4251878,5474945:166079
x1,221:5052728,5474945
x1,221:6527288,5474945
k1,221:6693368,5474945:166080
x1,221:7166538,5474945
x1,221:7890710,5474945
x1,221:8072900,5474945
x1,221:8363880,5474945
x1,221:9802395,5474945
k1,221:9968474,5474945:166079
x1,221:10769324,5474945
x1,221:12352674,5474945
k1,221:12518753,5474945:166079
x1,221:12991923,5474945
x1,221:13266519,5474945
x1,221:13584368,5474945
x1,221:14057538,5474945
x1,221:15343354,5474945
k1,221:15509433,5474945:166079
x1,221:16892898,5474945
k1,221:17058978,5474945:166080
x1,221:17532148,5474945
x1,221:18032187,5474945
k1,221:18198266,5474945:166079
x1,221:18926371,5474945
x1,221:20054901,5474945
x1,221:20892451,5474945
k1,221:21058530,5474945:166079
x1,221:21750590,5474945
x1,221:22842420,5474945
k1,221:23008499,5474945:166079
x1,221:23954839,5474945
k1,221:24120919,5474945:166080
x1,221:24594089,5474945
x1,221:26031949,5474945
k1,221:26198028,5474945:166079
x1,221:26962178,5474945
x1,221:27945218,5474945
x1,221:28584194,5474945
x1,221:29821514,5474945
x1,221:31551009,5474945
k1,221:31717088,5474945:166079
x1,221:32663428,5474945
x1,221:32954408,5474945
x1,221:33172643,5474945
x1,221:33377770,5474945
k1,222:33377770,5474945:0
)
(1,222:2706922,6261377:30670848,447283,142540
x1,222:4326317,6261377
k1,221:4487294,6261377:160977
x1,221:5288144,6261377
x1,221:7235874,6261377
k1,221:7396851,6261377:160977
x1,221:8343846,6261377
x1,221:9290186,6261377
k1,221:9451163,6261377:160977
x1,221:10033123,6261377
x1,221:11016163,6261377
x1,221:11655139,6261377
x1,221:12892459,6261377
x1,221:14458114,6261377
k1,221:14619091,6261377:160977
x1,221:15128961,6261377
k1,221:15289938,6261377:160977
x1,221:15580918,6261377
k1,221:15741895,6261377:160977
x1,221:16615490,6261377
x1,221:16906470,6261377
x1,221:17888855,6261377
k1,221:18049832,6261377:160977
x1,221:18886727,6261377
x1,221:19906467,6261377
k1,221:20067444,6261377:160977
x1,221:20540614,6261377
k1,221:20701591,6261377:160977
x1,221:21502441,6261377
k1,221:21663417,6261377:160976
x1,221:22609757,6261377
k1,221:22770734,6261377:160977
x1,221:23316649,6261377
k1,221:23477626,6261377:160977
x1,221:24278476,6261377
k1,221:24439453,6261377:160977
x1,221:24730433,6261377
x1,221:25313048,6261377
x1,221:26077198,6261377
k1,221:26238175,6261377:160977
x1,221:27184515,6261377
k1,221:27345492,6261377:160977
x1,221:28000852,6261377
k1,221:28161829,6261377:160977
x1,221:28999379,6261377
k1,221:29160356,6261377:160977
x1,221:29670226,6261377
x1,221:31089736,6261377
k1,221:31250713,6261377:160977
x1,221:32561433,6261377
k1,221:32722410,6261377:160977
x1,221:33377770,6261377
k1,221:33377770,6261377:0
)
(1,222:2706922,7047809:30670848,447283,142540
x1,222:3507772,7047809
g1,221:3671612,7047809
x1,221:4035992,7047809
x1,221:4691352,7047809
g1,221:4855192,7047809
x1,221:6256352,7047809
g1,221:6420192,7047809
x1,221:6966107,7047809
g1,221:7129947,7047809
x1,221:7420927,7047809
g1,221:7584767,7047809
x1,221:8640552,7047809
x1,221:9769082,7047809
g1,221:9932922,7047809
x1,221:10442792,7047809
g1,221:10606632,7047809
x1,221:11407482,7047809
g1,221:11571322,7047809
x1,221:11935702,7047809
x1,221:12591062,7047809
g1,221:12754902,7047809
x1,221:13300817,7047809
g1,221:13464657,7047809
x1,221:14302207,7047809
x1,221:14593187,7047809
x1,221:16176537,7047809
k1,222:33377769,7047809:17201232
g1,222:33377769,7047809
)
(1,224:2706922,7834241:30670848,447283,142540
h1,223:2706922,7834241:786432,0,0
x1,223:5714369,7834241
g1,223:5878209,7834241
x1,223:6934649,7834241
g1,223:7098489,7834241
x1,223:8227019,7834241
g1,223:8390859,7834241
x1,223:9009519,7834241
g1,223:9173359,7834241
x1,223:11430419,7834241
g1,223:11594259,7834241
x1,223:12540599,7834241
g1,223:12704439,7834241
x1,223:14452284,7834241
g1,223:14616124,7834241
x1,223:15781354,7834241
g1,223:15945194,7834241
x1,223:16637254,7834241
x1,223:16921680,7834241
g1,223:17085520,7834241
x1,223:18214705,7834241
g1,223:18378545,7834241
k1,224:33377770,7834241:14999225
g1,224:33377770,7834241
)
(1,226:4345324,9407105:29032446,447283,142540
(1,225:4345324,9407105:0,292945,0
g1,225:4345324,9407105
g1,225:3034602,9407105
g1,225:2706922,9407105
(1,225:2706922,9407105:1310722,292945,0
k1,225:4017644,9407105:1310722
(1,225:4017644,9407105:0,292945,0
k1,225:3691931,9407105:-325713
x1,225:4017644,9407105
)
)
g1,225:4345324,9407105
)
x1,225:5547254,9407105
g1,225:5711094,9407105
x1,225:7058514,9407105
k1,226:33377770,9407105:26319256
g1,226:33377770,9407105
)
(1,227:4345324,10193537:29032446,447283,142540
(1,226:4345324,10193537:0,292945,0
g1,226:4345324,10193537
g1,226:3034602,10193537
g1,226:2706922,10193537
(1,226:2706922,10193537:1310722,292945,0
k1,226:4017644,10193537:1310722
(1,226:4017644,10193537:0,292945,0
k1,226:3691931,10193537:-325713
x1,226:4017644,10193537
)
)
g1,226:4345324,10193537
)
x1,226:6274704,10193537
g1,226:6438544,10193537
x1,226:7785964,10193537
k1,227:33377770,10193537:25591806
g1,227:33377770,10193537
)
(1,228:4345324,10979969:29032446,447283,6881
(1,227:4345324,10979969:0,292945,0
g1,227:4345324,10979969
g1,227:3034602,10979969
g1,227:2706922,10979969
(1,227:2706922,10979969:1310722,292945,0
k1,227:4017644,10979969:1310722
(1,227:4017644,10979969:0,292945,0
k1,227:3691931,10979969:-325713
x1,227:4017644,10979969
)
)
g1,227:4345324,10979969
)
x1,227:5473854,10979969
g1,227:5637694,10979969
x1,227:6220309,10979969
g1,227:6384149,10979969
x1,227:7039509,10979969
k1,228:33377769,10979969:26338260
g1,228:33377769,10979969
)
(1,231:2706922,12552833:30670848,447283,142540
h1,230:2706922,12552833:786432,0,0
x1,230:5313289,12552833
k1,230:5487582,12552833:174293
x1,230:6470622,12552833
k1,230:6644915,12552833:174293
x1,230:7627955,12552833
k1,230:7802248,12552833:174293
x1,230:9367248,12552833
k1,230:9541541,12552833:174293
x1,230:10051411,12552833
k1,230:10225704,12552833:174293
x1,230:11026554,12552833
k1,230:11200847,12552833:174293
x1,230:12474867,12552833
x1,230:14003822,12552833
x1,230:14476992,12552833
x1,230:15195266,12552833
k1,230:15369559,12552833:174293
x1,230:16771374,12552833
k1,230:16945667,12552833:174293
x1,230:17746517,12552833
k1,230:17920810,12552833:174293
x1,230:19158785,12552833
k1,230:19333078,12552833:174293
x1,230:20316118,12552833
k1,230:20490411,12552833:174293
x1,230:21473451,12552833
k1,230:21647744,12552833:174293
x1,230:22667484,12552833
k1,230:22841777,12552833:174293
x1,230:24662367,12552833
k1,230:24836660,12552833:174293
x1,230:25455320,12552833
k1,230:25629613,12552833:174293
x1,230:27049778,12552833
k1,230:27224071,12552833:174293
x1,230:27988221,12552833
k1,230:28162514,12552833:174293
x1,230:28853919,12552833
x1,230:29460782,12552833
k1,230:29635075,12552833:174293
x1,230:31346220,12552833
k1,230:31520513,12552833:174293
x1,230:32066428,12552833
k1,230:32240721,12552833:174293
x1,230:32713891,12552833
x1,230:33377770,12552833
k1,230:33377770,12552833:0
)
(1,231:2706922,13339265:30670848,447283,142540
x1,231:4126432,13339265
g1,230:4290272,13339265
x1,230:5273312,13339265
g1,230:5437152,13339265
x1,230:6055812,13339265
x1,230:6370384,13339265
x1,230:6651533,13339265
g1,230:6815373,13339265
x1,230:9545603,13339265
g1,230:9709443,13339265
x1,230:10910718,13339265
g1,230:11074558,13339265
x1,230:11402238,13339265
x1,230:13173020,13339265
g1,230:13336860,13339265
x1,230:14302205,13339265
k1,231:33377769,13339265:19075564
g1,231:33377769,13339265
)
(1,233:2706922,14125697:30670848,447283,142540
h1,232:2706922,14125697:786432,0,0
x1,232:5167799,14125697
k1,232:5319222,14125697:151423
x1,232:5974582,14125697
k1,232:6126004,14125697:151422
x1,232:6963554,14125697
k1,232:7114977,14125697:151423
x1,232:8279552,14125697
k1,232:8430975,14125697:151423
x1,232:9231825,14125697
k1,232:9383247,14125697:151422
x1,232:12150177,14125697
k1,232:12301600,14125697:151423
x1,232:13247940,14125697
k1,232:13399362,14125697:151422
x1,232:14637337,14125697
k1,232:14788760,14125697:151423
x1,232:16682095,14125697
k1,232:16833518,14125697:151423
x1,232:18435218,14125697
k1,232:18586640,14125697:151422
x1,232:19205300,14125697
x1,232:19519872,14125697
x1,232:19801021,14125697
k1,232:19952444,14125697:151423
x1,232:21189764,14125697
k1,232:21341187,14125697:151423
x1,232:22069292,14125697
k1,232:22220714,14125697:151422
x1,232:22876074,14125697
k1,232:23027497,14125697:151423
x1,232:23537367,14125697
k1,232:23688789,14125697:151422
x1,232:24635784,14125697
k1,232:24787207,14125697:151423
x1,232:27044267,14125697
k1,232:27195690,14125697:151423
x1,232:29944270,14125697
k1,232:30095692,14125697:151422
x1,232:30823797,14125697
k1,232:30975220,14125697:151423
x1,232:33377770,14125697
k1,232:33377770,14125697:0
)
(1,233:2706922,14912129:30670848,447283,142540
x1,233:3216792,14912129
k1,232:3412999,14912129:196207
x1,232:4213849,14912129
k1,232:4410057,14912129:196208
x1,232:6830957,14912129
k1,232:7027164,14912129:196207
x1,232:8737654,14912129
k1,232:8933862,14912129:196208
x1,232:10681707,14912129
k1,232:10877914,14912129:196207
x1,232:11496574,14912129
k1,232:11692781,14912129:196207
x1,232:13985231,14912129
k1,232:14181439,14912129:196208
x1,232:14691309,14912129
k1,232:14887516,14912129:196207
x1,232:16453171,14912129
k1,232:16649379,14912129:196208
x1,232:18615459,14912129
k1,232:18811666,14912129:196207
x1,232:20558856,14912129
k1,232:20755063,14912129:196207
x1,232:22793888,14912129
k1,232:22990096,14912129:196208
x1,232:23754246,14912129
k1,232:23950453,14912129:196207
x1,232:25442708,14912129
k1,232:25638915,14912129:196207
x1,232:27714440,14912129
k1,232:27910648,14912129:196208
x1,232:29075878,14912129
k1,232:29272085,14912129:196207
x1,232:30727640,14912129
k1,232:30923848,14912129:196208
x1,232:32089078,14912129
k1,232:32285285,14912129:196207
x1,232:33377770,14912129
k1,232:33377770,14912129:0
)
(1,233:2706922,15698561:30670848,447283,142540
x1,233:3726007,15698561
k1,232:3931782,15698561:205775
$1,232:3931782,15698561
x1,232:4914822,15698561
k1,232:5091517,15698561:176695
x1,232:5508325,15698561
k1,232:5685019,15698561:176694
x1,232:6668059,15698561
$1,232:6668059,15698561
k1,232:6873834,15698561:205775
x1,232:8057414,15698561
k1,232:8263189,15698561:205775
x1,232:9064039,15698561
k1,232:9269814,15698561:205775
x1,232:10107364,15698561
k1,232:10313139,15698561:205775
x1,232:12315264,15698561
k1,232:12521039,15698561:205775
x1,232:14013294,15698561
k1,232:14219069,15698561:205775
x1,232:14874429,15698561
k1,232:15080205,15698561:205776
x1,232:15881055,15698561
k1,232:16086830,15698561:205775
x1,232:17524690,15698561
k1,232:17730465,15698561:205775
x1,232:18276380,15698561
k1,232:18482155,15698561:205775
x1,232:19719475,15698561
k1,232:19925250,15698561:205775
x1,232:22182310,15698561
k1,232:22388085,15698561:205775
x1,232:23407825,15698561
k1,232:23613600,15698561:205775
x1,232:24232260,15698561
k1,232:24438035,15698561:205775
x1,232:26003035,15698561
k1,232:26208810,15698561:205775
x1,232:28865640,15698561
k1,232:29071415,15698561:205775
x1,232:29835565,15698561
k1,232:30041340,15698561:205775
x1,232:30842190,15698561
k1,232:31047965,15698561:205775
x1,232:33377770,15698561
k1,232:33377770,15698561:0
)
(1,233:2706922,16484993:30670848,447283,142540
x1,233:3653262,16484993
k1,232:3840367,16484993:187105
x1,232:4641217,16484993
k1,232:4828322,16484993:187105
x1,232:8195562,16484993
k1,232:8382668,16484993:187106
x1,232:9365053,16484993
x1,232:9679625,16484993
x1,232:9960774,16484993
k1,232:10147879,16484993:187105
x1,232:10438859,16484993
k1,232:10625964,16484993:187105
x1,232:11609004,16484993
k1,232:11796109,16484993:187105
x1,232:13069474,16484993
k1,232:13256579,16484993:187105
x1,232:15440239,16484993
k1,232:15627344,16484993:187105
x1,232:18666249,16484993
k1,232:18853355,16484993:187106
x1,232:19690905,16484993
k1,232:19878010,16484993:187105
x1,232:20678860,16484993
k1,232:20865965,16484993:187105
x1,232:23049625,16484993
k1,232:23236730,16484993:187105
x1,232:24474705,16484993
k1,232:24661810,16484993:187105
x1,232:27173805,16484993
k1,232:27360910,16484993:187105
x1,232:28161105,16484993
k1,232:28348211,16484993:187106
x1,232:29221806,16484993
x1,232:30668185,16484993
k1,232:30855290,16484993:187105
x1,232:31365160,16484993
k1,232:31552265,16484993:187105
x1,232:32353115,16484993
k1,232:32540220,16484993:187105
x1,232:33377770,16484993
k1,232:33377770,16484993:0
)
(1,233:2706922,17271425:30670848,447283,142540
x1,233:4089732,17271425
x1,232:4808007,17271425
k1,232:4991184,17271425:183177
x1,232:5391609,17271425
x1,232:7420604,17271425
x1,232:7711584,17271425
k1,232:7894780,17271425:183196
x1,232:9060010,17271425
k1,232:9243206,17271425:183196
x1,232:10044056,17271425
k1,232:10227252,17271425:183196
x1,232:13211762,17271425
k1,232:13394958,17271425:183196
x1,232:14814468,17271425
k1,232:14997664,17271425:183196
x1,232:17382519,17271425
k1,232:17565715,17271425:183196
x1,232:18512055,17271425
k1,232:18695251,17271425:183196
x1,232:20515186,17271425
k1,232:20698382,17271425:183196
x1,232:21189902,17271425
k1,232:21373098,17271425:183196
x1,232:23193688,17271425
x1,232:24576498,17271425
x1,232:24781625,17271425
x1,232:26018945,17271425
k1,232:26202141,17271425:183196
x1,232:26966291,17271425
k1,232:27149487,17271425:183196
x1,232:28350762,17271425
k1,232:28533958,17271425:183196
x1,232:29553698,17271425
k1,232:29736894,17271425:183196
x1,232:31119704,17271425
k1,232:31302900,17271425:183196
x1,232:33377770,17271425
k1,232:33377770,17271425:0
)
(1,233:2706922,18057857:30670848,447283,92405
x1,233:3180092,18057857
x1,232:3843971,18057857
g1,232:4007811,18057857
x1,232:4954151,18057857
x1,232:7210556,18057857
x1,232:7683726,18057857
x1,232:8183765,18057857
g1,232:8347605,18057857
x1,232:9111755,18057857
g1,232:9275595,18057857
x1,232:10076445,18057857
g1,232:10240285,18057857
x1,232:12278455,18057857
g1,232:12442295,18057857
x1,232:12915465,18057857
x1,232:13415504,18057857
g1,232:13579344,18057857
x1,232:14507334,18057857
k1,233:33377770,18057857:18870436
g1,233:33377770,18057857
)
(1,234:2706922,19515932:30670848,448266,7863
(1,234:2706922,19515932:1310720,438108,7863
g1,234:2706922,19515932
x1,234:3689962,19515932
g1,234:4017642,19515932
)
g1,234:4181482,19515932
x1,234:4545862,19515932
x1,234:5869033,19515932
k1,234:33377769,19515932:27508736
g1,234:33377769,19515932
)
(1,237:2706922,21088796:30670848,447283,142540
h1,236:2706922,21088796:786432,0,0
x1,236:4330904,21088796
k1,236:4465484,21088796:134580
x1,236:5994439,21088796
k1,236:6129019,21088796:134580
x1,236:7876864,21088796
k1,236:8011444,21088796:134580
x1,236:8630104,21088796
k1,236:8764684,21088796:134580
x1,236:11385469,21088796
k1,236:11520049,21088796:134580
x1,236:12685279,21088796
k1,236:12819859,21088796:134580
x1,236:14603094,21088796
k1,236:14737674,21088796:134580
x1,236:17304064,21088796
k1,236:17438644,21088796:134580
x1,236:18166749,21088796
x1,236:18993813,21088796
k1,236:19128394,21088796:134581
x1,236:20402414,21088796
k1,236:20536994,21088796:134580
x1,236:22284839,21088796
k1,236:22419419,21088796:134580
x1,236:23038079,21088796
x1,236:23352651,21088796
x1,236:23633800,21088796
k1,236:23768380,21088796:134580
x1,236:24059360,21088796
k1,236:24193940,21088796:134580
x1,236:26287160,21088796
k1,236:26421740,21088796:134580
x1,236:28897035,21088796
k1,236:29031615,21088796:134580
x1,236:30779460,21088796
k1,236:30914040,21088796:134580
x1,236:31532700,21088796
k1,236:31667280,21088796:134580
x1,236:33377770,21088796
k1,236:33377770,21088796:0
)
(1,237:2706922,21875228:30670848,447283,142540
x1,237:3653262,21875228
x1,236:3971111,21875228
x1,236:4252260,21875228
k1,236:4465291,21875228:213031
x1,236:6158086,21875228
k1,236:6371116,21875228:213030
x1,236:7244711,21875228
k1,236:7457742,21875228:213031
x1,236:8586927,21875228
x1,236:9733807,21875228
k1,236:9946837,21875228:213030
x1,236:11257557,21875228
k1,236:11470588,21875228:213031
x1,236:14128073,21875228
k1,236:14341104,21875228:213031
x1,236:15579079,21875228
k1,236:15792109,21875228:213030
x1,236:17539954,21875228
k1,236:17752985,21875228:213031
x1,236:18371645,21875228
k1,236:18584675,21875228:213030
x1,236:19785950,21875228
k1,236:19998981,21875228:213031
x1,236:21674081,21875228
k1,236:21887111,21875228:213030
x1,236:22178091,21875228
k1,236:22391122,21875228:213031
x1,236:23828982,21875228
k1,236:24042013,21875228:213031
x1,236:24551883,21875228
k1,236:24764913,21875228:213030
x1,236:27641943,21875228
k1,236:27854974,21875228:213031
x1,236:28655824,21875228
k1,236:28868854,21875228:213030
x1,236:30834934,21875228
k1,236:31047965,21875228:213031
x1,236:33377770,21875228
k1,236:33377770,21875228:0
)
(1,237:2706922,22661660:30670848,447283,142540
x1,237:3980942,22661660
k1,236:4177943,22661660:197001
x1,236:4978793,22661660
k1,236:5175794,22661660:197001
x1,236:6486514,22661660
k1,236:6683516,22661660:197002
x1,236:7229431,22661660
k1,236:7426432,22661660:197001
x1,236:8227282,22661660
k1,236:8424283,22661660:197001
x1,236:9862143,22661660
k1,236:10059144,22661660:197001
x1,236:11005484,22661660
k1,236:11202485,22661660:197001
x1,236:14479285,22661660
k1,236:14676287,22661660:197002
x1,236:15622627,22661660
x1,236:15940476,22661660
x1,236:16221625,22661660
k1,236:16418626,22661660:197001
x1,236:17364966,22661660
k1,236:17561967,22661660:197001
x1,236:18690497,22661660
x1,236:19147283,22661660
k1,236:19344284,22661660:197001
x1,236:20145134,22661660
k1,236:20342135,22661660:197001
x1,236:21779995,22661660
k1,236:21976997,22661660:197002
x1,236:22377422,22661660
x1,236:23671758,22661660
k1,236:23868759,22661660:197001
x1,236:25143434,22661660
k1,236:25340435,22661660:197001
x1,236:25959095,22661660
k1,236:26156096,22661660:197001
x1,236:28849626,22661660
k1,236:29046627,22661660:197001
x1,236:30066367,22661660
k1,236:30263369,22661660:197002
x1,236:31064219,22661660
k1,236:31261220,22661660:197001
x1,236:31734390,22661660
x1,236:32234429,22661660
k1,236:32431430,22661660:197001
x1,236:33377770,22661660
k1,236:33377770,22661660:0
)
(1,237:2706922,23448092:30670848,447283,142540
x1,237:3544472,23448092
g1,236:3708312,23448092
x1,236:5929327,23448092
g1,236:6093167,23448092
x1,236:8749997,23448092
x1,236:8871238,23448092
g1,236:9035078,23448092
x1,236:10273053,23448092
x1,236:10729839,23448092
g1,236:10893679,23448092
x1,236:11330804,23448092
g1,236:11494644,23448092
x1,236:12113304,23448092
g1,236:12277144,23448092
x1,236:12568124,23448092
x1,236:14487673,23448092
g1,236:14651513,23448092
x1,236:16253213,23448092
g1,236:16417053,23448092
x1,236:17217903,23448092
g1,236:17381743,23448092
x1,236:19311123,23448092
g1,236:19474963,23448092
x1,236:20603493,23448092
g1,236:20767333,23448092
x1,236:21787073,23448092
g1,236:21950913,23448092
x1,236:23716453,23448092
k1,237:33377770,23448092:9661317
g1,237:33377770,23448092
)
[1,249:2706922,29411688:30670848,5111150,0
[1,249:2706922,29411688:30670848,5111150,0
(1,239:2706922,25071241:30670848,357826,114032
(1,239:2706922,25071241:6560416,357826,114032
x1,239:3027262,25071241
x1,239:3858783,25071241
g1,239:3989855,25071241
x1,239:4383071,25071241
g1,239:4514143,25071241
(1,239:4514143,25071241:0,0,0
(1,239:4514143,24415881:0,0,0
)
)
x1,239:5154823,25071241
g1,239:5285895,25071241
x1,239:5518679,25071241
x1,239:7054318,25071241
g1,239:7185390,25071241
x1,239:7622122,25071241
g1,239:7753194,25071241
x1,239:7985978,25071241
g1,239:8117050,25071241
x1,239:9267338,25071241
)
)
(1,249:2706922,27465991:30670848,2215182,1945697
h1,240:2706922,27465991:0,0,0
(1,248:2706922,27465991:30670848,2215182,1945697
$1,248:2706922,27465991
[1,248:2706922,27465991:30670848,2215182,1945697
(1,241:2706922,25709559:30670848,458750,196610
g1,241:2706922,25709559
(1,241:2706922,25709559:7359956,458750,196610
r1,241:2706922,25709559:0,655360,196610
k1,241:9673662,25709559:6966740
g1,241:10066878,25709559
)
k1,241:18321529,25709559:8254651
)
(1,241:2706922,25967115:30670848,458750,196610
g1,241:2706922,25967115
(1,241:2706922,25967115:7359956,458750,196610
r1,241:2706922,25967115:0,655360,196610
k1,241:9673662,25967115:6966740
g1,241:10066878,25967115
)
k1,241:18321529,25967115:8254651
)
(1,243:2706922,26199768:30670848,458750,196610
g1,242:2706922,26199768
(1,242:2706922,26199768:7359956,458750,196610
r1,242:2706922,26199768:0,655360,196610
g1,242:2706923,26199768
x1,242:3347603,26199768
g1,242:3478675,26199768
x1,242:3711459,26199768
x1,242:5247098,26199768
g1,242:5378170,26199768
x1,242:5814902,26199768
g1,242:5945974,26199768
x1,242:6178758,26199768
g1,242:6309830,26199768
x1,242:7882694,26199768
g1,242:8013766,26199768
x1,242:9673662,26199768
g1,242:9673662,26199768
g1,242:10066878,26199768
)
k1,242:18321529,26199768:8254651
(1,242:18321529,26199768:3611821,458750,196610
g1,242:18714745,26199768
g1,242:18714746,26199768
x1,242:20404526,26199768
g1,242:20535598,26199768
x1,242:20914134,26199768
g1,242:21045206,26199768
x1,242:21540134,26199768
g1,242:21540134,26199768
g1,242:21933350,26199768
)
k1,242:30188001,26199768:8254651
(1,243:30188001,26199768:3189769,458750,196610
g1,242:30581217,26199768
g1,242:30581218,26199768
x1,242:32270998,26199768
g1,242:32402070,26199768
x1,242:32751770,26199768
g1,242:32882842,26199768
x1,242:33377770,26199768
g1,243:33377770,26199768
)
g1,243:33377770,26199768
)
(1,243:2706922,26855128:30670848,458750,196610
g1,243:2706922,26855128
(1,243:2706922,26855128:7359956,458750,196610
r1,243:2706922,26855128:0,655360,196610
k1,243:9673662,26855128:6966740
g1,243:10066878,26855128
)
k1,243:18321529,26855128:8254651
)
(1,243:2706922,27112684:30670848,458750,196610
g1,243:2706922,27112684
(1,243:2706922,27112684:7359956,458750,196610
r1,243:2706922,27112684:0,655360,196610
k1,243:9673662,27112684:6966740
g1,243:10066878,27112684
)
k1,243:18321529,27112684:8254651
)
(1,245:2706922,27338783:30670848,458750,196610
g1,244:2706922,27338783
(1,244:2706922,27338783:7359956,458750,196610
r1,244:2706922,27338783:0,655360,196610
g1,244:2706923,27338783
x1,244:3609747,27338783
g1,244:3740819,27338783
x1,244:4235747,27338783
g1,244:4366819,27338783
x1,244:5444231,27338783
k1,244:9673662,27338783:4229431
g1,244:10066878,27338783
)
k1,244:18321529,27338783:8254651
(1,244:18321529,27338783:3611821,458750,196610
g1,244:18714745,27338783
g1,244:18714746,27338783
x1,244:18976890,27338783
k1,244:21540134,27338783:2563244
g1,244:21933350,27338783
)
k1,244:30188001,27338783:8254651
(1,245:30188001,27338783:3189769,458750,196610
g1,244:30581217,27338783
g1,244:30581218,27338783
x1,244:30843362,27338783
k1,245:33377770,27338783:2534408
)
g1,245:33377770,27338783
)
(1,246:2706922,27994143:30670848,458750,196610
g1,245:2706922,27994143
(1,245:2706922,27994143:7359956,458750,196610
r1,245:2706922,27994143:0,655360,196610
g1,245:2706923,27994143
x1,245:3609747,27994143
g1,245:3740819,27994143
x1,245:5313159,27994143
g1,245:5444231,27994143
x1,245:6521643,27994143
k1,245:9673662,27994143:3152019
g1,245:10066878,27994143
)
k1,245:18321529,27994143:8254651
(1,245:18321529,27994143:3611821,458750,196610
g1,245:18714745,27994143
g1,245:18714746,27994143
x1,245:18976890,27994143
k1,245:21540134,27994143:2563244
g1,245:21933350,27994143
)
k1,245:30188001,27994143:8254651
(1,246:30188001,27994143:3189769,458750,196610
g1,245:30581217,27994143
g1,245:30581218,27994143
x1,245:30843362,27994143
k1,246:33377770,27994143:2534408
)
g1,246:33377770,27994143
)
(1,247:2706922,28649503:30670848,458750,196610
g1,246:2706922,28649503
(1,246:2706922,28649503:7359956,458750,196610
r1,246:2706922,28649503:0,655360,196610
g1,246:2706923,28649503
x1,246:3609747,28649503
g1,246:3740819,28649503
x1,246:5313159,28649503
g1,246:5444231,28649503
x1,246:6521643,28649503
k1,246:9673662,28649503:3152019
g1,246:10066878,28649503
)
k1,246:18321529,28649503:8254651
(1,246:18321529,28649503:3611821,458750,196610
g1,246:18714745,28649503
g1,246:18714746,28649503
x1,246:18976890,28649503
k1,246:21540134,28649503:2563244
g1,246:21933350,28649503
)
k1,246:30188001,28649503:8254651
(1,247:30188001,28649503:3189769,458750,196610
g1,246:30581217,28649503
g1,246:30581218,28649503
x1,246:30843362,28649503
k1,247:33377770,28649503:2534408
)
g1,247:33377770,28649503
)
(1,247:2706922,29304863:30670848,458750,196610
g1,247:2706922,29304863
(1,247:2706922,29304863:7359956,458750,196610
r1,247:2706922,29304863:0,655360,196610
k1,247:9673662,29304863:6966740
g1,247:10066878,29304863
)
k1,247:18321529,29304863:8254651
)
(1,247:2706922,29555865:30670848,458750,196610
g1,247:2706922,29555865
(1,247:2706922,29555865:7359956,458750,196610
r1,247:2706922,29555865:0,655360,196610
k1,247:9673662,29555865:6966740
g1,247:10066878,29555865
)
k1,247:18321529,29555865:8254651
)
]
$1,248:33377770,27465991
)
g1,249:33377770,27465991
g1,249:33377770,27465991
)
]
]
(1,253:2706922,31437130:30670848,448266,134676
(1,253:2706922,31437130:1310720,438108,7863
g1,253:2706922,31437130
x1,253:3689962,31437130
g1,253:4017642,31437130
)
g1,253:4181482,31437130
x1,253:7604427,31437130
g1,253:7768267,31437130
x1,253:8278137,31437130
g1,253:8441977,31437130
x1,253:8696912,31437130
x1,253:9691748,31437130
x1,253:11123054,31437130
k1,253:33377770,31437130:22254716
g1,253:33377770,31437130
)
(1,256:2706922,33009994:30670848,447283,142540
h1,255:2706922,33009994:786432,0,0
x1,255:6404464,33009994
k1,255:6649132,33009994:244668
x1,255:7923807,33009994
k1,255:8168474,33009994:244667
x1,255:8787134,33009994
k1,255:9031802,33009994:244668
x1,255:10451967,33009994
k1,255:10696635,33009994:244668
x1,255:11169805,33009994
k1,255:11414472,33009994:244667
x1,255:12215322,33009994
k1,255:12459990,33009994:244668
x1,255:13406330,33009994
k1,255:13650998,33009994:244668
x1,255:14196913,33009994
k1,255:14441580,33009994:244667
x1,255:15242430,33009994
k1,255:15487098,33009994:244668
x1,255:16942653,33009994
x1,255:17070448,33009994
k1,255:17315116,33009994:244668
x1,255:18115966,33009994
k1,255:18360633,33009994:244667
x1,255:19198183,33009994
k1,255:19442851,33009994:244668
x1,255:20061511,33009994
x1,255:20889230,33009994
k1,255:21133898,33009994:244668
x1,255:22444618,33009994
k1,255:22689285,33009994:244667
x1,255:23344645,33009994
k1,255:23589313,33009994:244668
x1,255:23880293,33009994
k1,255:24124961,33009994:244668
x1,255:24743621,33009994
x1,255:25200407,33009994
k1,255:25445074,33009994:244667
x1,255:26682394,33009994
k1,255:26927062,33009994:244668
x1,255:28565462,33009994
k1,255:28810130,33009994:244668
x1,255:29757125,33009994
k1,255:30001792,33009994:244667
x1,255:30438917,33009994
k1,255:30683585,33009994:244668
x1,255:33377770,33009994
k1,255:33377770,33009994:0
)
(1,256:2706922,33796426:30670848,447283,142540
x1,256:5254307,33796426
x1,255:5375548,33796426
k1,255:5618432,33796426:242884
x1,255:7730002,33796426
k1,255:7972885,33796426:242883
x1,255:9720730,33796426
k1,255:9963614,33796426:242884
x1,255:11674104,33796426
k1,255:11916987,33796426:242883
x1,255:12900027,33796426
k1,255:13142911,33796426:242884
x1,255:13433891,33796426
x1,255:13745187,33796426
x1,255:14572251,33796426
k1,255:14815134,33796426:242883
x1,255:17252419,33796426
k1,255:17495303,33796426:242884
x1,255:18005173,33796426
k1,255:18248056,33796426:242883
x1,255:19048906,33796426
k1,255:19291790,33796426:242884
x1,255:19764960,33796426
x1,255:20264999,33796426
k1,255:20507883,33796426:242884
x1,255:22509353,33796426
k1,255:22752236,33796426:242883
x1,255:23262106,33796426
k1,255:23504990,33796426:242884
x1,255:24305840,33796426
k1,255:24548723,33796426:242883
x1,255:25350228,33796426
k1,255:25593112,33796426:242884
x1,255:26139027,33796426
k1,255:26381910,33796426:242883
x1,255:29074130,33796426
k1,255:29317014,33796426:242884
x1,255:30263354,33796426
k1,255:30506237,33796426:242883
x1,255:31598067,33796426
k1,255:31840951,33796426:242884
x1,255:32168631,33796426
x1,255:33377770,33796426
k1,255:33377770,33796426:0
)
(1,256:2706922,34582858:30670848,447283,142540
x1,256:4817837,34582858
g1,255:4981677,34582858
x1,255:7673897,34582858
g1,255:7837737,34582858
x1,255:8493097,34582858
g1,255:8656937,34582858
x1,255:10113147,34582858
g1,255:10276987,34582858
x1,255:10750157,34582858
g1,255:10913997,34582858
x1,255:11551007,34582858
g1,255:11714847,34582858
x1,255:11933082,34582858
x1,255:13243802,34582858
x1,255:13462037,34582858
g1,255:13625877,34582858
x1,255:14171792,34582858
g1,255:14335632,34582858
x1,255:15572952,34582858
g1,255:15736792,34582858
x1,255:16683132,34582858
g1,255:16846972,34582858
x1,255:17866057,34582858
x1,255:18183906,34582858
x1,255:18465055,34582858
g1,255:18628895,34582858
x1,255:18847130,34582858
x1,255:20157850,34582858
x1,255:20376085,34582858
g1,255:20539925,34582858
x1,255:21085840,34582858
g1,255:21249680,34582858
x1,255:21614060,34582858
x1,255:23860634,34582858
g1,255:24024474,34582858
x1,255:24242709,34582858
x1,255:25553429,34582858
x1,255:25771664,34582858
g1,255:25935504,34582858
x1,255:26445374,34582858
g1,255:26609214,34582858
x1,255:27410064,34582858
g1,255:27573904,34582858
x1,255:28047074,34582858
x1,255:28710953,34582858
k1,256:33377770,34582858:4666817
g1,256:33377770,34582858
)
(1,258:2706922,35369290:30670848,447283,142540
h1,257:2706922,35369290:786432,0,0
x1,257:4986264,35369290
k1,257:5182527,35369290:196263
x1,257:5473507,35369290
x1,257:7647991,35369290
k1,257:7844254,35369290:196263
x1,257:8390169,35369290
k1,257:8586432,35369290:196263
x1,257:9241792,35369290
x1,257:9698578,35369290
k1,257:9894841,35369290:196263
x1,257:11096116,35369290
k1,257:11292379,35369290:196263
x1,257:13984599,35369290
k1,257:14180862,35369290:196263
x1,257:15928707,35369290
k1,257:16124970,35369290:196263
x1,257:16743630,35369290
k1,257:16939893,35369290:196263
x1,257:18360058,35369290
k1,257:18556321,35369290:196263
x1,257:19356516,35369290
k1,257:19552778,35369290:196262
x1,257:20062648,35369290
x1,257:20373944,35369290
x1,257:20982773,35369290
k1,257:21179036,35369290:196263
x1,257:21652206,35369290
k1,257:21848469,35369290:196263
x1,257:22649319,35369290
k1,257:22845582,35369290:196263
x1,257:23791922,35369290
k1,257:23988185,35369290:196263
x1,257:24534100,35369290
k1,257:24730363,35369290:196263
x1,257:25677358,35369290
k1,257:25873621,35369290:196263
x1,257:28130681,35369290
k1,257:28326944,35369290:196263
x1,257:28836814,35369290
k1,257:29033077,35369290:196263
x1,257:29833927,35369290
k1,257:30030190,35369290:196263
x1,257:33377770,35369290
k1,257:33377770,35369290:0
)
(1,258:2706922,36155722:30670848,447283,142540
x1,258:4727397,36155722
g1,257:4891237,36155722
x1,257:6492937,36155722
g1,257:6656777,36155722
x1,257:7676517,36155722
g1,257:7840357,36155722
x1,257:8823397,36155722
x1,257:9280183,36155722
g1,257:9444023,36155722
x1,257:10427063,36155722
g1,257:10590903,36155722
x1,257:11100773,36155722
g1,257:11264613,36155722
x1,257:13667163,36155722
g1,257:13831003,36155722
x1,257:15032278,36155722
g1,257:15196118,36155722
x1,257:17633403,36155722
g1,257:17797243,36155722
x1,257:18598748,36155722
g1,257:18762588,36155722
x1,257:21346673,36155722
g1,257:21510513,36155722
x1,257:22020383,36155722
g1,257:22184223,36155722
x1,257:22985073,36155722
g1,257:23148913,36155722
x1,257:24968193,36155722
g1,257:25132033,36155722
x1,257:26879223,36155722
g1,257:27043063,36155722
x1,257:27989403,36155722
g1,257:28153243,36155722
x1,257:29209028,36155722
g1,257:29372868,36155722
x1,257:30555793,36155722
k1,258:33377770,36155722:2821977
g1,258:33377770,36155722
)
(1,260:2706922,36942154:30670848,447283,142540
h1,259:2706922,36942154:786432,0,0
x1,259:6149529,36942154
g1,259:6313369,36942154
x1,259:9079644,36942154
g1,259:9243484,36942154
x1,259:9898844,36942154
g1,259:10062684,36942154
x1,259:11482849,36942154
g1,259:11646689,36942154
x1,259:14668554,36942154
x1,259:14992957,36942154
g1,259:15156797,36942154
x1,259:16394772,36942154
g1,259:16558612,36942154
x1,259:19398287,36942154
g1,259:19562127,36942154
x1,259:20326277,36942154
g1,259:20490117,36942154
x1,259:21581947,36942154
x1,259:22300222,36942154
g1,259:22464062,36942154
x1,259:24721122,36942154
g1,259:24884962,36942154
x1,259:26050192,36942154
x1,259:26171433,36942154
k1,260:33377770,36942154:7206337
g1,260:33377770,36942154
)
(1,263:2706922,37728586:30670848,447283,142540
h1,261:2706922,37728586:786432,0,0
x1,261:4512439,37728586
k1,261:4637176,37728586:124737
x1,261:6311621,37728586
k1,261:6436357,37728586:124736
x1,261:7564887,37728586
k1,261:7689624,37728586:124737
x1,261:8563219,37728586
k1,261:8687956,37728586:124737
x1,261:11563021,37728586
x1,261:12727596,37728586
x1,261:13613642,37728586
x1,261:13904622,37728586
k1,261:14029358,37728586:124736
x1,261:14575273,37728586
k1,261:14700010,37728586:124737
x1,261:15536905,37728586
k1,261:15661642,37728586:124737
x1,261:16462492,37728586
k1,261:16587228,37728586:124736
x1,261:17825203,37728586
k1,261:17949940,37728586:124737
x1,261:20133600,37728586
k1,261:20258337,37728586:124737
x1,261:20768207,37728586
k1,261:20892943,37728586:124736
x1,261:23641523,37728586
k1,261:23766260,37728586:124737
x1,261:24785345,37728586
k1,261:24910082,37728586:124737
x1,261:26766717,37728586
k1,261:26891453,37728586:124736
x1,261:27729003,37728586
k1,261:27853740,37728586:124737
x1,261:28691290,37728586
k1,261:28816027,37728586:124737
x1,261:30272237,37728586
k1,261:30396973,37728586:124736
x1,261:31015633,37728586
k1,261:31140370,37728586:124737
x1,261:33377770,37728586
k1,261:33377770,37728586:0
)
(1,263:2706922,38515018:30670848,447283,142540
x1,263:3143392,38515018
k1,262:3326778,38515018:183386
x1,262:4127628,38515018
k1,262:4311014,38515018:183386
x1,262:5985459,38515018
k1,262:6168846,38515018:183387
x1,262:7297376,38515018
k1,262:7480762,38515018:183386
x1,262:8900927,38515018
k1,262:9084313,38515018:183386
x1,262:11159838,38515018
k1,262:11343224,38515018:183386
x1,262:12107374,38515018
k1,262:12290761,38515018:183387
x1,262:13164356,38515018
x1,262:14829625,38515018
k1,262:15013011,38515018:183386
x1,262:17705231,38515018
k1,262:17888617,38515018:183386
x1,262:19563062,38515018
k1,262:19746448,38515018:183386
x1,262:21021123,38515018
k1,262:21204509,38515018:183386
x1,262:23643759,38515018
k1,262:23827146,38515018:183387
x1,262:24627996,38515018
k1,262:24811382,38515018:183386
x1,262:27833247,38515018
x1,262:28157650,38515018
k1,262:28341036,38515018:183386
x1,262:30197671,38515018
k1,262:30381057,38515018:183386
x1,262:30890927,38515018
k1,262:31074313,38515018:183386
x1,262:31474738,38515018
x1,262:32193013,38515018
k1,262:32376380,38515018:183367
x1,262:33377770,38515018
k1,262:33377770,38515018:0
)
(1,263:2706922,39301450:30670848,447283,142540
x1,263:4127087,39301450
x1,262:4444936,39301450
g1,262:4608776,39301450
x1,262:5628516,39301450
g1,262:5792356,39301450
x1,262:8012061,39301450
g1,262:8175901,39301450
x1,262:8976751,39301450
g1,262:9140591,39301450
x1,262:11577876,39301450
g1,262:11741716,39301450
x1,262:15309496,39301450
x1,262:15430737,39301450
k1,263:33377769,39301450:17947032
g1,263:33377769,39301450
)
(1,265:2706922,40087882:30670848,447283,142540
h1,264:2706922,40087882:786432,0,0
x1,264:3929824,40087882
k1,264:4080295,40087882:150471
x1,264:4881145,40087882
k1,264:5031615,40087882:150470
x1,264:6706060,40087882
k1,264:6856531,40087882:150471
x1,264:7985061,40087882
k1,264:8135531,40087882:150470
x1,264:8973081,40087882
k1,264:9123552,40087882:150471
x1,264:10215382,40087882
k1,264:10365852,40087882:150470
x1,264:10875722,40087882
k1,264:11026193,40087882:150471
x1,264:11827043,40087882
x1,264:12283829,40087882
k1,264:12434299,40087882:150470
x1,264:13235149,40087882
k1,264:13385620,40087882:150471
x1,264:16077840,40087882
k1,264:16228310,40087882:150470
x1,264:16738180,40087882
k1,264:16888651,40087882:150471
x1,264:18563751,40087882
k1,264:18714222,40087882:150471
x1,264:20060987,40087882
k1,264:20211457,40087882:150470
x1,264:21667667,40087882
k1,264:21818138,40087882:150471
x1,264:22436798,40087882
k1,264:22587268,40087882:150470
x1,264:23861288,40087882
k1,264:24011759,40087882:150471
x1,264:24667119,40087882
k1,264:24817589,40087882:150470
x1,264:25763929,40087882
x1,264:26922605,40087882
k1,264:27073076,40087882:150471
x1,264:27873926,40087882
k1,264:28024396,40087882:150470
x1,264:31046261,40087882
x1,264:31370664,40087882
k1,264:31521135,40087882:150471
x1,264:33377770,40087882
k1,264:33377770,40087882:0
)
(1,265:2706922,40874314:30670848,447283,142540
x1,265:3980942,40874314
g1,264:4144782,40874314
x1,264:4435762,40874314
x1,264:7694212,40874314
x1,264:7985192,40874314
g1,264:8149032,40874314
x1,264:8986582,40874314
g1,264:9150422,40874314
x1,264:10096762,40874314
g1,264:10260602,40874314
x1,264:11607367,40874314
g1,264:11771207,40874314
x1,264:12281077,40874314
g1,264:12444917,40874314
x1,264:12845342,40874314
x1,264:13563617,40874314
g1,264:13727457,40874314
x1,264:14728847,40874314
k1,265:33377771,40874314:18648924
g1,265:33377771,40874314
)
(1,268:2706922,42332389:30670848,448266,134676
(1,268:2706922,42332389:1310720,438108,7863
g1,268:2706922,42332389
x1,268:3689962,42332389
g1,268:4017642,42332389
)
x1,268:5947022,42332389
g1,268:6110862,42332389
x1,268:8477367,42332389
k1,268:33377771,42332389:24900404
g1,268:33377771,42332389
)
(1,271:2706922,43905253:30670848,447283,142540
h1,269:2706922,43905253:786432,0,0
x1,269:5459434,43905253
k1,269:5615410,43905253:155976
x1,269:7945215,43905253
k1,269:8101190,43905253:155975
x1,269:9849035,43905253
k1,269:10005011,43905253:155976
x1,269:10623671,43905253
k1,269:10779647,43905253:155976
x1,269:11653242,43905253
k1,269:11809217,43905253:155975
x1,269:12938402,43905253
x1,269:14085282,43905253
k1,269:14241258,43905253:155976
x1,269:15570328,43905253
k1,269:15726304,43905253:155976
x1,269:16891534,43905253
k1,269:17047509,43905253:155975
x1,269:17848359,43905253
k1,269:18004335,43905253:155976
x1,269:19024075,43905253
k1,269:19180051,43905253:155976
x1,269:20526816,43905253
k1,269:20682791,43905253:155975
x1,269:23521811,43905253
k1,269:23677787,43905253:155976
x1,269:24624127,43905253
k1,269:24780103,43905253:155976
x1,269:27400888,43905253
k1,269:27556863,43905253:155975
x1,269:30032158,43905253
x1,269:30343454,43905253
x1,269:31134473,43905253
x1,269:31255714,43905253
k1,269:31411690,43905253:155976
x1,269:33377770,43905253
k1,269:33377770,43905253:0
)
(1,271:2706922,44691685:30670848,447283,142540
x1,271:3872152,44691685
k1,269:4127786,44691685:255634
x1,269:4928636,44691685
k1,269:5184270,44691685:255634
x1,269:8588210,44691685
k1,269:8843844,44691685:255634
x1,269:10081819,44691685
x1,269:11938454,44691685
k1,269:12194088,44691685:255634
x1,269:14523893,44691685
k1,269:14779527,44691685:255634
x1,269:16527372,44691685
k1,269:16783006,44691685:255634
x1,269:17401666,44691685
k1,269:17657300,44691685:255634
x1,269:18167170,44691685
k1,269:18422804,44691685:255634
x1,269:20169994,44691685
k1,269:20425628,44691685:255634
x1,269:21371968,44691685
k1,269:21627602,44691685:255634
x1,269:22137472,44691685
x1,269:23103473,44691685
x1,269:23308600,44691685
x1,269:24436475,44691685
k1,269:24692109,44691685:255634
x1,269:26002829,44691685
k1,269:26258463,44691685:255634
x1,269:28024003,44691685
k1,269:28279637,44691685:255634
x1,269:30900422,44691685
k1,269:31156056,44691685:255634
x1,269:32139096,44691685
k1,269:32394730,44691685:255634
x1,269:33377770,44691685
k1,269:33377770,44691685:0
)
]
(1,272:2706922,44691685:30670848,0,0
h1,272:2706922,44691685:30670848,0,0
)
]
]
]
!41596
}2
!10
{3
[1,316:4736287,44691685:28358645,39955398,0
[1,316:4736287,4736287:0,0,0
(1,316:4736287,2656652:0,0,0
k1,316:4736287,2656652:2377984
)
]
[1,316:4736287,44691685:28358645,39955398,0
[1,316:2424084,44691685:30670848,41969252,0
[1,316:2424084,3377793:30670848,655360,0
(1,316:2424084,3377793:30670848,358613,107741
(1,316:2424084,3377793:30670848,358613,107741
k1,316:10406894,3377793:7982810
x1,316:10727234,3377793
x1,316:11852880,3377793
g1,316:11983952,3377793
x1,316:13119560,3377793
g1,316:13250632,3377793
x1,316:13345528,3377793
g1,316:13476600,3377793
x1,316:13768104,3377793
x1,316:13943216,3377793
x1,316:16615511,3377793
g1,316:16746583,3377793
x1,316:18202531,3377793
x1,316:18415916,3377793
x1,316:18670195,3377793
g1,316:18801267,3377793
x1,316:19325555,3377793
x1,316:20699714,3377793
g1,316:20830786,3377793
x1,316:21355074,3377793
g1,316:21486146,3377793
x1,316:22883898,3377793
g1,316:23014970,3377793
x1,316:23801402,3377793
x1,316:24849978,3377793
k1,316:32832788,3377793:7982810
x1,316:33094932,3377793
)
)
]
[1,316:2424084,44691685:30670848,40658532,0
(1,271:2424084,4688513:30670848,447283,142540
x1,271:3352074,4688513
k1,269:3556437,4688513:204363
x1,269:4502777,4688513
k1,269:4707140,4688513:204363
x1,269:5580735,4688513
k1,269:5785099,4688513:204364
x1,269:6914284,4688513
x1,269:8061164,4688513
k1,269:8265527,4688513:204363
x1,269:9430757,4688513
k1,269:9635120,4688513:204363
x1,269:11455055,4688513
k1,269:11659418,4688513:204363
x1,269:12605758,4688513
k1,269:12810121,4688513:204363
x1,269:15722541,4688513
k1,269:15926904,4688513:204363
x1,269:17164879,4688513
k1,269:17369243,4688513:204364
x1,269:19790143,4688513
k1,269:19994506,4688513:204363
x1,269:20832056,4688513
k1,269:21036419,4688513:204363
x1,269:23366224,4688513
k1,269:23570587,4688513:204363
x1,269:25318432,4688513
k1,269:25522795,4688513:204363
x1,269:26141455,4688513
x1,269:26456027,4688513
x1,269:26737176,4688513
k1,269:26941539,4688513:204363
x1,269:27232519,4688513
k1,269:27436883,4688513:204364
x1,269:29986233,4688513
k1,269:30190596,4688513:204363
x1,269:30736511,4688513
k1,269:30940874,4688513:204363
x1,269:31596234,4688513
x1,269:31917360,4688513
k1,269:32121723,4688513:204363
x1,269:32594893,4688513
x1,269:33094932,4688513
k1,269:33094932,4688513:0
)
(1,271:2424084,5474945:30670848,447283,142540
x1,271:3662059,5474945
g1,269:3825899,5474945
x1,269:5026519,5474945
g1,269:5190359,5474945
x1,269:6501079,5474945
g1,269:6664919,5474945
x1,269:8338709,5474945
g1,269:8502549,5474945
x1,269:8793529,5474945
g1,269:8957369,5474945
x1,269:10194689,5474945
g1,269:10358529,5474945
x1,269:10904444,5474945
g1,269:11068284,5474945
x1,269:13034364,5474945
g1,269:13198204,5474945
x1,269:14817599,5474945
g1,269:14981439,5474945
x1,269:16801374,5474945
g1,270:16965214,5474945
x1,270:17766064,5474945
g1,270:17929904,5474945
x1,270:18403074,5474945
x1,270:18903113,5474945
g1,270:19066953,5474945
x1,270:20158128,5474945
g1,270:20321968,5474945
x1,270:20759093,5474945
g1,270:20922933,5474945
x1,270:21760483,5474945
g1,270:21924323,5474945
x1,270:23380533,5474945
g1,270:23544373,5474945
x1,270:23835353,5474945
x1,270:25245032,5474945
g1,270:25408872,5474945
x1,270:26173022,5474945
g1,270:26336862,5474945
x1,270:27137712,5474945
g1,270:27301552,5474945
x1,270:28211847,5474945
g1,270:28375687,5474945
x1,270:29776847,5474945
k1,271:33094932,5474945:3318085
g1,271:33094932,5474945
)
(1,272:2424084,7459746:30670848,448266,134676
(1,272:2424084,7459746:1310720,438108,7863
g1,272:2424084,7459746
x1,272:3407124,7459746
g1,272:3734804,7459746
)
x1,272:5372549,7459746
x1,272:5872588,7459746
g1,272:6036428,7459746
x1,272:8730613,7459746
g1,272:8894453,7459746
x1,272:9659258,7459746
g1,272:9823098,7459746
x1,272:10623948,7459746
g1,272:10787788,7459746
x1,272:11370403,7459746
x1,272:12547429,7459746
x1,272:13885018,7459746
g1,272:14048858,7459746
x1,272:14558728,7459746
g1,272:14722568,7459746
x1,272:15923843,7459746
g1,272:16087683,7459746
x1,272:16560853,7459746
x1,272:17020915,7459746
k1,272:33094932,7459746:16074017
g1,272:33094932,7459746
)
(1,274:2424084,9032610:30670848,447283,142540
h1,273:2424084,9032610:786432,0,0
x1,273:3683686,9032610
x1,273:3962869,9032610
x1,273:4787311,9032610
k1,273:4981334,9032610:194023
x1,273:5309014,9032610
x1,273:8218157,9032610
k1,273:8412180,9032610:194023
x1,273:8885350,9032610
k1,273:9079373,9032610:194023
x1,273:9880223,9032610
k1,273:10074246,9032610:194023
x1,273:11020586,9032610
k1,273:11214609,9032610:194023
x1,273:11760524,9032610
k1,273:11954547,9032610:194023
x1,273:12245527,9032610
k1,273:12439550,9032610:194023
x1,273:13586430,9032610
k1,273:13780453,9032610:194023
x1,273:16074868,9032610
k1,273:16268891,9032610:194023
x1,273:18562651,9032610
k1,273:18756674,9032610:194023
x1,273:19084354,9032610
x1,273:20639523,9032610
k1,273:20833546,9032610:194023
x1,273:21779886,9032610
k1,273:21973909,9032610:194023
x1,273:24194269,9032610
k1,273:24388292,9032610:194023
x1,273:26136137,9032610
k1,273:26330160,9032610:194023
x1,273:26948820,9032610
k1,273:27142843,9032610:194023
x1,273:29545393,9032610
k1,273:29739416,9032610:194023
x1,273:30249286,9032610
k1,273:30443309,9032610:194023
x1,273:31608539,9032610
k1,273:31802562,9032610:194023
x1,273:33094932,9032610
k1,273:33094932,9032610:0
)
(1,274:2424084,9819042:30670848,447283,142540
x1,274:4061829,9819042
k1,273:4265400,9819042:203571
x1,273:4593080,9819042
x1,273:6359931,9819042
k1,273:6563502,9819042:203571
x1,273:8237947,9819042
k1,273:8441518,9819042:203571
x1,273:10189363,9819042
k1,273:10392935,9819042:203572
x1,273:12759440,9819042
k1,273:12963011,9819042:203571
x1,273:13581671,9819042
k1,273:13785242,9819042:203571
x1,273:14076222,9819042
x1,273:16359496,9819042
k1,273:16563067,9819042:203571
x1,273:17983232,9819042
k1,273:18186803,9819042:203571
x1,273:19916298,9819042
k1,273:20119869,9819042:203571
x1,273:20738529,9819042
x1,273:22251755,9819042
k1,273:22455326,9819042:203571
x1,273:23401666,9819042
k1,273:23605237,9819042:203571
x1,273:26043832,9819042
k1,273:26247404,9819042:203572
x1,273:27995249,9819042
k1,273:28198820,9819042:203571
x1,273:28817480,9819042
k1,273:29021051,9819042:203571
x1,273:29312031,9819042
x1,273:31595305,9819042
k1,273:31798876,9819042:203571
x1,273:32308746,9819042
k1,273:32512317,9819042:203571
x1,273:33094932,9819042
k1,273:33094932,9819042:0
)
(1,274:2424084,10605474:30670848,447283,142540
x1,274:3862599,10605474
g1,273:4026439,10605474
x1,273:4863989,10605474
g1,273:5027829,10605474
x1,273:6229104,10605474
x1,273:8449464,10605474
g1,273:8613304,10605474
x1,273:10068859,10605474
x1,273:12128000,10605474
g1,273:12291840,10605474
x1,273:12837755,10605474
g1,273:13001595,10605474
x1,273:15186565,10605474
g1,273:15350405,10605474
x1,273:16625080,10605474
g1,273:16788920,10605474
x1,273:17407580,10605474
g1,273:17571420,10605474
x1,273:18190080,10605474
x1,273:19500800,10605474
g1,273:19664640,10605474
x1,273:21084150,10605474
g1,273:21247990,10605474
x1,273:22267730,10605474
g1,273:22431570,10605474
x1,273:25362340,10605474
g1,273:25526180,10605474
x1,273:26072095,10605474
g1,273:26235935,10605474
x1,273:26526915,10605474
g1,273:26690755,10605474
x1,273:28875070,10605474
g1,273:29038910,10605474
x1,273:29912505,10605474
x1,273:31522724,10605474
k1,274:33094932,10605474:1572208
g1,274:33094932,10605474
)
(1,275:2424084,12590276:30670848,448266,134676
(1,275:2424084,12590276:1310720,448266,7863
g1,275:2424084,12590276
x1,275:3407124,12590276
g1,275:3734804,12590276
)
x1,275:4135229,12590276
x1,275:4761097,12590276
g1,275:4924937,12590276
x1,275:6891017,12590276
g1,275:7054857,12590276
x1,275:8037897,12590276
g1,275:8201737,12590276
x1,275:10312652,12590276
k1,275:33094932,12590276:22782280
g1,275:33094932,12590276
)
(1,277:2424084,14163140:30670848,447283,142540
h1,276:2424084,14163140:786432,0,0
x1,276:4884961,14163140
k1,276:5148962,14163140:264001
x1,276:5513342,14163140
x1,276:6168702,14163140
k1,276:6432702,14163140:264000
x1,276:7633977,14163140
k1,276:7897978,14163140:264001
x1,276:8990463,14163140
k1,276:9254464,14163140:264001
x1,276:9764334,14163140
k1,276:10028334,14163140:264000
x1,276:10975329,14163140
k1,276:11239330,14163140:264001
x1,276:11567010,14163140
x1,276:12622140,14163140
k1,276:12886141,14163140:264001
x1,276:13977971,14163140
x1,276:14559931,14163140
x1,276:15360781,14163140
k1,276:15624781,14163140:264000
x1,276:17080336,14163140
x1,276:17908055,14163140
[1,276:17947375,14163140:196610,26214,0
]
x1,276:21018395,14163140
k1,276:21282396,14163140:264001
x1,276:22737951,14163140
x1,276:23565670,14163140
[1,276:23604990,14163140:196610,26214,0
]
x1,276:28442860,14163140
k1,276:28706861,14163140:264001
x1,276:29726601,14163140
x1,276:30600851,14163140
k1,276:30864851,14163140:264000
x1,276:32030081,14163140
k1,276:32294082,14163140:264001
x1,276:33094932,14163140
k1,276:33094932,14163140:0
)
(1,277:2424084,14949572:30670848,447283,8846
x1,277:4134574,14949572
g1,276:4298414,14949572
x1,276:5135964,14949572
g1,276:5299804,14949572
x1,276:6246144,14949572
g1,276:6409984,14949572
x1,276:7210834,14949572
g1,276:7374674,14949572
x1,276:8576604,14949572
g1,276:8740444,14949572
x1,276:9250314,14949572
g1,276:9414154,14949572
x1,276:10215004,14949572
g1,276:10378844,14949572
x1,276:11907799,14949572
g1,276:12071639,14949572
x1,276:12799744,14949572
x1,276:12981934,14949572
x1,276:13710039,14949572
x1,276:13837834,14949572
k1,277:33094932,14949572:19257098
g1,277:33094932,14949572
)
(1,280:2424084,15736004:30670848,447283,142540
h1,278:2424084,15736004:786432,0,0
x1,278:4557281,15736004
x1,278:5424322,15736004
g1,278:5588162,15736004
x1,278:8100157,15736004
g1,278:8263997,15736004
x1,278:10011842,15736004
g1,278:10175682,15736004
x1,278:12141762,15736004
g1,278:12305602,15736004
x1,278:13470832,15736004
g1,278:13634672,15736004
x1,278:14435522,15736004
g1,278:14599362,15736004
x1,278:16310507,15736004
g1,278:16474347,15736004
x1,278:19313367,15736004
x1,278:20323932,15736004
x1,278:20778752,15736004
g1,278:20942592,15736004
x1,278:22725827,15736004
g1,278:22889667,15736004
k1,280:33094932,15736004:10205265
g1,280:33094932,15736004
)
(1,281:4062486,17308868:29032446,447283,142540
(1,280:4062486,17308868:0,292945,0
g1,280:4062486,17308868
g1,280:2751764,17308868
g1,280:2424084,17308868
(1,280:2424084,17308868:1310722,292945,0
k1,280:3734806,17308868:1310722
(1,280:3734806,17308868:0,292945,0
k1,280:3409093,17308868:-325713
x1,280:3734806,17308868
)
)
g1,280:4062486,17308868
)
x1,280:4353466,17308868
g1,280:4517306,17308868
x1,280:4934114,17308868
g1,280:5097954,17308868
x1,280:6262529,17308868
x1,280:7129570,17308868
g1,280:7293410,17308868
x1,280:10205830,17308868
g1,280:10369670,17308868
x1,280:11498200,17308868
k1,281:33094932,17308868:21596732
g1,281:33094932,17308868
)
(1,282:4062486,18095300:29032446,447283,142540
(1,281:4062486,18095300:0,292945,0
g1,281:4062486,18095300
g1,281:2751764,18095300
g1,281:2424084,18095300
(1,281:2424084,18095300:1310722,292945,0
k1,281:3734806,18095300:1310722
(1,281:3734806,18095300:0,292945,0
k1,281:3409093,18095300:-325713
x1,281:3734806,18095300
)
)
g1,281:4062486,18095300
)
x1,281:4390166,18095300
g1,281:4554006,18095300
x1,281:4970814,18095300
g1,281:5134654,18095300
x1,281:8047074,18095300
g1,281:8210914,18095300
x1,281:10648199,18095300
g1,281:10812039,18095300
x1,281:12049359,18095300
k1,282:33094931,18095300:21045572
g1,282:33094931,18095300
)
(1,283:4062486,18881732:29032446,447283,6881
(1,282:4062486,18881732:0,292945,0
g1,282:4062486,18881732
g1,282:2751764,18881732
g1,282:2424084,18881732
(1,282:2424084,18881732:1310722,292945,0
k1,282:3734806,18881732:1310722
(1,282:3734806,18881732:0,292945,0
k1,282:3409093,18881732:-325713
x1,282:3734806,18881732
)
)
g1,282:4062486,18881732
)
x1,282:4353466,18881732
g1,282:4517306,18881732
x1,282:4934114,18881732
g1,282:5097954,18881732
x1,282:7318314,18881732
g1,282:7482154,18881732
x1,282:8319704,18881732
g1,282:8483544,18881732
x1,282:8774524,18881732
x1,282:10985708,18881732
k1,283:33094932,18881732:22109224
g1,283:33094932,18881732
)
(1,285:4062486,19668164:29032446,438435,142540
h1,284:4062486,19668164:0,0,0
x1,284:7121051,19668164
g1,284:7284891,19668164
x1,284:8850546,19668164
k1,285:33094932,19668164:24244386
g1,285:33094932,19668164
)
(1,286:4062486,20454596:29032446,447283,142540
(1,285:4062486,20454596:0,292945,0
g1,285:4062486,20454596
g1,285:2751764,20454596
g1,285:2424084,20454596
(1,285:2424084,20454596:1310722,292945,0
k1,285:3734806,20454596:1310722
(1,285:3734806,20454596:0,292945,0
k1,285:3409093,20454596:-325713
x1,285:3734806,20454596
)
)
g1,285:4062486,20454596
)
x1,285:4608401,20454596
g1,285:4772241,20454596
x1,285:5189049,20454596
g1,285:5352889,20454596
x1,285:6881844,20454596
k1,286:33094932,20454596:26213088
g1,286:33094932,20454596
)
(1,287:4062486,21241028:29032446,447283,142540
(1,286:4062486,21241028:0,292945,0
g1,286:4062486,21241028
g1,286:2751764,21241028
g1,286:2424084,21241028
(1,286:2424084,21241028:1310722,292945,0
k1,286:3734806,21241028:1310722
(1,286:3734806,21241028:0,292945,0
k1,286:3409093,21241028:-325713
x1,286:3734806,21241028
)
)
g1,286:4062486,21241028
)
x1,286:4572356,21241028
g1,286:4736196,21241028
x1,286:5153004,21241028
g1,286:5316844,21241028
x1,286:6590864,21241028
k1,287:33094932,21241028:26504068
g1,287:33094932,21241028
)
(1,288:4062486,22027460:29032446,447283,6881
(1,287:4062486,22027460:0,292945,0
g1,287:4062486,22027460
g1,287:2751764,22027460
g1,287:2424084,22027460
(1,287:2424084,22027460:1310722,292945,0
k1,287:3734806,22027460:1310722
(1,287:3734806,22027460:0,292945,0
k1,287:3409093,22027460:-325713
x1,287:3734806,22027460
)
)
g1,287:4062486,22027460
)
x1,287:4608401,22027460
g1,287:4772241,22027460
x1,287:5189049,22027460
g1,287:5352889,22027460
x1,287:7318314,22027460
k1,288:33094932,22027460:25776618
g1,288:33094932,22027460
)
(1,289:4062486,22813892:29032446,447283,142540
(1,288:4062486,22813892:0,292945,0
g1,288:4062486,22813892
g1,288:2751764,22813892
g1,288:2424084,22813892
(1,288:2424084,22813892:1310722,292945,0
k1,288:3734806,22813892:1310722
(1,288:3734806,22813892:0,292945,0
k1,288:3409093,22813892:-325713
x1,288:3734806,22813892
)
)
g1,288:4062486,22813892
)
x1,288:4608401,22813892
g1,288:4772241,22813892
x1,288:5189049,22813892
g1,288:5352889,22813892
x1,288:6044949,22813892
x1,288:6653778,22813892
g1,288:6817618,22813892
x1,288:8783043,22813892
k1,289:33094931,22813892:24311888
g1,289:33094931,22813892
)
(1,292:2424084,24386756:30670848,438108,7863
(1,292:2424084,24386756:1310720,438108,7863
g1,292:2424084,24386756
x1,292:3407124,24386756
g1,292:3734804,24386756
)
x1,292:4135229,24386756
x1,292:6287431,24386756
k1,292:33094931,24386756:26807500
g1,292:33094931,24386756
)
(1,294:2424084,25959620:30670848,447283,142540
h1,293:2424084,25959620:786432,0,0
x1,293:3574896,25959620
x1,293:5786080,25959620
k1,293:5972080,25959620:186000
x1,293:7719925,25959620
k1,293:7905924,25959620:185999
x1,293:8524584,25959620
k1,293:8710584,25959620:186000
x1,293:9001564,25959620
x1,293:9316136,25959620
x1,293:10759238,25959620
k1,293:10945237,25959620:185999
x1,293:11345662,25959620
k1,293:11531662,25959620:186000
x1,293:12441957,25959620
x1,293:12879082,25959620
x1,293:13843772,25959620
k1,293:14029771,25959620:185999
x1,293:15084901,25959620
x1,293:15630816,25959620
x1,293:16722646,25959620
k1,293:16908646,25959620:186000
x1,293:17964431,25959620
x1,293:19347896,25959620
k1,293:19533895,25959620:185999
x1,293:21281740,25959620
k1,293:21467740,25959620:186000
x1,293:22086400,25959620
k1,293:22272399,25959620:185999
x1,293:22891059,25959620
x1,293:24347269,25959620
k1,293:24533269,25959620:186000
x1,293:25043139,25959620
k1,293:25229138,25959620:185999
x1,293:26029988,25959620
k1,293:26215988,25959620:186000
x1,293:26689158,25959620
x1,293:27189197,25959620
k1,293:27375196,25959620:185999
x1,293:28030556,25959620
k1,293:28216556,25959620:186000
x1,293:29162896,25959620
x1,293:29999791,25959620
x1,293:30327471,25959620
x1,293:30691851,25959620
x1,293:31003147,25959620
x1,293:31284296,25959620
k1,293:31470295,25959620:185999
x1,293:32052910,25959620
x1,293:32671570,25959620
x1,293:32889805,25959620
x1,293:33094932,25959620
k1,294:33094932,25959620:0
)
(1,294:2424084,26746052:30670848,544799,142540
x1,294:3880294,26746052
k1,293:4062037,26746052:181743
x1,293:4717397,26746052
x1,293:5663737,26746052
(1,293:5663737,26746052:262144,544799,0
$1,293:5663737,26746052
(1,293:5663737,26508157:262144,306904,0
x1,293:5893113,26508157
)
$1,293:5925881,26746052
)
x1,293:6089721,26746052
k1,293:6271464,26746052:181743
x1,293:7290549,26746052
k1,293:7472292,26746052:181743
x1,293:8528077,26746052
x1,293:9911542,26746052
k1,293:10093286,26746052:181744
x1,293:11841131,26746052
k1,293:12022874,26746052:181743
x1,293:12641534,26746052
k1,293:12823277,26746052:181743
x1,293:14279487,26746052
k1,293:14461230,26746052:181743
x1,293:15226035,26746052
x1,293:16026885,26746052
k1,293:16208628,26746052:181743
x1,293:18155703,26746052
k1,293:18337446,26746052:181743
x1,293:19283786,26746052
k1,293:19465529,26746052:181743
x1,293:19975399,26746052
k1,293:20157143,26746052:181744
x1,293:22086523,26746052
k1,293:22268266,26746052:181743
x1,293:23396796,26746052
k1,293:23578539,26746052:181743
x1,293:24597624,26746052
k1,293:24779367,26746052:181743
x1,293:25325282,26746052
k1,293:25507025,26746052:181743
x1,293:26398970,26746052
k1,293:26580713,26746052:181743
x1,293:27053883,26746052
k1,293:27235626,26746052:181743
x1,293:28036476,26746052
k1,293:28218219,26746052:181743
x1,293:29274004,26746052
k1,293:29455748,26746052:181744
x1,293:30001663,26746052
k1,293:30183406,26746052:181743
x1,293:30984256,26746052
k1,293:31165999,26746052:181743
x1,293:32403319,26746052
k1,293:32585062,26746052:181743
x1,293:33094932,26746052
k1,293:33094932,26746052:0
)
(1,294:2424084,27532484:30670848,447283,142540
x1,294:4025784,27532484
k1,293:4203262,27532484:177478
x1,293:5004112,27532484
x1,293:5321961,27532484
k1,293:5499438,27532484:177477
x1,293:6299633,27532484
k1,293:6477111,27532484:177478
x1,293:7605641,27532484
x1,293:9407881,27532484
k1,293:9585359,27532484:177478
x1,293:10531699,27532484
k1,293:10709176,27532484:177477
x1,293:11582771,27532484
x1,293:11873751,27532484
x1,293:13183816,27532484
k1,293:13361294,27532484:177478
x1,293:14635314,27532484
k1,293:14812792,27532484:177478
x1,293:15613642,27532484
k1,293:15791119,27532484:177477
x1,293:17101839,27532484
k1,293:17279317,27532484:177478
x1,293:17752487,27532484
x1,293:18252526,27532484
k1,293:18430004,27532484:177478
x1,293:19085364,27532484
k1,293:19262841,27532484:177477
x1,293:19553821,27532484
k1,293:19731299,27532484:177478
x1,293:20677639,27532484
k1,293:20855117,27532484:177478
x1,293:21838157,27532484
k1,293:22015634,27532484:177477
x1,293:23471189,27532484
k1,293:23648667,27532484:177478
x1,293:23939647,27532484
x1,293:24257496,27532484
x1,293:25386026,27532484
x1,293:26223576,27532484
k1,293:26401054,27532484:177478
x1,293:26874224,27532484
k1,293:27051701,27532484:177477
x1,293:27852551,27532484
k1,293:28030029,27532484:177478
x1,293:29085814,27532484
k1,293:29263292,27532484:177478
x1,293:29809207,27532484
k1,293:29986684,27532484:177477
x1,293:30787534,27532484
k1,293:30965012,27532484:177478
x1,293:31765862,27532484
x1,293:33094932,27532484
k1,293:33094932,27532484:0
)
(1,294:2424084,28318916:30670848,447283,142540
x1,294:3443169,28318916
g1,293:3607009,28318916
x1,293:4881029,28318916
x1,293:7283579,28318916
g1,293:7447419,28318916
x1,293:8685394,28318916
g1,293:8849234,28318916
x1,293:9286359,28318916
g1,293:9450199,28318916
x1,293:9741179,28318916
x1,293:10055751,28318916
x1,293:10694727,28318916
x1,293:11786557,28318916
g1,293:11950397,28318916
x1,293:12460267,28318916
g1,293:12624107,28318916
x1,293:13424957,28318916
g1,293:13588797,28318916
x1,293:14280202,28318916
x1,293:14998477,28318916
g1,293:15162317,28318916
x1,293:15562742,28318916
x1,293:16317717,28318916
x1,293:17591737,28318916
x1,293:17882717,28318916
g1,293:18046557,28318916
x1,293:18810707,28318916
g1,293:18974547,28318916
x1,293:19775397,28318916
g1,293:19939237,28318916
x1,293:20412407,28318916
x1,293:20912446,28318916
g1,293:21076286,28318916
x1,293:21622201,28318916
g1,293:21786041,28318916
x1,293:22586891,28318916
g1,293:22750731,28318916
x1,293:23806516,28318916
x1,293:25098886,28318916
k1,294:33094932,28318916:7996046
g1,294:33094932,28318916
)
(1,296:2424084,29105348:30670848,447283,142540
h1,295:2424084,29105348:786432,0,0
x1,295:4884961,29105348
g1,295:5048801,29105348
x1,295:5704161,29105348
g1,295:5868001,29105348
x1,295:6705551,29105348
g1,295:6869391,29105348
x1,295:8725371,29105348
g1,295:8889211,29105348
x1,295:9690061,29105348
g1,295:9853901,29105348
x1,295:10872986,29105348
x1,295:11953674,29105348
g1,295:12117514,29105348
x1,295:12663429,29105348
g1,295:12827269,29105348
x1,295:13628119,29105348
g1,295:13791959,29105348
x1,295:16049019,29105348
g1,295:16212859,29105348
x1,295:16758774,29105348
g1,295:16922614,29105348
x1,295:17869609,29105348
g1,295:18033449,29105348
x1,295:18943089,29105348
g1,295:19106929,29105348
x1,295:20563139,29105348
g1,295:20726979,29105348
x1,295:21236849,29105348
g1,295:21400689,29105348
x1,295:22201539,29105348
g1,295:22365379,29105348
x1,295:24549694,29105348
g1,295:24713534,29105348
x1,295:24931769,29105348
x1,295:26418125,29105348
g1,295:26581965,29105348
x1,295:28475300,29105348
g1,295:28639140,29105348
x1,295:30714665,29105348
g1,295:30878505,29105348
x1,295:32497900,29105348
k1,296:33094932,29105348:597032
g1,296:33094932,29105348
)
(1,298:2424084,31483365:30670848,449576,8847
(1,298:2424084,31483365:819200,449576,8847
g1,298:2424084,31483365
x1,298:2915604,31483365
g1,298:3243284,31483365
)
x1,298:6666229,31483365
k1,298:33094933,31483365:26428704
g1,298:33094933,31483365
)
(1,300:2424084,33069336:30670848,447283,142540
h1,299:2424084,33069336:786432,0,0
x1,299:4048066,33069336
k1,299:4347362,33069336:299296
x1,299:5039422,33069336
x1,299:6131252,33069336
k1,299:6430549,33069336:299297
x1,299:8178394,33069336
k1,299:8477690,33069336:299296
x1,299:9096350,33069336
k1,299:9395646,33069336:299296
x1,299:10560876,33069336
x1,299:12016431,33069336
k1,299:12315728,33069336:299297
x1,299:13480958,33069336
k1,299:13780254,33069336:299296
x1,299:14762639,33069336
x1,299:15563489,33069336
k1,299:15862785,33069336:299296
x1,299:16518145,33069336
x1,299:17318995,33069336
x1,299:18265335,33069336
k1,299:18564632,33069336:299297
x1,299:20257427,33069336
$1,299:20257427,33069336
k1,299:20366651,33069336:109224
(1,299:20366651,33069336:709968,66191,8191
x1,299:20530491,33069336
g1,299:20639715,33069336
x1,299:20803555,33069336
g1,299:20912779,33069336
x1,299:21076619,33069336
)
k1,299:21185843,33069336:109224
x1,299:21349683,33069336
$1,299:21349683,33069336
x1,299:21731758,33069336
k1,299:22031054,33069336:299296
x1,299:22431479,33069336
x1,299:22759159,33069336
x1,299:23586223,33069336
k1,299:23885519,33069336:299296
x1,299:24577579,33069336
x1,299:25414474,33069336
k1,299:25713771,33069336:299297
x1,299:27461616,33069336
k1,299:27760912,33069336:299296
x1,299:28379572,33069336
x1,299:28694144,33069336
x1,299:28975293,33069336
k1,299:29274589,33069336:299296
x1,299:29565569,33069336
k1,299:29864866,33069336:299297
x1,299:30774506,33069336
x1,299:31958086,33069336
k1,299:32257382,33069336:299296
x1,299:33094932,33069336
k1,300:33094932,33069336:0
)
(1,300:2424084,33855768:30670848,447283,142540
x1,300:5828024,33855768
k1,299:6172375,33855768:344351
x1,299:8556575,33855768
k1,299:8900925,33855768:344350
x1,299:10648115,33855768
k1,299:10992466,33855768:344351
x1,299:11938806,33855768
k1,299:12283156,33855768:344350
x1,299:12793026,33855768
x1,299:13084006,33855768
x1,299:14685706,33855768
k1,299:15030057,33855768:344351
x1,299:15830252,33855768
k1,299:16174602,33855768:344350
x1,299:16684472,33855768
k1,299:17028823,33855768:344351
x1,299:17647483,33855768
k1,299:17991834,33855768:344351
x1,299:18501049,33855768
x1,299:20065394,33855768
k1,299:20409744,33855768:344350
x1,299:20919614,33855768
k1,299:21263965,33855768:344351
x1,299:21809880,33855768
k1,299:22154230,33855768:344350
x1,299:22846290,33855768
x1,299:24101960,33855768
k1,299:24446311,33855768:344351
x1,299:25647586,33855768
k1,299:25991936,33855768:344350
x1,299:26828831,33855768
x1,299:27292170,33855768
x1,299:28384655,33855768
k1,299:28729006,33855768:344351
x1,299:30476851,33855768
k1,299:30821202,33855768:344351
x1,299:31439862,33855768
k1,299:31784212,33855768:344350
x1,299:33094932,33855768
k1,300:33094932,33855768:0
)
(1,300:2424084,34642200:30670848,447283,142540
x1,300:4244674,34642200
k1,299:4485846,34642200:241172
x1,299:5905356,34642200
k1,299:6146529,34642200:241173
x1,299:6692444,34642200
k1,299:6933616,34642200:241172
x1,299:7952701,34642200
k1,299:8193873,34642200:241172
x1,299:9249003,34642200
x1,299:10777958,34642200
k1,299:11019131,34642200:241173
x1,299:11856681,34642200
x1,299:12858071,34642200
k1,299:13099243,34642200:241172
x1,299:13827348,34642200
x1,299:14502369,34642200
x1,299:16322959,34642200
k1,299:16564131,34642200:241172
x1,299:17983641,34642200
k1,299:18224814,34642200:241173
x1,299:19025009,34642200
k1,299:19266181,34642200:241172
x1,299:20103731,34642200
k1,299:20344903,34642200:241172
x1,299:20926863,34642200
x1,299:22018693,34642200
x1,299:23274363,34642200
k1,299:23515535,34642200:241172
x1,299:24389785,34642200
x1,299:25481615,34642200
k1,299:25722788,34642200:241173
x1,299:26997463,34642200
k1,299:27238635,34642200:241172
x1,299:27857295,34642200
k1,299:28098467,34642200:241172
x1,299:28899317,34642200
x1,299:29845657,34642200
x1,299:30791997,34642200
k1,299:31033170,34642200:241173
x1,299:32052910,34642200
k1,299:32294082,34642200:241172
x1,299:33094932,34642200
k1,299:33094932,34642200:0
)
(1,300:2424084,35428632:30670848,447283,142540
x1,300:2897254,35428632
x1,299:3397293,35428632
k1,299:3554752,35428632:157459
x1,299:4501092,35428632
k1,299:4658551,35428632:157459
x1,299:5496101,35428632
k1,299:5653560,35428632:157459
x1,299:6563855,35428632
x1,299:7874575,35428632
k1,299:8032034,35428632:157459
x1,299:8905629,35428632
x1,299:9196609,35428632
x1,299:10688864,35428632
x1,299:10810105,35428632
k1,299:10967565,35428632:157460
x1,299:11513480,35428632
k1,299:11670939,35428632:157459
x1,299:12617934,35428632
k1,299:12775387,35428632:157453
x1,299:13248557,35428632
x1,299:14115598,35428632
k1,299:14273057,35428632:157459
x1,299:14782927,35428632
x1,299:15620477,35428632
k1,299:15777936,35428632:157459
x1,299:16578786,35428632
k1,299:16736245,35428632:157459
x1,299:17428305,35428632
x1,299:18520135,35428632
k1,299:18677594,35428632:157459
x1,299:19952269,35428632
k1,299:20109728,35428632:157459
x1,299:20728388,35428632
k1,299:20885847,35428632:157459
x1,299:22087122,35428632
x1,299:23106207,35428632
k1,299:23263666,35428632:157459
x1,299:24992506,35428632
k1,299:25149966,35428632:157460
x1,299:26023561,35428632
x1,299:27587906,35428632
k1,299:27745365,35428632:157459
x1,299:28291280,35428632
x1,299:29492555,35428632
k1,299:29650014,35428632:157459
x1,299:30195929,35428632
k1,299:30353388,35428632:157459
x1,299:31045448,35428632
x1,299:32137278,35428632
k1,299:32294737,35428632:157459
x1,299:33094932,35428632
k1,299:33094932,35428632:0
)
(1,300:2424084,36215064:30670848,447283,142540
x1,300:3898644,36215064
k1,299:4061665,36215064:163021
x1,299:5718415,36215064
k1,299:5881436,36215064:163021
x1,299:6937221,36215064
k1,299:7100241,36215064:163020
x1,299:8028231,36215064
k1,299:8191251,36215064:163020
x1,299:9064846,36215064
x1,299:9538016,36215064
x1,299:10593801,36215064
k1,299:10756822,36215064:163021
x1,299:11703162,36215064
k1,299:11866183,36215064:163021
x1,299:12958668,36215064
x1,299:14051153,36215064
k1,299:14214174,36215064:163021
x1,299:15962019,36215064
k1,299:16125040,36215064:163021
x1,299:16743700,36215064
k1,299:16906720,36215064:163020
x1,299:18689955,36215064
k1,299:18852976,36215064:163021
x1,299:19471636,36215064
x1,299:20782356,36215064
k1,299:20945377,36215064:163021
x1,299:21418547,36215064
x1,299:22437632,36215064
k1,299:22600653,36215064:163021
x1,299:23110523,36215064
k1,299:23273543,36215064:163020
x1,299:24074393,36215064
k1,299:24237414,36215064:163021
x1,299:25147054,36215064
x1,299:26166794,36215064
k1,299:26329815,36215064:163021
x1,299:26875730,36215064
k1,299:27038751,36215064:163021
x1,299:27548621,36215064
k1,299:27711642,36215064:163021
x1,299:28002622,36215064
k1,299:28165642,36215064:163020
x1,299:28638812,36215064
x1,299:28956661,36215064
x1,299:29903001,36215064
k1,299:30066022,36215064:163021
x1,299:30611937,36215064
x1,299:30939617,36215064
x1,299:32385996,36215064
k1,299:32549017,36215064:163021
x1,299:33094932,36215064
k1,299:33094932,36215064:0
)
(1,300:2424084,37001496:30670848,447283,142540
x1,300:3443169,37001496
k1,299:3589200,37001496:146031
x1,299:4135115,37001496
k1,299:4281146,37001496:146031
x1,299:5081996,37001496
k1,299:5228028,37001496:146032
x1,299:5920088,37001496
x1,299:6920823,37001496
k1,299:7066854,37001496:146031
x1,299:7941104,37001496
x1,299:9032934,37001496
k1,299:9178965,37001496:146031
x1,299:10926810,37001496
k1,299:11072841,37001496:146031
x1,299:11691501,37001496
k1,299:11837533,37001496:146032
x1,299:13548023,37001496
k1,299:13694054,37001496:146031
x1,299:14167224,37001496
k1,299:14313255,37001496:146031
x1,299:15114105,37001496
k1,299:15260136,37001496:146031
x1,299:16097686,37001496
k1,299:16243717,37001496:146031
x1,299:16789632,37001496
k1,299:16935664,37001496:146032
x1,299:17773214,37001496
x1,299:18792954,37001496
k1,299:18938985,37001496:146031
x1,299:19484900,37001496
k1,299:19630931,37001496:146031
x1,299:19921911,37001496
k1,299:20067942,37001496:146031
x1,299:21305262,37001496
k1,299:21451293,37001496:146031
x1,299:22543123,37001496
x1,299:23052338,37001496
x1,299:23363634,37001496
x1,299:23863018,37001496
k1,299:24009050,37001496:146032
x1,299:24919345,37001496
x1,299:25356470,37001496
x1,299:26321160,37001496
k1,299:26467191,37001496:146031
x1,299:27013106,37001496
k1,299:27159137,37001496:146031
x1,299:28505902,37001496
k1,299:28651933,37001496:146031
x1,299:29197848,37001496
k1,299:29343880,37001496:146032
x1,299:30254175,37001496
x1,299:30691300,37001496
x1,299:31492150,37001496
k1,299:31638181,37001496:146031
x1,299:32148051,37001496
k1,299:32294082,37001496:146031
x1,299:33094932,37001496
k1,299:33094932,37001496:0
)
(1,300:2424084,37787928:30670848,447283,142540
x1,300:3443824,37787928
k1,299:3626233,37787928:182409
x1,299:4353683,37787928
x1,299:4644663,37787928
x1,299:6063518,37787928
k1,299:6245928,37787928:182410
x1,299:6755798,37787928
k1,299:6938207,37787928:182409
x1,299:8248927,37787928
k1,299:8431336,37787928:182409
x1,299:8941206,37787928
k1,299:9123616,37787928:182410
x1,299:9924466,37787928
k1,299:10106875,37787928:182409
x1,299:10725535,37787928
x1,299:11562430,37787928
x1,299:11690225,37787928
k1,299:11872634,37787928:182409
x1,299:13547079,37787928
k1,299:13729489,37787928:182410
x1,299:14348149,37787928
x1,299:15439979,37787928
k1,299:15622388,37787928:182409
x1,299:16605428,37787928
k1,299:16787837,37787928:182409
x1,299:17443197,37787928
k1,299:17625607,37787928:182410
x1,299:18426457,37787928
k1,299:18608866,37787928:182409
x1,299:19300926,37787928
x1,299:20392756,37787928
k1,299:20575165,37787928:182409
x1,299:21375360,37787928
k1,299:21557769,37787928:182409
x1,299:22103684,37787928
k1,299:22286094,37787928:182410
x1,299:23269134,37787928
k1,299:23451543,37787928:182409
x1,299:24507328,37787928
k1,299:24689719,37787928:182391
x1,299:25453869,37787928
x1,299:25781549,37787928
x1,299:26291419,37787928
x1,299:27566094,37787928
k1,299:27748503,37787928:182409
x1,299:28294418,37787928
k1,299:28476827,37787928:182409
x1,299:29423822,37787928
k1,299:29606232,37787928:182410
x1,299:30625972,37787928
k1,299:30808381,37787928:182409
x1,299:31026616,37787928
x1,299:31311042,37787928
x1,299:31966402,37787928
x1,299:32148592,37787928
x1,299:33094932,37787928
k1,299:33094932,37787928:0
)
(1,300:2424084,38574360:30670848,447283,142540
x1,300:3734804,38574360
g1,299:3898644,38574360
x1,299:4736194,38574360
x1,299:5737584,38574360
k1,300:33094932,38574360:27357348
g1,300:33094932,38574360
)
(1,307:2424084,39360792:30670848,447283,142540
h1,301:2424084,39360792:786432,0,0
x1,301:4229601,39360792
k1,301:4466914,39360792:237313
x1,301:5158974,39360792
x1,301:5995869,39360792
k1,301:6233182,39360792:237313
x1,301:7398412,39360792
x1,301:8235307,39360792
k1,301:8472620,39360792:237313
x1,301:9418960,39360792
k1,301:9656273,39360792:237313
x1,301:10565913,39360792
x1,301:11585653,39360792
k1,301:11822966,39360792:237313
x1,301:13570811,39360792
k1,301:13808124,39360792:237313
x1,301:14426784,39360792
k1,301:14664097,39360792:237313
x1,301:16120307,39360792
k1,301:16357620,39360792:237313
x1,301:16976280,39360792
x1,301:17486150,39360792
x1,301:17942936,39360792
k1,301:18180250,39360792:237314
x1,301:18981100,39360792
k1,301:19218413,39360792:237313
x1,301:19582793,39360792
x1,301:20347598,39360792
x1,301:21039003,39360792
x1,301:22058743,39360792
k1,301:22296056,39360792:237313
x1,301:22805926,39360792
k1,301:23043239,39360792:237313
x1,301:23370919,39360792
k1,301:23608232,39360792:237313
x1,301:24118102,39360792
k1,301:24355415,39360792:237313
x1,301:25301755,39360792
k1,301:25539068,39360792:237313
x1,301:26412663,39360792
k1,301:26649976,39360792:237313
x1,301:27414781,39360792
x1,301:27779161,39360792
x1,301:28762201,39360792
k1,301:28999514,39360792:237313
x1,301:30710004,39360792
k1,301:30947317,39360792:237313
x1,301:32111892,39360792
x1,301:33094932,39360792
k1,301:33094932,39360792:0
)
(1,307:2424084,40147224:30670848,447283,142540
x1,307:3333724,40147224
x1,307:4608399,40147224
k1,301:4820967,40147224:212568
x1,301:5366882,40147224
k1,301:5579450,40147224:212568
x1,301:7217850,40147224
k1,301:7430418,40147224:212568
x1,301:8413458,40147224
k1,301:8626026,40147224:212568
x1,301:9754556,40147224
k1,301:9967123,40147224:212567
x1,301:10767973,40147224
x1,301:11933203,40147224
k1,301:12145771,40147224:212568
x1,301:13638681,40147224
k1,301:13851249,40147224:212568
x1,301:14615399,40147224
k1,301:14827967,40147224:212568
x1,301:15738262,40147224
k1,301:15950830,40147224:212568
x1,301:17079360,40147224
x1,301:17807465,40147224
x1,301:18827205,40147224
k1,301:19039773,40147224:212568
x1,301:20532683,40147224
k1,301:20745251,40147224:212568
x1,301:21291166,40147224
k1,301:21503734,40147224:212568
x1,301:22159094,40147224
x1,301:23542559,40147224
k1,301:23755127,40147224:212568
x1,301:24664767,40147224
x1,301:26356907,40147224
k1,301:26569474,40147224:212567
x1,301:26933854,40147224
x1,301:27469938,40147224
k1,301:27682506,40147224:212568
x1,301:29029271,40147224
k1,301:29241839,40147224:212568
x1,301:30698049,40147224
x1,301:31936024,40147224
k1,301:32148592,40147224:212568
x1,301:33094932,40147224
k1,307:33094932,40147224:0
)
(1,307:2424084,40933656:30670848,447283,142540
x1,307:5518694,40933656
k1,301:5874293,40933656:355599
x1,301:6384163,40933656
k1,301:6739761,40933656:355598
x1,301:7868291,40933656
k1,301:8223890,40933656:355599
x1,301:9206930,40933656
k1,301:9562528,40933656:355598
x1,301:10472823,40933656
x1,301:11347073,40933656
k1,301:11702672,40933656:355599
x1,301:12867902,40933656
k1,301:13223500,40933656:355598
x1,301:14352030,40933656
x1,301:15044090,40933656
k1,301:15399689,40933656:355599
x1,301:16091094,40933656
x1,301:16564264,40933656
x1,301:17431305,40933656
k1,301:17786903,40933656:355598
x1,301:19424648,40933656
k1,301:19780247,40933656:355599
x1,301:21091622,40933656
k1,301:21447220,40933656:355598
x1,301:24426486,40933656
x1,301:25566812,40933656
x1,301:26569513,40933656
x1,301:29169326,40933656
x1,301:33094932,40933656
k1,307:33094932,40933656:0
)
(1,307:2424084,41720088:30670848,447283,142540
x1,307:3770849,41720088
x1,301:4637890,41720088
k1,301:4834771,41720088:196881
x1,301:5708366,41720088
k1,301:5905247,41720088:196881
x1,301:6560607,41720088
k1,301:6757489,41720088:196882
x1,301:7230659,41720088
x1,301:7730698,41720088
k1,301:7927579,41720088:196881
x1,301:9383789,41720088
k1,301:9580670,41720088:196881
x1,301:10381520,41720088
k1,301:10578401,41720088:196881
x1,301:11634186,41720088
k1,301:11831067,41720088:196881
x1,301:12376982,41720088
k1,301:12573863,41720088:196881
x1,301:12938243,41720088
k1,301:13135125,41720088:196882
x1,301:13644995,41720088
k1,301:13841876,41720088:196881
x1,301:14642726,41720088
k1,301:14839607,41720088:196881
x1,301:16150327,41720088
k1,301:16347208,41720088:196881
x1,301:17657928,41720088
k1,301:17854809,41720088:196881
x1,301:18400724,41720088
k1,301:18597605,41720088:196881
x1,301:19398455,41720088
k1,301:19595337,41720088:196882
x1,301:20068507,41720088
x1,301:20732386,41720088
k1,301:20929267,41720088:196881
x1,301:21730117,41720088
x1,301:22186903,41720088
x1,301:22477883,41720088
x1,301:22789179,41720088
x1,301:23288563,41720088
x1,301:23426188,41720088
k1,301:23623069,41720088:196881
x1,301:24023494,41720088
k1,301:24220375,41720088:196881
x1,301:24875735,41720088
x1,301:25196861,41720088
k1,301:25393742,41720088:196881
x1,301:26085802,41720088
x1,301:27250377,41720088
k1,301:27447258,41720088:196881
x1,301:27993828,41720088
k1,301:28190710,41720088:196882
x1,301:28809370,41720088
x1,301:29309409,41720088
k1,301:29506290,41720088:196881
x1,301:30016160,41720088
k1,301:30213041,41720088:196881
x1,301:31413661,41720088
k1,301:31610542,41720088:196881
x1,301:32957307,41720088
x1,301:33094932,41720088
k1,301:33094932,41720088:0
)
(1,307:2424084,42506520:30670848,447283,142540
x1,307:3770849,42506520
g1,301:3934689,42506520
x1,301:5063219,42506520
g1,301:5227059,42506520
x1,301:5845719,42506520
g1,301:6009559,42506520
x1,301:7720049,42506520
g1,301:7883889,42506520
x1,301:8502549,42506520
x1,301:9002588,42506520
g1,301:9166428,42506520
x1,301:9676298,42506520
g1,301:9840138,42506520
x1,301:11040758,42506520
g1,301:11204598,42506520
x1,301:12551363,42506520
g1,301:12715203,42506520
x1,301:13225073,42506520
g1,301:13388913,42506520
x1,301:13934828,42506520
x1,301:14249400,42506520
x1,301:14530549,42506520
g1,301:14694389,42506520
x1,301:16313784,42506520
g1,301:16477624,42506520
x1,301:16842004,42506520
x1,301:17378088,42506520
g1,301:17541928,42506520
x1,301:17832908,42506520
x1,301:18150757,42506520
x1,301:18951607,42506520
x1,301:19916297,42506520
g1,301:20080137,42506520
x1,301:20917032,42506520
g1,301:21080872,42506520
x1,301:22118962,42506520
g1,301:22282802,42506520
x1,301:22774322,42506520
g1,301:22938162,42506520
k1,307:33094932,42506520:10156770
g1,307:33094932,42506520
)
(1,293:2424084,44691685:30670848,453377,196610
h1,293:2424084,44691685:0,0,0
(1,293:2424084,44691685:786432,453377,0
k1,293:2784532,44691685:360448
$1,293:2784532,44691685
(1,293:2784532,44501369:425984,263061,0
x1,293:2981140,44501369
g1,293:3177748,44501369
)
$1,293:3210516,44691685
)
g1,293:3341588,44691685
(1,293:3341588,44691685:0,435814,0
r1,293:3341588,44691685:0,435814,0
)
r1,293:3341588,44691685:0,649987,196610
g1,293:3210516,44691685
g1,293:3210516,44691685
(1,293:3210516,44691685:0,0,0
(1,293:3210516,44036325:0,0,0
)
)
x1,293:3502020,44691685
x1,293:5067019,44691685
g1,293:5198091,44691685
x1,293:5576627,44691685
x1,293:6107730,44691685
r1,293:6107730,44691685:0,196610,196610
k1,293:33094932,44691685:26987202
g1,293:33094932,44691685
)
]
(1,316:2424084,44691685:30670848,0,0
h1,316:2424084,44691685:30670848,0,0
)
]
]
]
!39402
}3
!10
{4
[1,372:4736287,44691685:28641483,39955398,0
[1,372:4736287,4736287:0,0,0
(1,372:4736287,2656652:0,0,0
k1,372:4736287,2656652:2095146
)
]
[1,372:4736287,44691685:28641483,39955398,0
[1,372:2706922,44691685:30670848,41969252,0
[1,372:2706922,3377793:30670848,655360,0
(1,372:2706922,3377793:30670848,358613,107741
(1,372:2706922,3377793:30670848,358613,107741
x1,372:2969066,3377793
k1,372:10951876,3377793:7982810
x1,372:11272216,3377793
x1,372:12397862,3377793
g1,372:12528934,3377793
x1,372:13664542,3377793
g1,372:13795614,3377793
x1,372:13890510,3377793
g1,372:14021582,3377793
x1,372:14313086,3377793
x1,372:14488198,3377793
x1,372:17160493,3377793
g1,372:17291565,3377793
x1,372:18747513,3377793
x1,372:18960898,3377793
x1,372:19215177,3377793
g1,372:19346249,3377793
x1,372:19870537,3377793
x1,372:21244696,3377793
g1,372:21375768,3377793
x1,372:21900056,3377793
g1,372:22031128,3377793
x1,372:23428880,3377793
g1,372:23559952,3377793
x1,372:24346384,3377793
x1,372:25394960,3377793
k1,372:33377770,3377793:7982810
)
)
]
[1,372:2706922,44691685:30670848,40658532,0
[1,306:2706922,11965614:30670848,7932461,0
[1,306:2706922,11965614:30670848,7932461,0
(1,304:2706922,10783345:30670848,6488048,0
k1,304:5393929,10783345:2687007
(1,304:5393929,10783345:25296834,6488048,0
(1,304:5393929,10783345:25296896,6488064,0
(1,304:5393929,10783345:25296896,6488064,0
(1,304:5393929,10783345:0,6488064,0
(1,304:5393929,10783345:25296896,6488064,0
)
k1,304:5393929,10783345:-25296896
)
)
)
)
k1,304:33377770,10783345:2687007
)
(1,305:2706922,11851582:30670848,357826,114032
k1,305:13644880,11851582:10937958
(1,305:13644880,11851582:8794932,357826,114032
x1,305:14475352,11851582
g1,305:14606424,11851582
x1,305:14999640,11851582
g1,305:15130712,11851582
(1,305:15130712,11851582:0,0,0
(1,305:15130712,11196222:0,0,0
)
)
x1,305:15712672,11851582
g1,305:15843744,11851582
x1,305:16659536,11851582
g1,305:16790608,11851582
x1,305:18392308,11851582
g1,305:18523380,11851582
x1,305:19134700,11851582
g1,305:19265772,11851582
x1,305:20721720,11851582
g1,305:20852792,11851582
x1,305:22439812,11851582
)
k1,305:33377770,11851582:10937958
)
]
]
(1,309:2706922,13863603:30670848,449576,134348
(1,309:2706922,13863603:819200,449576,8847
g1,309:2706922,13863603
x1,309:3198442,13863603
g1,309:3526122,13863603
)
x1,309:6367107,13863603
k1,309:33377771,13863603:27010664
g1,309:33377771,13863603
)
(1,311:2706922,15449574:30670848,447283,142540
h1,310:2706922,15449574:786432,0,0
x1,310:6114794,15449574
k1,310:6254604,15449574:139810
x1,310:7200944,15449574
k1,310:7340754,15449574:139810
x1,310:7886669,15449574
x1,310:8942454,15449574
x1,310:9706604,15449574
k1,310:9846414,15449574:139810
x1,310:11594259,15449574
k1,310:11734069,15449574:139810
x1,310:12352729,15449574
k1,310:12492539,15449574:139810
x1,310:13948749,15449574
k1,310:14088559,15449574:139810
x1,310:14598429,15449574
k1,310:14738239,15449574:139810
x1,310:16522129,15449574
x1,310:17579880,15449574
k1,310:17719690,15449574:139810
x1,310:18666030,15449574
k1,310:18805840,15449574:139810
x1,310:19971070,15449574
x1,310:21426625,15449574
k1,310:21566435,15449574:139810
x1,310:22512775,15449574
x1,310:23349670,15449574
x1,310:23677350,15449574
x1,310:24041730,15449574
x1,310:24353026,15449574
x1,310:25144045,15449574
k1,310:25283855,15449574:139810
x1,310:26449085,15449574
k1,310:26588895,15449574:139810
x1,310:27571280,15449574
x1,310:28372130,15449574
k1,310:28511940,15449574:139810
x1,310:29167300,15449574
x1,310:29968150,15449574
x1,310:30914490,15449574
k1,310:31054300,15449574:139810
x1,310:31564170,15449574
k1,310:31703980,15449574:139810
x1,310:33159535,15449574
x1,310:33377770,15449574
k1,311:33377770,15449574:0
)
(1,311:2706922,16236006:30670848,447283,142540
x1,311:3507772,16236006
x1,311:4308622,16236006
k1,310:4482173,16236006:173551
x1,310:5137533,16236006
k1,310:5311084,16236006:173551
x1,310:6111934,16236006
k1,310:6285486,16236006:173552
x1,310:7523461,16236006
k1,310:7697012,16236006:173551
x1,310:8971032,16236006
k1,310:9144583,16236006:173551
x1,310:10200368,16236006
k1,310:10373919,16236006:173551
x1,310:10919834,16236006
k1,310:11093385,16236006:173551
x1,310:11894235,16236006
k1,310:12067786,16236006:173551
x1,310:13305106,16236006
k1,310:13478658,16236006:173552
x1,310:14097318,16236006
k1,310:14270869,16236006:173551
x1,310:14780084,16236006
x1,310:16344429,16236006
k1,310:16517980,16236006:173551
x1,310:17027850,16236006
k1,310:17201401,16236006:173551
x1,310:17492381,16236006
x1,310:17810230,16236006
x1,310:18793270,16236006
x1,310:19667520,16236006
k1,310:19841071,16236006:173551
x1,310:20350941,16236006
k1,310:20524493,16236006:173552
x1,310:21325343,16236006
k1,310:21498894,16236006:173551
x1,310:21972064,16236006
x1,310:22854178,16236006
k1,310:23027729,16236006:173551
x1,310:24046814,16236006
x1,310:24364663,16236006
k1,310:24538214,16236006:173551
x1,310:26286059,16236006
k1,310:26459610,16236006:173551
x1,310:27515395,16236006
k1,310:27688946,16236006:173551
x1,310:28307606,16236006
k1,310:28481158,16236006:173552
x1,310:29354753,16236006
x1,310:29645733,16236006
x1,310:30955798,16236006
k1,310:31129349,16236006:173551
x1,310:32403369,16236006
k1,310:32576920,16236006:173551
x1,310:33377770,16236006
k1,310:33377770,16236006:0
)
(1,311:2706922,17022438:30670848,447283,142540
x1,311:3289537,17022438
x1,311:5036727,17022438
x1,311:5874277,17022438
g1,310:6038117,17022438
x1,310:6511287,17022438
x1,310:7011326,17022438
g1,310:7175166,17022438
x1,310:7830526,17022438
g1,310:7994366,17022438
x1,310:8940706,17022438
g1,310:9104546,17022438
x1,310:10560101,17022438
k1,311:33377769,17022438:22817668
g1,311:33377769,17022438
)
(1,316:2706922,19929333:30670848,2242622,1905768
(1,311:2706922,19929333:0,0,0
g1,311:2706922,19929333
g1,311:2706922,19929333
g1,311:2379242,19929333
(1,311:2379242,19929333:0,0,0
)
g1,311:2706922,19929333
)
(1,316:2706922,19929333:30670848,2242622,1905768
$1,316:2706922,19929333
g1,311:4279786,19929333
(1,316:4279786,19929333:0,0,0
(1,311:4279786,19929333:0,0,0
$1,311:4279786,19929333
(1,311:4279786,19142901:0,0,0
)
$1,311:4279786,19929333
)
)
[1,315:4279786,19929333:11733341,2242622,1905768
(1,313:4279786,18331584:11733341,644873,629148
g1,313:4279786,18331584
(1,313:4279786,18331584:835189,644873,629148
r1,313:4279786,18331584:0,786432,235932
g1,313:4378090,18331584
$1,313:4378090,18331584
x1,313:4794898,18331584
(1,313:4794898,18429887:221773,202768,0
x1,313:4973352,18429887
)
$1,313:5016671,18331584
g1,313:5016671,18331584
g1,313:5114975,18331584
)
g1,313:5114975,18331584
(1,313:5114975,18331584:613416,644873,629148
g1,313:5213279,18331584
g1,313:5213279,18331584
$1,313:5213279,18331584
x1,313:5630087,18331584
$1,313:5630087,18331584
g1,313:5630087,18331584
g1,313:5728391,18331584
)
g1,313:5728391,18331584
(1,313:5728391,18331584:10284736,644873,629148
g1,313:5826695,18331584
$1,313:5826695,18331584
[1,313:5826695,18331584:1183120,591526,193363
(1,313:6035427,18198218:0,413204,0
x1,313:6253662,18198218
)
(1,313:5826695,18331584:1183120,591526,193363
x1,313:6316904,18331584
[1,313:6316904,18517378:692911,777320,7569
(1,313:6316904,18060921:292946,320863,0
(1,313:6316904,17894395:260178,154337,0
x1,313:6544314,17894395
)
)
(1,313:6316904,18517378:692911,309657,7569
x1,313:6495358,18517378
x1,313:6964661,18517378
)
]
)
]
g1,313:7119039,18331584
(1,313:7119039,18331584:4076555,644873,308020
(1,313:7119039,17723411:251003,36700,916193
x1,313:7370042,17723411
)
(1,313:7370042,18331584:3746909,644873,308020
(1,313:7370042,17723411:233308,36700,916193
x1,313:7603350,17723411
)
[1,313:7603350,18331584:1183120,591526,193363
(1,313:7812082,18198218:0,413204,0
x1,313:8030317,18198218
)
(1,313:7603350,18331584:1183120,591526,193363
x1,313:8093559,18331584
[1,313:8093559,18517378:692911,777320,7569
(1,313:8093559,18060921:292946,320863,0
(1,313:8093559,17894395:260178,154337,0
x1,313:8320969,17894395
)
)
(1,313:8093559,18517378:692911,309657,7569
x1,313:8272013,18517378
x1,313:8741316,18517378
)
]
)
]
g1,313:8932102,18331584
x1,313:9348910,18331584
g1,313:9494542,18331584
[1,313:9494542,18331584:1389101,591526,169442
(1,313:9703274,18198218:0,413204,0
x1,313:9921509,18198218
)
(1,313:9494542,18331584:1389101,591526,169442
x1,313:9984751,18331584
[1,313:9984751,18493457:898892,753399,7569
(1,313:9984751,18060921:292946,320863,0
(1,313:9984751,17894395:260178,154337,0
x1,313:10212161,17894395
)
)
(1,313:9984751,18493457:898892,202768,7569
x1,313:10850875,18493457
)
]
)
]
(1,313:10883643,17723411:233308,36700,916193
x1,313:11116951,17723411
)
)
h1,313:11116951,18331584:78643,0,0
)
$1,313:11195594,18331584
$1,313:11195594,18331584
h1,313:11195594,18331584:0,0,0
r1,313:11195594,18331584:0,629148,629148
$1,313:11195594,18331584
k1,313:15914823,18331584:4719229
g1,313:16013127,18331584
)
g1,313:16013127,18331584
)
(1,315:4279786,20037487:11733341,1076755,1797614
g1,314:4279786,20037487
(1,314:4279786,20037487:835189,1076755,1797614
r1,314:4279786,20037487:0,786432,235932
g1,314:4378090,20037487
$1,314:4378090,20037487
x1,314:4711013,20037487
$1,314:4711013,20037487
k1,314:5016671,20037487:305658
g1,314:5114975,20037487
)
g1,314:5114975,20037487
(1,314:5114975,20037487:613416,1076755,1797614
g1,314:5213279,20037487
g1,314:5213279,20037487
$1,314:5213279,20037487
x1,314:5630087,20037487
$1,314:5630087,20037487
g1,314:5630087,20037487
g1,314:5728391,20037487
)
g1,314:5728391,20037487
(1,315:5728391,20037487:10284736,1076755,1797614
g1,314:5826695,20037487
$1,315:5826695,20037487
(1,315:5826695,20037487:10088128,1076755,1797614
(1,315:5826695,20037487:10088128,1076755,1797614
h1,315:5826695,20037487:78643,0,0
[1,315:5905338,20037487:9930842,1076755,1797614
(1,315:5905338,19593809:9930842,633077,0
k1,315:10646626,19593809:4741288
[1,315:10646626,19593809:448266,633077,0
(1,315:10739032,19454545:0,493813,0
x1,315:11057537,19454545
)
(1,315:10646626,19593809:448266,428277,0
x1,315:11079819,19593809
)
]
k1,315:15836180,19593809:4741288
)
(1,315:5905338,21099955:9930842,1102445,735146
x1,315:6229086,21099955
(1,315:6229086,21198258:236454,202768,3440
x1,315:6432772,21198258
)
x1,315:7075025,21099955
g1,315:7307527,21099955
x1,315:7724335,21099955
g1,315:7906375,21099955
(1,315:7906375,21099955:1547960,379453,8191
x1,315:9289840,21099955
x1,315:9454335,21099955
)
x1,315:9672570,21099955
g1,315:9818202,21099955
x1,315:9982042,21099955
g1,315:10127674,21099955
(1,315:10127674,21099955:5708506,1102445,735146
[1,315:10127674,20064655:262143,36700,1770446
(1,315:10127674,20064655:262143,36700,469237
x1,315:10389817,20064655
)
(1,315:10127674,20520784:262143,-13108,163184
x1,315:10389817,20520784
)
(1,315:10127674,20670860:262143,-13108,163184
x1,315:10389817,20670860
)
(1,315:10127674,20820936:262143,-13108,163184
x1,315:10389817,20820936
)
(1,315:10127674,20971012:262143,-13108,163184
x1,315:10389817,20971012
)
(1,315:10127674,21121088:262143,-13108,163184
x1,315:10389817,21121088
)
(1,315:10127674,21271164:262143,-13108,563937
x1,315:10389817,21271164
)
]
x1,315:10806625,21099955
g1,315:10952257,21099955
x1,315:11116097,21099955
g1,315:11261729,21099955
(1,315:11261729,21099955:1351219,1076755,660108
[1,315:11261729,20139693:262143,36700,1620370
(1,315:11261729,20139693:262143,36700,469237
x1,315:11523872,20139693
)
(1,315:11261729,20595822:262143,-13108,163184
x1,315:11523872,20595822
)
(1,315:11261729,20745898:262143,-13108,163184
x1,315:11523872,20745898
)
(1,315:11261729,20895974:262143,-13108,163184
x1,315:11523872,20895974
)
(1,315:11261729,21046050:262143,-13108,163184
x1,315:11523872,21046050
)
(1,315:11261729,21196126:262143,-13108,563937
x1,315:11523872,21196126
)
]
(1,315:11523872,21099955:826933,1076755,551319
(1,315:11523872,21099955:826933,1076755,551319
h1,315:11523872,21099955:78643,0,0
[1,315:11602515,21099955:669647,1076755,551319
(1,315:11602515,20656277:669647,633077,0
k1,315:11713206,20656277:110691
[1,315:11713206,20656277:448266,633077,0
(1,315:11805612,20517013:0,493813,0
x1,315:12124117,20517013
)
(1,315:11713206,20656277:448266,428277,0
x1,315:12146399,20656277
)
]
k1,315:12272162,20656277:110690
)
(1,315:11602515,21549531:669647,428277,101743
x1,315:12035708,21549531
(1,315:12035708,21647834:236454,202768,3440
x1,315:12239394,21647834
)
)
]
h1,315:12272162,21099955:78643,0,0
)
)
[1,315:12350805,20139693:262143,36700,1620370
(1,315:12350805,20139693:262143,36700,469237
x1,315:12612948,20139693
)
(1,315:12350805,20595822:262143,-13108,163184
x1,315:12612948,20595822
)
(1,315:12350805,20745898:262143,-13108,163184
x1,315:12612948,20745898
)
(1,315:12350805,20895974:262143,-13108,163184
x1,315:12612948,20895974
)
(1,315:12350805,21046050:262143,-13108,163184
x1,315:12612948,21046050
)
(1,315:12350805,21196126:262143,-13108,563937
x1,315:12612948,21196126
)
]
)
(1,315:12612948,20200278:363987,202768,3440
x1,315:12944167,20200278
)
g1,315:13122567,21099955
x1,315:13539375,21099955
g1,315:13685007,21099955
x1,315:14230922,21099955
g1,315:14376554,21099955
x1,315:14793362,21099955
g1,315:14938994,21099955
x1,315:15574037,21099955
[1,315:15574037,20064655:262143,36700,1770446
(1,315:15574037,20064655:262143,36700,469237
x1,315:15836180,20064655
)
(1,315:15574037,20520784:262143,-13108,163184
x1,315:15836180,20520784
)
(1,315:15574037,20670860:262143,-13108,163184
x1,315:15836180,20670860
)
(1,315:15574037,20820936:262143,-13108,163184
x1,315:15836180,20820936
)
(1,315:15574037,20971012:262143,-13108,163184
x1,315:15836180,20971012
)
(1,315:15574037,21121088:262143,-13108,163184
x1,315:15836180,21121088
)
(1,315:15574037,21271164:262143,-13108,563937
x1,315:15836180,21271164
)
]
)
)
]
h1,315:15836180,20037487:78643,0,0
)
)
$1,315:15914823,20037487
g1,315:15914823,20037487
g1,315:16013127,20037487
)
g1,315:16013127,20037487
)
]
(1,316:16013127,19929333:0,0,0
(1,316:16013127,19929333:0,0,0
$1,316:16013127,19929333
h1,316:16013127,19929333:0,0,0
$1,316:16013127,19929333
)
)
$1,316:16013127,19929333
k1,316:32613620,19929333:16600493
(1,316:32613620,19929333:764150,438435,116326
x1,316:33377770,19929333
)
)
g1,316:33377770,19929333
g1,316:33377770,19929333
)
(1,319:2706922,23478793:30670848,449576,11468
(1,319:2706922,23478793:819200,449576,8847
g1,319:2706922,23478793
x1,319:3198442,23478793
g1,319:3526122,23478793
)
x1,319:5420112,23478793
g1,319:5583952,23478793
x1,319:7440587,23478793
g1,319:7604427,23478793
x1,319:9860832,23478793
k1,319:33377770,23478793:23516938
g1,319:33377770,23478793
)
(1,321:2706922,25064764:30670848,447283,142540
h1,320:2706922,25064764:786432,0,0
x1,320:4330904,25064764
k1,320:4549425,25064764:218521
x1,320:6478805,25064764
k1,320:6697327,25064764:218522
x1,320:7497522,25064764
k1,320:7716043,25064764:218521
x1,320:9899703,25064764
k1,320:10118225,25064764:218522
x1,320:10628095,25064764
k1,320:10846616,25064764:218521
x1,320:13249166,25064764
k1,320:13467687,25064764:218521
x1,320:14268537,25064764
k1,320:14487059,25064764:218522
x1,320:16780164,25064764
k1,320:16998685,25064764:218521
x1,320:17289665,25064764
x1,320:18845489,25064764
x1,320:19156785,25064764
x1,320:19437934,25064764
k1,320:19656455,25064764:218521
x1,320:21476390,25064764
k1,320:21694912,25064764:218522
x1,320:23696382,25064764
k1,320:23914903,25064764:218521
x1,320:26644478,25064764
k1,320:26863000,25064764:218522
x1,320:28536790,25064764
k1,320:28755311,25064764:218521
x1,320:29556161,25064764
k1,320:29774682,25064764:218521
x1,320:31412427,25064764
k1,320:31630949,25064764:218522
x1,320:32540589,25064764
k1,320:32759110,25064764:218521
x1,320:33377770,25064764
k1,320:33377770,25064764:0
)
(1,321:2706922,25851196:30670848,447283,142540
x1,321:5419457,25851196
k1,320:5651148,25851196:231691
x1,320:7252848,25851196
k1,320:7484540,25851196:231692
x1,320:8285390,25851196
x1,320:8603239,25851196
k1,320:8834930,25851196:231691
x1,320:9744570,25851196
k1,320:9976262,25851196:231692
x1,320:10631622,25851196
k1,320:10863313,25851196:231691
x1,320:12665553,25851196
k1,320:12897245,25851196:231692
x1,320:14062475,25851196
k1,320:14294166,25851196:231691
x1,320:16295636,25851196
k1,320:16527328,25851196:231692
x1,320:19256903,25851196
k1,320:19488594,25851196:231691
x1,320:21454019,25851196
k1,320:21685711,25851196:231692
x1,320:22814241,25851196
x1,320:23816942,25851196
k1,320:24048633,25851196:231691
x1,320:24558503,25851196
k1,320:24790195,25851196:231692
x1,320:26610130,25851196
k1,320:26841821,25851196:231691
x1,320:27642671,25851196
k1,320:27874363,25851196:231692
x1,320:28820703,25851196
x1,320:30998464,25851196
k1,320:31230155,25851196:231691
x1,320:33377770,25851196
k1,320:33377770,25851196:0
)
(1,321:2706922,26637628:30670848,447283,142540
x1,321:3471072,26637628
k1,320:3693198,26637628:222126
x1,320:4494048,26637628
k1,320:4716174,26637628:222126
x1,320:6809394,26637628
k1,320:7031520,26637628:222126
x1,320:7359200,26637628
x1,320:7855962,26637628
k1,320:8078089,26637628:222127
x1,320:9279364,26637628
k1,320:9501490,26637628:222126
x1,320:10339040,26637628
k1,320:10561166,26637628:222126
x1,320:13182606,26637628
k1,320:13404732,26637628:222126
x1,320:14205582,26637628
k1,320:14427708,26637628:222126
x1,320:16575323,26637628
k1,320:16797449,26637628:222126
x1,320:19709214,26637628
k1,320:19931340,26637628:222126
x1,320:21588090,26637628
k1,320:21810216,26637628:222126
x1,320:22829301,26637628
k1,320:23051428,26637628:222127
x1,320:23997768,26637628
x1,320:25556869,26637628
k1,320:25778995,26637628:222126
x1,320:27780465,26637628
k1,320:28002591,26637628:222126
x1,320:28621251,26637628
x1,320:28939100,26637628
x1,320:29693419,26637628
k1,320:29915545,26637628:222126
x1,320:30716395,26637628
k1,320:30938521,26637628:222126
x1,320:31229501,26637628
x1,320:32785325,26637628
x1,320:33096621,26637628
x1,320:33377770,26637628
k1,320:33377770,26637628:0
)
(1,321:2706922,27424060:30670848,447283,142540
x1,321:4199832,27424060
k1,320:4396534,27424060:196702
x1,320:4906404,27424060
k1,320:5103105,27424060:196701
x1,320:7723235,27424060
k1,320:7919937,27424060:196702
x1,320:8866277,27424060
k1,320:9062978,27424060:196701
x1,320:10738078,27424060
x1,320:11525820,27424060
k1,320:11722522,27424060:196702
x1,320:12523372,27424060
k1,320:12720073,27424060:196701
x1,320:14521658,27424060
k1,320:14718360,27424060:196702
x1,320:17194310,27424060
k1,320:17391012,27424060:196702
x1,320:19556977,27424060
k1,320:19753678,27424060:196701
x1,320:23212013,27424060
k1,320:23408715,27424060:196702
x1,320:27176380,27424060
k1,320:27373081,27424060:196701
x1,320:28902036,27424060
x1,320:29958476,27424060
k1,320:30155178,27424060:196702
x1,320:30701093,27424060
k1,320:30897794,27424060:196701
x1,320:31516454,27424060
x1,320:31834303,27424060
k1,320:32031005,27424060:196702
x1,320:33377770,27424060
k1,320:33377770,27424060:0
)
(1,321:2706922,28210492:30670848,447283,142540
x1,321:6310747,28210492
k1,320:6484111,28210492:173364
x1,320:7030026,28210492
k1,320:7203391,28210492:173365
x1,320:9023981,28210492
k1,320:9197345,28210492:173364
x1,320:10835090,28210492
k1,320:11008455,28210492:173365
x1,320:11954795,28210492
k1,320:12128159,28210492:173364
x1,320:15313864,28210492
k1,320:15487229,28210492:173365
x1,320:17598799,28210492
k1,320:17772163,28210492:173364
x1,320:18572358,28210492
k1,320:18745723,28210492:173365
x1,320:21730888,28210492
k1,320:21904252,28210492:173364
x1,320:22668402,28210492
k1,320:22841767,28210492:173365
x1,320:25317717,28210492
k1,320:25491081,28210492:173364
x1,320:26765101,28210492
k1,320:26938466,28210492:173365
x1,320:27739316,28210492
k1,320:27912680,28210492:173364
x1,320:28859020,28210492
x1,320:30418121,28210492
k1,320:30591486,28210492:173365
x1,320:32265931,28210492
x1,320:32403556,28210492
k1,320:32576920,28210492:173364
x1,320:33377770,28210492
k1,320:33377770,28210492:0
)
(1,321:2706922,28996924:30670848,447283,142540
x1,321:5583297,28996924
g1,320:5747137,28996924
x1,320:6257007,28996924
g1,320:6420847,28996924
x1,320:9040977,28996924
g1,320:9204817,28996924
x1,320:9823477,28996924
x1,320:10141326,28996924
g1,320:10305166,28996924
x1,320:12089056,28996924
g1,320:12252896,28996924
x1,320:13017046,28996924
g1,320:13180886,28996924
x1,320:14782586,28996924
g1,320:14946426,28996924
x1,320:15892766,28996924
x1,320:17451867,28996924
g1,320:17615707,28996924
x1,320:17906687,28996924
x1,320:19262626,28996924
k1,321:33377770,28996924:14115144
g1,321:33377770,28996924
)
(1,322:2706922,30911936:30670848,438763,135004
(1,322:2706922,30911936:0,0,0
g1,322:2706922,30911936
)
(1,322:2706922,30911936:0,0,0
(1,322:2706922,30911936:0,0,0
(1,322:2706922,30125504:0,0,0
)
)
g1,322:2706922,30911936
)
x1,322:4527512,30911936
x1,322:8124783,30911936
k1,322:33377771,30911936:25252988
g1,322:33377771,30911936
)
(1,325:2706922,32497907:30670848,447283,142540
h1,324:2706922,32497907:786432,0,0
x1,324:5240544,32497907
x1,324:8682495,32497907
k1,324:8879977,32497907:197482
x1,324:9826317,32497907
k1,324:10023799,32497907:197482
x1,324:12679974,32497907
k1,324:12877455,32497907:197481
x1,324:14952325,32497907
k1,324:15149807,32497907:197482
x1,324:16897652,32497907
k1,324:17095134,32497907:197482
x1,324:17713794,32497907
k1,324:17911276,32497907:197482
x1,324:18784871,32497907
k1,324:18982353,32497907:197482
x1,324:20111538,32497907
x1,324:21258418,32497907
k1,324:21455899,32497907:197481
x1,324:22784969,32497907
k1,324:22982451,32497907:197482
x1,324:24147681,32497907
k1,324:24345163,32497907:197482
x1,324:25146013,32497907
k1,324:25343495,32497907:197482
x1,324:26363235,32497907
k1,324:26560717,32497907:197482
x1,324:27907482,32497907
k1,324:28104963,32497907:197481
x1,324:30943983,32497907
k1,324:31141465,32497907:197482
x1,324:31469145,32497907
x1,324:31965907,32497907
k1,324:32163389,32497907:197482
x1,324:32782049,32497907
x1,324:33096621,32497907
x1,324:33377770,32497907
k1,324:33377770,32497907:0
)
(1,325:2706922,33284339:30670848,447283,8846
x1,325:3362282,33284339
g1,324:3526122,33284339
x1,324:5947022,33284339
g1,324:6110862,33284339
x1,324:6511287,33284339
x1,324:6756392,33284339
x1,324:7256431,33284339
g1,324:7420271,33284339
x1,324:8548801,33284339
x1,324:9005587,33284339
g1,324:9169427,33284339
x1,324:11681422,33284339
g1,324:11845262,33284339
x1,324:12391177,33284339
g1,324:12555017,33284339
x1,324:14575492,33284339
k1,325:33377770,33284339:18802278
g1,325:33377770,33284339
)
(1,334:2706922,35199351:30670848,449576,134348
(1,334:2706922,35199351:4007526,449576,134348
g1,334:2706922,35199351
x1,334:3180092,35199351
x1,334:5422078,35199351
g1,334:5585918,35199351
g1,334:5749758,35199351
x1,334:6386768,35199351
g1,334:6714448,35199351
)
x1,334:7551998,35199351
g1,334:7715838,35199351
x1,334:10045643,35199351
g1,334:10209483,35199351
x1,334:12795533,35199351
k1,334:33377769,35199351:20582236
g1,334:33377769,35199351
)
(1,336:2706922,36785322:30670848,447283,142540
h1,335:2706922,36785322:786432,0,0
x1,335:5604924,36785322
k1,335:5837436,36785322:232512
x1,335:8313386,36785322
k1,335:8545898,36785322:232512
x1,335:9164558,36785322
k1,335:9397071,36785322:232513
x1,335:11799621,36785322
k1,335:12032133,36785322:232512
x1,335:13888768,36785322
k1,335:14121280,36785322:232512
x1,335:15869125,36785322
k1,335:16101637,36785322:232512
x1,335:16756997,36785322
k1,335:16989510,36785322:232513
x1,335:17572125,36785322
k1,335:17804637,36785322:232512
x1,335:19478427,36785322
k1,335:19710939,36785322:232512
x1,335:22622049,36785322
k1,335:22854561,36785322:232512
x1,335:24875036,36785322
k1,335:25107548,36785322:232512
x1,335:27365263,36785322
k1,335:27597776,36785322:232513
x1,335:30509541,36785322
k1,335:30742053,36785322:232512
x1,335:32489898,36785322
k1,335:32722410,36785322:232512
x1,335:33377770,36785322
k1,335:33377770,36785322:0
)
(1,336:2706922,37571754:30670848,447283,142540
x1,336:3325582,37571754
x1,335:3640154,37571754
x1,335:3921303,37571754
g1,335:4085143,37571754
x1,335:6414948,37571754
g1,335:6578788,37571754
x1,335:7088658,37571754
g1,335:7252498,37571754
x1,335:8053348,37571754
g1,335:8217188,37571754
x1,335:9455163,37571754
g1,335:9619003,37571754
x1,335:10820278,37571754
g1,335:10984118,37571754
x1,335:11930458,37571754
x1,335:12248307,37571754
x1,335:12693296,37571754
g1,335:12857136,37571754
x1,335:13876221,37571754
x1,335:14194070,37571754
g1,335:14357910,37571754
x1,335:15377650,37571754
g1,335:15541490,37571754
x1,335:19109270,37571754
g1,335:19273110,37571754
x1,335:19891770,37571754
g1,335:20055610,37571754
x1,335:22057080,37571754
g1,335:22220920,37571754
x1,335:22857930,37571754
g1,335:23021770,37571754
x1,335:23622735,37571754
g1,335:23786575,37571754
x1,335:24223700,37571754
g1,335:24387540,37571754
x1,335:25315530,37571754
k1,336:33377770,37571754:8062240
g1,336:33377770,37571754
)
(1,337:2706922,39093550:30670848,448266,134676
(1,337:2706922,39093550:1383465,438108,7863
g1,337:2706922,39093550
x1,337:3762707,39093550
g1,337:4090387,39093550
)
x1,337:6383492,39093550
g1,337:6547332,39093550
x1,337:7057202,39093550
g1,337:7221042,39093550
x1,337:7548722,39093550
g1,337:7712562,39093550
x1,337:8841092,39093550
x1,337:10952662,39093550
g1,337:11116502,39093550
x1,337:12755557,39093550
g1,337:12919397,39093550
x1,337:13574757,39093550
g1,337:13738597,39093550
x1,337:16141147,39093550
k1,337:33377771,39093550:17236624
g1,337:33377771,39093550
)
(1,346:2706922,40666414:30670848,447283,142540
h1,338:2706922,40666414:786432,0,0
x1,338:5021654,40666414
g1,338:5185494,40666414
x1,338:5622619,40666414
g1,338:5786459,40666414
x1,338:6842244,40666414
g1,338:7006084,40666414
x1,338:7806934,40666414
g1,338:7970774,40666414
x1,338:9645874,40666414
g1,338:9809714,40666414
x1,338:10319584,40666414
g1,338:10483424,40666414
x1,338:12412804,40666414
g1,338:12576644,40666414
x1,338:12867624,40666414
g1,338:13031464,40666414
x1,338:16016629,40666414
g1,338:16180469,40666414
x1,338:17855569,40666414
g1,338:18019409,40666414
x1,338:18820259,40666414
g1,338:18984099,40666414
x1,338:21568839,40666414
g1,338:21732679,40666414
x1,338:22133104,40666414
g1,338:22296944,40666414
x1,338:23279984,40666414
g1,338:23443824,40666414
x1,338:24845639,40666414
k1,346:33377770,40666414:8532131
g1,346:33377770,40666414
)
(1,359:2706922,42581426:30670848,449576,8847
(1,359:2706922,42581426:0,0,0
g1,359:2706922,42581426
)
(1,359:2706922,42581426:0,0,0
(1,359:2706922,42581426:0,0,0
(1,359:2706922,41794994:0,0,0
)
)
g1,359:2706922,42581426
)
x1,359:4271267,42581426
x1,359:5751725,42581426
k1,359:33377769,42581426:27626044
g1,359:33377769,42581426
)
(1,367:3624426,44036325:29753344,358613,114032
(1,365:3624426,44036325:0,0,0
g1,365:3624426,44036325
g1,365:2313704,44036325
g1,365:1986024,44036325
(1,365:1986024,44036325:1310722,0,0
g1,365:1986024,44036325
g1,365:1986024,44036325
(1,365:1986024,44036325:0,0,0
(1,365:1986024,43380965:0,0,0
)
)
k1,365:3296746,44036325:1310722
)
g1,365:3624426,44036325
)
x1,365:4920466,44036325
k1,365:5083216,44036325:162750
x1,365:5403556,44036325
x1,365:5626902,44036325
k1,365:5789652,44036325:162750
x1,365:6284580,44036325
x1,365:7407605,44036325
x1,365:7661884,44036325
x1,365:7758877,44036325
k1,365:7921627,44036325:162750
x1,365:8533471,44036325
k1,365:8696221,44036325:162750
x1,365:9307541,44036325
k1,365:9470291,44036325:162750
x1,365:10795167,44036325
k1,365:10957917,44036325:162750
x1,365:11598597,44036325
k1,365:11761347,44036325:162750
x1,365:12940995,44036325
k1,365:13103745,44036325:162750
x1,365:14093601,44036325
x1,365:15928085,44036325
k1,365:16090835,44036325:162750
x1,365:17969883,44036325
k1,365:18132634,44036325:162751
x1,365:18540530,44036325
k1,365:18703280,44036325:162750
x1,365:20625320,44036325
k1,365:20788070,44036325:162750
x1,365:21370554,44036325
x1,365:22673409,44036325
x1,365:23037265,44036325
k1,365:23200015,44036325:162750
x1,365:23782499,44036325
k1,366:23945249,44036325:162750
x1,366:25809617,44036325
x1,366:26549387,44036325
k1,366:26712137,44036325:162750
x1,366:27192909,44036325
k1,366:27355659,44036325:162750
x1,366:28549463,44036325
k1,366:28712213,44036325:162750
x1,366:30837677,44036325
k1,366:31000427,44036325:162750
x1,366:32238271,44036325
k1,366:32401021,44036325:162750
x1,366:33012341,44036325
x1,366:33377770,44036325
k1,366:33377770,44036325:0
)
(1,367:3624426,44691685:29753344,357826,114032
x1,367:4002962,44691685
x1,366:4775238,44691685
g1,366:4906310,44691685
x1,366:5561670,44691685
g1,366:5692742,44691685
x1,366:6610246,44691685
k1,367:33377770,44691685:26767524
g1,367:33377770,44691685
)
]
(1,372:2706922,44691685:30670848,0,0
h1,372:2706922,44691685:30670848,0,0
)
]
]
]
!28395
}4
!10
{5
[1,379:4736287,44691685:28358645,39955398,0
[1,379:4736287,4736287:0,0,0
(1,379:4736287,2656652:0,0,0
k1,379:4736287,2656652:2377984
)
]
[1,379:4736287,44691685:28358645,39955398,0
[1,379:2424084,44691685:30670848,41969252,0
[1,379:2424084,3377793:30670848,655360,0
(1,379:2424084,3377793:30670848,358613,107741
(1,379:2424084,3377793:30670848,358613,107741
k1,379:10406894,3377793:7982810
x1,379:10727234,3377793
x1,379:11852880,3377793
g1,379:11983952,3377793
x1,379:13119560,3377793
g1,379:13250632,3377793
x1,379:13345528,3377793
g1,379:13476600,3377793
x1,379:13768104,3377793
x1,379:13943216,3377793
x1,379:16615511,3377793
g1,379:16746583,3377793
x1,379:18202531,3377793
x1,379:18415916,3377793
x1,379:18670195,3377793
g1,379:18801267,3377793
x1,379:19325555,3377793
x1,379:20699714,3377793
g1,379:20830786,3377793
x1,379:21355074,3377793
g1,379:21486146,3377793
x1,379:22883898,3377793
g1,379:23014970,3377793
x1,379:23801402,3377793
x1,379:24849978,3377793
k1,379:32832788,3377793:7982810
x1,379:33094932,3377793
)
)
]
[1,379:2424084,44691685:30670848,40658532,0
(1,369:3341588,4688513:29753344,357826,114032
(1,368:3341588,4688513:0,0,0
g1,368:3341588,4688513
g1,368:2030866,4688513
g1,368:1703186,4688513
(1,368:1703186,4688513:1310722,0,0
g1,368:1703186,4688513
g1,368:1703186,4688513
(1,368:1703186,4688513:0,0,0
(1,368:1703186,4033153:0,0,0
)
)
k1,368:3013908,4688513:1310722
)
g1,368:3341588,4688513
)
x1,368:4462516,4688513
g1,368:4593588,4688513
x1,368:5205432,4688513
g1,368:5336504,4688513
x1,368:6151772,4688513
x1,368:6406051,4688513
x1,368:6762042,4688513
g1,368:6893114,4688513
x1,368:7533794,4688513
g1,368:7664866,4688513
x1,368:8844514,4688513
g1,368:8975586,4688513
x1,368:10634958,4688513
g1,368:10766030,4688513
x1,368:13416830,4688513
g1,368:13547902,4688513
x1,368:14159222,4688513
g1,368:14290294,4688513
x1,368:14930974,4688513
g1,368:15062046,4688513
x1,368:16838334,4688513
g1,368:16969406,4688513
x1,368:19066558,4688513
g1,368:19197630,4688513
x1,368:19634362,4688513
g1,368:19765434,4688513
x1,368:21382338,4688513
g1,368:21513410,4688513
x1,368:23056914,4688513
g1,368:23187986,4688513
x1,368:23624718,4688513
g1,368:23755790,4688513
x1,368:25445046,4688513
g1,368:25576118,4688513
x1,368:26129766,4688513
x1,368:27175720,4688513
g1,368:27306792,4688513
x1,368:28355368,4688513
g1,368:28486440,4688513
x1,368:29010728,4688513
x1,368:29272872,4688513
x1,368:29928232,4688513
k1,369:33094932,4688513:3166700
g1,369:33094932,4688513
)
(1,371:3341588,5343873:29753344,357826,114032
(1,370:3341588,5343873:0,0,0
g1,370:3341588,5343873
g1,370:2030866,5343873
g1,370:1703186,5343873
(1,370:1703186,5343873:1310722,0,0
g1,370:1703186,5343873
g1,370:1703186,5343873
(1,370:1703186,5343873:0,0,0
(1,370:1703186,4688513:0,0,0
)
)
k1,370:3013908,5343873:1310722
)
g1,370:3341588,5343873
)
x1,370:4622424,5343873
x1,370:5671000,5343873
g1,370:5802072,5343873
x1,370:7433132,5343873
g1,370:7564204,5343873
x1,370:9107708,5343873
g1,370:9238780,5343873
x1,370:10665892,5343873
g1,370:10796964,5343873
x1,370:11408284,5343873
g1,370:11539356,5343873
x1,370:12719004,5343873
g1,370:12850076,5343873
x1,370:14043880,5343873
g1,370:14174952,5343873
x1,370:15980600,5343873
g1,370:16111672,5343873
x1,370:18441084,5343873
x1,370:18538077,5343873
g1,370:18669149,5343873
x1,370:19732405,5343873
g1,370:19863477,5343873
x1,370:21043125,5343873
k1,371:33094932,5343873:12051807
g1,371:33094932,5343873
)
(1,373:3341588,5999233:29753344,357826,114032
(1,372:3341588,5999233:0,0,0
g1,372:3341588,5999233
g1,372:2030866,5999233
g1,372:1703186,5999233
(1,372:1703186,5999233:1310722,0,0
g1,372:1703186,5999233
g1,372:1703186,5999233
(1,372:1703186,5999233:0,0,0
(1,372:1703186,5343873:0,0,0
)
)
k1,372:3013908,5999233:1310722
)
g1,372:3341588,5999233
)
x1,372:3633092,5999233
x1,372:5430351,5999233
x1,372:5540451,5999233
k1,372:5717689,5999233:177238
x1,372:6183781,5999233
k1,372:6361019,5999233:177238
x1,372:7118091,5999233
k1,372:7295329,5999233:177238
x1,372:8430937,5999233
x1,372:8541037,5999233
k1,372:8718275,5999233:177238
x1,372:9446511,5999233
k1,372:9623749,5999233:177238
x1,372:11341841,5999233
x1,372:11707270,5999233
x1,372:11804263,5999233
k1,372:11981501,5999233:177238
x1,372:12593345,5999233
k1,372:12770583,5999233:177238
x1,372:15085839,5999233
k1,372:15263077,5999233:177238
x1,372:15816725,5999233
k1,372:15993963,5999233:177238
x1,372:18804147,5999233
k1,372:18981385,5999233:177238
x1,372:19593229,5999233
k1,372:19770467,5999233:177238
x1,372:20090807,5999233
x1,372:20626105,5999233
x1,372:20880384,5999233
x1,372:20977377,5999233
k1,372:21154615,5999233:177238
x1,372:21882851,5999233
k1,372:22060089,5999233:177238
x1,372:24579293,5999233
k1,372:24756531,5999233:177238
x1,372:25076871,5999233
x1,372:25300217,5999233
k1,372:25477455,5999233:177238
x1,372:26657103,5999233
k1,372:26834341,5999233:177238
x1,372:28144537,5999233
x1,372:28978679,5999233
k1,372:29155916,5999233:177237
x1,372:29592648,5999233
k1,372:29769886,5999233:177238
x1,372:30876658,5999233
k1,372:31053896,5999233:177238
x1,372:32102472,5999233
k1,372:32279664,5999233:177192
x1,372:33094932,5999233
k1,372:33094932,5999233:0
)
(1,373:3341588,6654593:29753344,357826,114032
x1,373:5205432,6654593
k1,372:5347761,6654593:142329
x1,372:5755657,6654593
k1,372:5897985,6654593:142328
x1,372:7412129,6654593
k1,372:7554458,6654593:142329
x1,372:8952210,6654593
k1,372:9094538,6654593:142328
x1,372:9531270,6654593
k1,372:9673599,6654593:142329
x1,372:11799587,6654593
k1,372:11941916,6654593:142329
x1,372:12815904,6654593
k1,372:12958232,6654593:142328
x1,372:13889892,6654593
k1,372:14032221,6654593:142329
x1,372:16435033,6654593
x1,372:16631117,6654593
k1,372:16773445,6654593:142328
x1,372:17559877,6654593
k1,372:17702206,6654593:142329
x1,372:20381318,6654593
k1,372:20523646,6654593:142328
x1,372:20843986,6654593
x1,372:22083403,6654593
k1,372:22225732,6654593:142329
x1,372:23973184,6654593
k1,372:24115513,6654593:142329
x1,372:24639801,6654593
k1,372:24782129,6654593:142328
x1,372:25830705,6654593
k1,372:25973034,6654593:142329
x1,372:26293374,6654593
x1,372:28614922,6654593
k1,372:28757250,6654593:142328
x1,372:30387786,6654593
k1,372:30530115,6654593:142329
x1,372:30850455,6654593
x1,372:32997939,6654593
x1,372:33094932,6654593
k1,372:33094932,6654593:0
)
(1,373:3341588,7309953:29753344,357826,114032
x1,373:5016688,7309953
g1,372:5147760,7309953
x1,372:6531356,7309953
g1,372:6662428,7309953
x1,372:7826872,7309953
g1,372:7957944,7309953
x1,372:9225148,7309953
k1,373:33094932,7309953:23869784
g1,373:33094932,7309953
)
(1,376:3341588,7965313:29753344,357826,114032
(1,374:3341588,7965313:0,0,0
g1,374:3341588,7965313
g1,374:2030866,7965313
g1,374:1703186,7965313
(1,374:1703186,7965313:1310722,0,0
g1,374:1703186,7965313
g1,374:1703186,7965313
(1,374:1703186,7965313:0,0,0
(1,374:1703186,7309953:0,0,0
)
)
k1,374:3013908,7965313:1310722
)
g1,374:3341588,7965313
)
x1,374:3633092,7965313
x1,374:5430351,7965313
x1,374:5540451,7965313
k1,374:5681044,7965313:140593
x1,374:6147136,7965313
k1,374:6287728,7965313:140592
x1,374:7467376,7965313
k1,374:7607969,7965313:140593
x1,374:8685381,7965313
x1,374:9519523,7965313
k1,374:9660115,7965313:140592
x1,374:10096847,7965313
k1,375:10237440,7965313:140593
x1,375:11286016,7965313
k1,375:11426598,7965313:140582
x1,375:12358782,7965313
k1,375:12499375,7965313:140593
x1,375:14450775,7965313
k1,375:14591367,7965313:140592
x1,375:14999263,7965313
k1,375:15139856,7965313:140593
x1,375:16799752,7965313
k1,375:16940344,7965313:140592
x1,375:18367456,7965313
k1,375:18508049,7965313:140593
x1,375:18944781,7965313
k1,375:19085373,7965313:140592
x1,375:21386473,7965313
k1,375:21527066,7965313:140593
x1,375:22517446,7965313
k1,375:22658038,7965313:140592
x1,375:23764810,7965313
k1,375:23905403,7965313:140593
x1,375:24196907,7965313
x1,375:26417266,7965313
k1,375:26557858,7965313:140592
x1,375:28217230,7965313
k1,375:28357823,7965313:140593
x1,375:30920543,7965313
k1,375:31061136,7965313:140593
x1,375:31469032,7965313
k1,375:31609624,7965313:140592
x1,375:33094932,7965313
k1,375:33094932,7965313:0
)
(1,376:3341588,8620673:29753344,357826,73924
x1,376:4652308,8620673
g1,375:4783380,8620673
x1,375:5438740,8620673
k1,376:33094932,8620673:27656192
g1,376:33094932,8620673
)
]
(1,379:2424084,44691685:30670848,0,0
h1,379:2424084,44691685:30670848,0,0
)
]
]
]
!8344
}5
!9
{6
[1,402:4736287,44691685:28641483,39955398,0
[1,402:4736287,4736287:0,0,0
(1,402:4736287,2656652:0,0,0
k1,402:4736287,2656652:2095146
)
]
[1,402:4736287,44691685:28641483,39955398,0
[1,402:2706922,44691685:30670848,41969252,0
[1,402:2706922,3377793:30670848,655360,0
(1,402:2706922,3377793:30670848,358613,107741
(1,402:2706922,3377793:30670848,358613,107741
x1,402:2969066,3377793
k1,402:10951876,3377793:7982810
x1,402:11272216,3377793
x1,402:12397862,3377793
g1,402:12528934,3377793
x1,402:13664542,3377793
g1,402:13795614,3377793
x1,402:13890510,3377793
g1,402:14021582,3377793
x1,402:14313086,3377793
x1,402:14488198,3377793
x1,402:17160493,3377793
g1,402:17291565,3377793
x1,402:18747513,3377793
x1,402:18960898,3377793
x1,402:19215177,3377793
g1,402:19346249,3377793
x1,402:19870537,3377793
x1,402:21244696,3377793
g1,402:21375768,3377793
x1,402:21900056,3377793
g1,402:22031128,3377793
x1,402:23428880,3377793
g1,402:23559952,3377793
x1,402:24346384,3377793
x1,402:25394960,3377793
k1,402:33377770,3377793:7982810
)
)
]
[1,402:2706922,44691685:30670848,40658532,0
(1,384:2706922,4688513:30670848,449576,134348
(1,384:2706922,4688513:0,0,0
g1,384:2706922,4688513
)
(1,384:2706922,4688513:0,0,0
(1,384:2706922,4688513:0,0,0
(1,384:2706922,3902081:0,0,0
)
)
g1,384:2706922,4688513
)
x1,384:6093167,4688513
g1,384:6257007,4688513
x1,384:6802922,4688513
g1,384:6966762,4688513
x1,384:7439932,4688513
x1,384:9227753,4688513
g1,384:9391593,4688513
x1,384:9609828,4688513
x1,384:10212104,4688513
g1,384:10375944,4688513
x1,384:11577874,4688513
x1,384:12281730,4688513
g1,384:12445570,4688513
x1,384:15102400,4688513
k1,384:33377770,4688513:18275370
g1,384:33377770,4688513
)
(1,386:2706922,6274484:30670848,449576,134348
(1,386:2706922,6274484:819200,449576,8847
g1,386:2706922,6274484
x1,386:3198442,6274484
g1,386:3526122,6274484
)
x1,386:4618607,6274484
g1,386:4782447,6274484
x1,386:6311402,6274484
g1,386:6475242,6274484
x1,386:6693477,6274484
x1,386:7295753,6274484
g1,386:7459593,6274484
x1,386:8661523,6274484
x1,386:9365379,6274484
g1,386:9529219,6274484
x1,386:12186049,6274484
k1,386:33377769,6274484:21191720
g1,386:33377769,6274484
)
(1,389:2706922,7860455:30670848,447283,142540
h1,388:2706922,7860455:786432,0,0
x1,388:4512439,7860455
k1,388:4742054,7860455:229615
x1,388:5542904,7860455
k1,388:5772518,7860455:229614
x1,388:7919478,7860455
k1,388:8149093,7860455:229615
x1,388:8586218,7860455
k1,388:8815833,7860455:229615
x1,388:10707858,7860455
k1,388:10937473,7860455:229615
x1,388:11483388,7860455
k1,388:11713002,7860455:229614
x1,388:12549897,7860455
k1,388:12779512,7860455:229615
x1,388:13580362,7860455
k1,388:13809977,7860455:229615
x1,388:15266187,7860455
k1,388:15495802,7860455:229615
x1,388:16733777,7860455
k1,388:16963391,7860455:229614
x1,388:18856071,7860455
k1,388:19085686,7860455:229615
x1,388:19741046,7860455
k1,388:19970661,7860455:229615
x1,388:20771511,7860455
k1,388:21001126,7860455:229615
x1,388:22311846,7860455
k1,388:22541394,7860455:229548
x1,388:25520660,7860455
x1,388:26660986,7860455
x1,388:27663687,7860455
x1,388:30773370,7860455
x1,388:30978497,7860455
x1,388:33377770,7860455
k1,388:33377770,7860455:0
)
(1,389:2706922,8646887:30670848,447283,142540
x1,389:5436497,8646887
x1,389:6454927,8646887
x1,389:8529797,8646887
x1,389:10640712,8646887
x1,389:12024177,8646887
x1,389:12970517,8646887
x1,388:13288366,8646887
k1,388:13414251,8646887:125885
x1,388:14178401,8646887
k1,388:14304286,8646887:125885
x1,388:16415201,8646887
k1,388:16541086,8646887:125885
x1,388:17341936,8646887
k1,388:17467821,8646887:125885
x1,388:18559651,8646887
x1,388:19277926,8646887
k1,388:19403773,8646887:125847
x1,388:20204623,8646887
k1,388:20330508,8646887:125885
x1,388:21168058,8646887
k1,388:21293943,8646887:125885
x1,388:21839858,8646887
k1,388:21965743,8646887:125885
x1,388:24258848,8646887
k1,388:24384733,8646887:125885
x1,388:25476563,8646887
x1,388:26194838,8646887
k1,388:26320685,8646887:125847
x1,388:28741585,8646887
k1,388:28867470,8646887:125885
x1,388:29886555,8646887
k1,388:30012440,8646887:125885
x1,388:30813290,8646887
k1,388:30939175,8646887:125885
x1,388:33377770,8646887
k1,388:33377770,8646887:0
)
(1,389:2706922,9433319:30670848,447283,142540
x1,389:4891237,9433319
g1,388:5055077,9433319
x1,388:5855927,9433319
g1,388:6019767,9433319
x1,388:7257742,9433319
x1,388:8552078,9433319
g1,388:8715918,9433319
x1,388:9990593,9433319
g1,388:10154433,9433319
k1,389:33377769,9433319:23223336
g1,389:33377769,9433319
)
(1,391:4345324,11006183:29032446,379453,142540
g1,391:3185337,11006183
(1,390:3185337,11006183:0,338820,0
g1,390:3185337,11006183
g1,390:1874615,11006183
g1,390:1658346,11006183
(1,390:1658346,11006183:1310722,338820,0
k1,390:2969068,11006183:1310722
(1,390:2969068,10960308:0,292945,0
k1,390:2643355,10960308:-325713
x1,390:2969068,10960308
)
)
g1,390:3185337,11006183
)
x1,390:5205157,11006183
k1,391:33377769,11006183:28172612
g1,391:33377769,11006183
)
(1,392:4345324,11792615:29032446,447283,6881
g1,392:3185337,11792615
(1,391:3185337,11792615:0,338820,0
g1,391:3185337,11792615
g1,391:1874615,11792615
g1,391:1658346,11792615
(1,391:1658346,11792615:1310722,338820,0
k1,391:2969068,11792615:1310722
(1,391:2969068,11746740:0,292945,0
k1,391:2643355,11746740:-325713
x1,391:2969068,11746740
)
)
g1,391:3185337,11792615
)
x1,391:6443132,11792615
k1,392:33377770,11792615:26934638
g1,392:33377770,11792615
)
(1,393:4345324,12579047:29032446,447283,142540
g1,393:3185337,12579047
(1,392:3185337,12579047:0,338820,0
g1,392:3185337,12579047
g1,392:1874615,12579047
g1,392:1658346,12579047
(1,392:1658346,12579047:1310722,338820,0
k1,392:2969068,12579047:1310722
(1,392:2969068,12533172:0,292945,0
k1,392:2643355,12533172:-325713
x1,392:2969068,12533172
)
)
g1,392:3185337,12579047
)
x1,392:5897217,12579047
k1,393:33377769,12579047:27480552
g1,393:33377769,12579047
)
(1,394:4345324,13365479:29032446,447283,6881
g1,394:3185337,13365479
(1,393:3185337,13365479:0,338820,0
g1,393:3185337,13365479
g1,393:1874615,13365479
g1,393:1658346,13365479
(1,393:1658346,13365479:1310722,338820,0
k1,393:2969068,13365479:1310722
(1,393:2969068,13319604:0,292945,0
k1,393:2643355,13319604:-325713
x1,393:2969068,13319604
)
)
g1,393:3185337,13365479
)
x1,393:4113982,13365479
g1,393:4277822,13365479
x1,393:5115372,13365479
k1,394:33377770,13365479:28262398
g1,394:33377770,13365479
)
(1,395:4345324,14151911:29032446,447283,142540
g1,395:3185337,14151911
(1,394:3185337,14151911:0,338820,0
g1,394:3185337,14151911
g1,394:1874615,14151911
g1,394:1658346,14151911
(1,394:1658346,14151911:1310722,338820,0
k1,394:2969068,14151911:1310722
(1,394:2969068,14106036:0,292945,0
k1,394:2643355,14106036:-325713
x1,394:2969068,14106036
)
)
g1,394:3185337,14151911
)
x1,394:6170502,14151911
g1,394:6334342,14151911
x1,394:8846337,14151911
g1,394:9010177,14151911
x1,394:9774327,14151911
g1,394:9938167,14151911
x1,394:10811762,14151911
g1,394:10975602,14151911
x1,394:12140832,14151911
g1,394:12304672,14151911
x1,394:13651437,14151911
g1,394:13815277,14151911
x1,394:17310312,14151911
g1,394:17474152,14151911
x1,394:18967062,14151911
k1,395:33377770,14151911:14410708
g1,395:33377770,14151911
)
(1,396:4345324,14938343:29032446,447283,142540
g1,396:3185337,14938343
(1,395:3185337,14938343:0,338820,0
g1,395:3185337,14938343
g1,395:1874615,14938343
g1,395:1658346,14938343
(1,395:1658346,14938343:1310722,338820,0
k1,395:2969068,14938343:1310722
(1,395:2969068,14892468:0,292945,0
k1,395:2643355,14892468:-325713
x1,395:2969068,14892468
)
)
g1,395:3185337,14938343
)
x1,395:5259552,14938343
g1,395:5423392,14938343
x1,395:6369732,14938343
g1,395:6533572,14938343
x1,395:8390207,14938343
g1,395:8554047,14938343
x1,395:9900812,14938343
x1,395:10556172,14938343
g1,395:10720012,14938343
x1,395:12304017,14938343
g1,395:12467857,14938343
x1,395:13395847,14938343
k1,396:33377771,14938343:19981924
g1,396:33377771,14938343
)
(1,399:2706922,16511207:30670848,447283,142540
h1,398:2706922,16511207:786432,0,0
x1,398:4512439,16511207
k1,398:4702114,16511207:189675
x1,398:5793944,16511207
x1,398:6512219,16511207
k1,398:6701867,16511207:189648
x1,398:8848827,16511207
k1,398:9038502,16511207:189675
x1,398:9475627,16511207
k1,398:9665302,16511207:189675
x1,398:10466152,16511207
k1,398:10655827,16511207:189675
x1,398:11966547,16511207
k1,398:12156221,16511207:189674
x1,398:13248051,16511207
x1,398:13966326,16511207
k1,398:14155975,16511207:189649
x1,398:16576875,16511207
k1,398:16766550,16511207:189675
x1,398:17604100,16511207
k1,398:17793774,16511207:189674
x1,398:18885604,16511207
x1,398:19603879,16511207
k1,398:19793528,16511207:189649
x1,398:21759608,16511207
k1,398:21949283,16511207:189675
x1,398:23041768,16511207
k1,398:23231442,16511207:189674
x1,398:24031637,16511207
k1,398:24221312,16511207:189675
x1,398:26404972,16511207
k1,398:26594647,16511207:189675
x1,398:27358797,16511207
k1,398:27548472,16511207:189675
x1,398:28640302,16511207
x1,398:29358577,16511207
k1,398:29548225,16511207:189648
x1,398:30421820,16511207
k1,398:30611495,16511207:189675
x1,398:33377770,16511207
k1,398:33377770,16511207:0
)
(1,399:2706922,17297639:30670848,447283,142540
x1,399:3980942,17297639
g1,398:4144782,17297639
x1,398:4945632,17297639
g1,398:5109472,17297639
x1,398:6201302,17297639
x1,398:6919577,17297639
g1,398:7083417,17297639
x1,398:9340477,17297639
g1,398:9504317,17297639
x1,398:11815117,17297639
k1,399:33377769,17297639:21562652
g1,399:33377769,17297639
)
(1,401:2706922,18084071:30670848,449576,142540
h1,400:2706922,18084071:786432,0,0
x1,400:5057699,18084071
x1,400:6283222,18084071
k1,400:6482249,18084071:199027
x1,400:7756269,18084071
k1,400:7955295,18084071:199026
x1,400:8956685,18084071
k1,400:9155712,18084071:199027
x1,400:9993262,18084071
k1,400:10192289,18084071:199027
x1,400:11466964,18084071
k1,400:11665991,18084071:199027
x1,400:11884226,18084071
x1,400:12486502,18084071
k1,400:12685528,18084071:199026
x1,400:16399453,18084071
k1,400:16598480,18084071:199027
x1,400:19001685,18084071
k1,400:19200712,18084071:199027
x1,400:19746627,18084071
k1,400:19945653,18084071:199026
x1,400:20746503,18084071
k1,400:20945530,18084071:199027
x1,400:22037360,18084071
x1,400:22755635,18084071
k1,400:22954626,18084071:198991
x1,400:25211686,18084071
k1,400:25410713,18084071:199027
x1,400:27812608,18084071
k1,400:28011635,18084071:199027
x1,400:28557550,18084071
k1,400:28756577,18084071:199027
x1,400:29411937,18084071
k1,400:29610963,18084071:199026
x1,400:31904068,18084071
k1,400:32103095,18084071:199027
x1,400:33377770,18084071
k1,400:33377770,18084071:0
)
(1,401:2706922,18870503:30670848,447283,142540
x1,401:2997902,18870503
k1,400:3225161,18870503:227259
x1,400:3843821,18870503
x1,400:4300607,18870503
k1,400:4527865,18870503:227258
x1,400:5747490,18870503
x1,400:6038470,18870503
k1,400:6265729,18870503:227259
x1,400:7103279,18870503
k1,400:7330538,18870503:227259
x1,400:7767663,18870503
k1,400:7994921,18870503:227258
x1,400:9196196,18870503
k1,400:9423455,18870503:227259
x1,400:11025155,18870503
k1,400:11252414,18870503:227259
x1,400:13473429,18870503
k1,400:13700688,18870503:227259
x1,400:17413958,18870503
k1,400:17641216,18870503:227258
x1,400:18296576,18870503
x1,400:20828232,18870503
k1,400:21055491,18870503:227259
x1,400:22329511,18870503
k1,400:22556770,18870503:227259
x1,400:23357620,18870503
k1,400:23584878,18870503:227258
x1,400:24713408,18870503
k1,400:24940667,18870503:227259
x1,400:27919933,18870503
x1,400:29060259,18870503
x1,400:30062960,18870503
x1,400:33172643,18870503
x1,400:33377770,18870503
k1,401:33377770,18870503:0
)
(1,401:2706922,19656935:30670848,447283,105513
x1,401:6125280,19656935
x1,401:8709365,19656935
x1,401:9655705,19656935
x1,400:10191789,19656935
x1,400:12994764,19656935
x1,400:14268784,19656935
k1,401:33377770,19656935:19108986
g1,401:33377770,19656935
)
]
(1,402:2706922,44691685:30670848,0,0
h1,402:2706922,44691685:30670848,0,0
)
]
]
]
!11883
}6
Input:59:D:\Narendra_Journals\Elsevier\Procedia_Templates\13-03-2019\TRPRO_EWGT_2018_TeX_Template\trpro-template-EWGT_2018.aux
!137
Postamble:
Count:3484
!27
Post scriptum:

